An All-Sky Search for Bursts of Very High Energy Gamma Rays with HAWC

A new ground-based wide-field extensive air shower array known as the High-Altitude Water Cherenkov (HAWC) Observatory promises a new window to monitoring the $\sim$100 GeV gamma-ray sky with the potential for detecting a high energy spectral cutoff in gamma-ray bursts (GRBs). It represents a roughly 15 times sensitivity gain over the previous generation of wide-field gamma-ray air shower instruments and is able to detect the Crab Nebula at high significance ($>$5 $\sigma$) with each daily transit. Its wide field-of-view ($\sim$2 sr) and $>$95% uptime make it an ideal instrument for detecting GRB emission at $\sim$100 GeV with an expectation for observing $\sim$1 GRB per year based on existing measurements of GRB emission. An all-sky, self-triggered search for VHE emission produced by GRBs with HAWC has been developed. We present the results of this search on three characteristic GRB emission timescales, 0.2 seconds, 1 second, and 10 seconds, in the first year of the fully-populated HAWC detector which is the most sensitive dataset to date. No significant detections were found, allowing us to place upper limits on the rate of GRBs containing appreciable emission in the $\sim$100 GeV band. These constraints exclude previously unexamined parameter space.

==> Abbreviations-supertabular.tex <==
%List of Abbreviations


\renewcommand{\baselinestretch}{1}
\small\normalsize
\hbox{\ }

\vspace{-4em}

\begin{center}
\large{List of Abbreviations}
\end{center} 

\vspace{3pt}

\begin{supertabular}{ll}
AAA & Antiaircraft artillery \\
ABCCC & Airborne Battlefield Command and Control Center \\
AEHF & Advanced Extremely High Frequency \\
AGM & Air-to-ground guided missile \\
AIT & Assembly, Integration, and Testing \\
AOR & Area of Responsibility \\
APAM & Anti-personnel, anti-material \\
ASOC & Air Support Operations Center \\
ATACM & Army Tactical Missile System \\
ATO & Air Tasking Order \\
AWACS & Airborne Warning and Control System \\
\\
BAT & Brilliant Ani-Armor Submunition \\
BDA & Bomb-damage assessment  \\
BFT & Blue Force Tracking \\
BLOS & Beyond Line-of-Sight \\
BMD & Ballistic Missile Defense \\
\\
C$^{3}$ & Command, Control, and Communications \\
CAFMS & Computer-aided Force Management System \\
CALCM & Conventional Air-Launched Cruise Missile \\
CBU & Cluster Bomb Unit \\
CCAFS & Cape Canaveral Air Force Station \\
CENTAF & CENTCOM's Air Force component \\
CENTCOM & U.S. Central Command \\
CINC & Commander-in-Chief \\
CONUS & Continental United States \\
\\
DAGR & Defense Advanced GPS Reciever \\
DMA & Defense Mapping Agency \\
DOD & Department of Defense \\
DOP & Dilution of Precision \\
DOT & Department of Transportation \\
DSMAC & Digital Scene Mapping Area Correlator \\
\\
EFOG-M & Enhanced Fiber Optic Guided Missile \\
\\
FAA & Federal Aviation Administration \\
FLIR & Forward-looking infrared \\
\\
GAM & Global Positioning System Aided Munition \\
GPS & Global Positioning System \\
GWAPS & Gulf War Air Power Survey \\
\\
HARM & High-Speed Antiradiation Missile \\
HEO & Highly Elliptical Orbit \\
\\
IADS & Integrated Air Defense System \\
ICBM & Inter-Continental Ballistic Missile \\
INS & Inertial navigation system \\
IIR & Imaging infrared \\
IR & Infrared \\
ISR & Intelligence, Surveillance, and Reconnaissance \\
\\
JDAM & Joint Direct Attack Munition \\
JFC & Joint Force Commander \\
JSOW & Joint Standoff Weapon \\
\\
LANTIRN & Low-Altitude Navigation and Targeting Infrared for Night System \\
LEO & Low Earth Orbit \\
LGB & Laser-guided bomb \\
\\
MAJIC & Microsatellte Area-Wide Joint Information Communication \\
MARCENT & CENTCOM's Marine component \\
MARS & Mid-Atlantic Regional Spaceport \\
MLRS & Multiple Launch Rocket System \\
MUOS & Mobile User Objective System \\
\\
NASA & National Aeronautics and Space Administration \\
NAVCENT & CENTCOM's Navy component \\
NPOESS & National Polar-Orbiting Operational Environmental Satellite System \\
\\
ORS & Opertionally Responsive Space \\
ORSO & Operationally Responsive Space Office \\
\\
PDOP & Position Dilution of Precision \\
PGM & Precision-guided munition \\
P$^{3}I$ & Preplanned Product Improvement \\
PnP & Plug and Play \\
PnPSat & Plug and Play Satellite \\
PPS & Precise Positioning Service \\
\\
RCS & Radar cross section \\
\\
SA & Situational Awareness \\
SADARM & Sense and Destroy Armor Munition \\
SAM & Surface-to-air missile \\
SAR & Synthetic aperture radar \\
SBIRS & Space Based Infrared System \\
SEAD & Suppression of enemy air defenses \\
SFW & Sensor Fuzed Weapon \\
SIGINT & Signal Intelligence \\
SLAM & Standoff Land Attack Missile \\
SLAM-ER & SLAM-Expanded Response \\
SpaceX & Space Exploration Technologies Corporation \\
SPS & Standard Positioning Service \\
\\
TACC & Tactical Air Control Center \\
TACS & Tactical Air Control System \\
TACP & Tactical Air Control Party \\
TASM & Tomahawk Anti-Ship Missile \\
TBIP & Tomahawk Baseline Improvement Program \\
TERCOM & Terrain Contour Mapping \\
TFR & Terrain-following radar \\
TLAM & Tomahawk Land Attack Missile \\
\\
USAF & U.S. Air Force \\
\\
VAFB & Vandenberg Air Force Base \\
\\
WGS & Wideband Global SATCOM \\
%$\alpha$ & alpha \\
%$\beta$  & beta \\
%&  \\ 
%IREAP & Institute for Research in Electronics and Applied Physics \\
%NSA & National Security Agency
\end{supertabular}


==> Acknowledgements.tex <==
%Acknowledgments

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{-.65in}

\begin{center}
\large{Acknowledgments} 
\end{center} 

\vspace{1ex}
Many thanks to Jordan and Andy.


==> Chapter1.tex <==
%Chapter 1

\renewcommand{\thechapter}{1}

\chapter{Introduction}

\section{Source of Nonlinearity in an Optical Fiber}

The response of any dielectric to light becomes nonlinear
for intense electromagnetic fields.  Standard optical fibers are made of
fused silica which is a dielectric. The total polarization $\bf{P}$
is nonlinear in the electric field $\bf{E}$ and is given by [1-5] -
%\cite{Agrawal1,Bloembergen,Shen,Butcher,Boyd} -
%1.1
\begin{equation}
{\bf P} = \epsilon_{0} \left( \chi^{(1)} : {\bf E} + \chi^{(2)} 
: {\bf EE} + \chi^{(3)} : {\bf EEE} + \ldots \right),
\end{equation}
where $\epsilon_0$ is the permittivity of free-space, and
$\chi^{(j)}$ 
is the ${\it j}$-th order susceptibility of the dielectric. The linear
susceptibility $\chi^{(1)}$ represents the dominant contribution to
$\bf{P}$ and its effects are included through the refractive index
n($\omega$) and the attenuation coefficient $\alpha(\omega)$. $\chi^{(2)}$
is responsible for nonlinear effects such as sum-frequency generation and
second harmonic generation \cite{Agrawal1, Shen}. Fused silica does not
manifest these effects as it is centro-symmetric \cite{Newell}. Hence, the dominant nonlinear
contribution to ${\bf P}$ is due to $\chi^{(3)}$ which results in effects
such as third harmonic generation, four-wave-mixing,  self- and
cross-phase modulation. The cubic nonlinearity results in an intensity
dependent refractive index

\begin{verbatim}
122	23333
1114	14444
\end{verbatim}

%1.2
\begin{equation}
\tilde{n}(\omega,|E|^2) = n(\omega)+n_2|E|^2 ,
\end{equation}
where n($\omega$) is the linear part given by the Sellmier
equation which
takes into account the resonance frequencies ($\omega_j$) of fused
silica \cite{Agrawal1,Marcuse},
%1.3
\begin{equation}
n^2(\omega) = 1 + \sum_{j=1}^m {B_j\omega^2_j \over \omega^2_j - \omega^2}
\end{equation}
and n$_2$ is given by
%1.4
\begin{equation}
n_2 = {3 \over 8n}Re(\chi_{xxxx}^3)
\end{equation}
for an optical wave assumed to be linearly polarized along one of the 
axes of a polarization maintaining fiber. The tensorial nature of $\chi^{(3)}$ needs to be
considered for the case in which the light is not polarized along one of
the fiber axes.\footnote{This is my footnote.  I started playing the piano when I was eight years old.  This is my footnote.  I started playing the piano when I was eight years old.  This is my footnote.  I started playing the piano when I was eight years old.  This is my footnote.  I started playing the piano when I was eight years old.}

The following is an equation array to ensure the long equation does not go outside the margins.
\begin{eqnarray}
W & = & \int d^3{\bf r} \left[ \sum_s \left( \int d^3{\bf v} {T_{0s} \langle h^2_s \rangle {\bf r} \over 2F_{0s}} - {q^2_s\varphi^2 n_{0s} \over T_{0s}} \right) + {|\delta {\bf B}|^2 \over 8 \pi} \right] \nonumber \\
& = & \int d^3{\bf r} \left( \sum_s \int d^3{\bf v} {T_{0s}\delta f^2_s \over 2F_{0s}} + {|\delta {\bf B}|^2 \over 8\pi} \right) .
\end{eqnarray} 

The experimentally measured value of $n_{2}$ for fused silica ranges from $2.2 - 3.4 \times
10^{-20}$\,m$^2$/W, which is small compared to most other nonlinear media by
at least 2 orders of magnitude \cite{Agrawal1}. Despite this, nonlinear effects are
easily observed for silica fibers for relatively low input power levels due
to the fact that the effective fiber core areas are small and the fiber losses are low. 
Single mode fibers (those which propagate a single transverse mode of light for a given 
wavelength) have effective fiber core diameters of the order of 5$\mu$m thus causing 
the light intensities within the fiber to be large despite the smallness of the input 
power. The low loss in the fiber ($<$10 dB/km) allows one to use long fibers to observe 
nonlinear phenomena.

\section{Physics of Pulse Propagation}

Mathematically speaking, in the classical limit, pulse propagation in an
optical fiber is governed by Maxwell's equations \cite{Agrawal2,Diament}, 
%1.5
\begin{eqnarray} 
\vec{\nabla}\times\vec{E} & = &- {\partial \vec{B} \over \partial t} \nonumber\\
\vec{\nabla}\times\vec{H} & = & \vec{J}+ {\partial \vec{D} \over \partial t}
\nonumber\\ 
\vec{\nabla}\cdot\vec{D} & = & \rho_{f} \nonumber\\
\vec{\nabla}\cdot\vec{B} & = & 0 ,
\end{eqnarray}
where $\vec{E}$ and $\vec{H}$ are electric and magnetic field
vectors, and
$\vec{D}$ and $\vec{B}$ are electric and magnetic flux densities, 
respectively. $\vec{J}$ is the current density and $\rho_{f}$ is the free
charge density.

This is the second equation array.
\begin{eqnarray}
W & = & \int d^3{\rm r} \left[ \sum_s \left( \int d^3{\rm v} \right){T_{s} \langle h^2_s \rangle {\rm r} \over 2F_{0s}} \right] + {|\delta \rm B|^2 \over 8\pi} \nonumber \\ 
& = & \int d^3 
\end{eqnarray}

Under the following assumptions \cite{Agrawal2} -
\begin{enumerate}
\item[(a)]
there are no free charges ($\vec{J}=\rho_{f}=0$), a good approximation for an optical fiber, 
\item[(b)] the medium is non-magnetic ($\vec{M}=0$), which an optical fiber is,
\item[(c)] the wavelength of light propagated is away from any material
resonances (0.5 - 2 $\mu$m), the results described in this thesis lie in this wavelength range, i.e., the results presented in Chap.\ 2 and Chap.\ 3 lie in the 600-700\,nm regime and the results presented in Chap.\ 4 lie in the 800\,nm regime,
\item[(d)] the electric-dipole approximation is valid, due to which the second-order parametric processes such as three-wave-mixing and second harmonic generation can be neglected (in practice they do occur because of quadrupole and magnetic-dipole effects but with a very low efficiency),
\item[(e)] the medium only responds locally, which is a valid approximation for the projects considered herein,
\item[(f)] the nonlinear polarization $\vec{P}_{NL}$ can be taken as a
perturbation to the total induced polarization $\vec{P}$, which is justified as the nonlinear effects are relatively weak for the results presented in this thesis,
\item[(g)] only 3rd order nonlinear effects need to be taken into
account, which is valid up to 5th order in ${\bf E}$ since the 2nd and 4th order effects are absent due to the centrosymmetric nature of the disordered liquidlike state of fused silica,
\item[(h)] the imaginary part of the dielectric constant
$\epsilon(\omega)$ is small compared to the real part (low loss, which is a good approximation for the wavelength regimes and fiber lengths considered here),
\item[(i)] the wavelength of light is higher than the cutoff wavelength
of the fiber so that the single transverse mode condition is satisfied (or else there would be multimode propagation and nonuniform modal dispersion would have to be taken into account),
\item[(j)] the optical fiber is polarization maintaining and the light
pulse is traveling along one of the 2 principal axes of the fiber, a very good approximation for the results of Chap.\ 2, and Chap.\ 3, in the case of Chap.\ 4, this approximation is relaxed as the incident light travels along both axes of the fiber, thus requiring a set of two coupled NLSEs for simulation, one for each axis,
\item[(k)] the slowly varying envelope approximation is valid, i.e.,
$\Delta\omega/\omega_{0} \ll 1$ where $\Delta \omega$ is the spectral
width of the pulse spectrum which is centered at $\omega_{0}$, this approximation is valid for the studies considered in Chap.\ 2 and Chap.\ 4, in Chap.\ 3, the Raman Stokes wave is considered as a separate slowly varying envelope from the pump wave, as the two taken together would not satisfy this condition,
\item[(l)] the nonlinear response of the medium is instantaneous, an
approximation valid for pulse widths greater than $\sim$70\,fs, which amounts to neglecting the contribution of molecular vibrations to $\chi^{(3)}$ (the Raman effect), which have been included in the study presented in Chap.\ 4 since the pulse width was $\sim$ 140\,fs.
\end{enumerate}
The propagation of the slowly varying envelope A(z,t) of a light
pulse
along an optical fiber is governed by the nonlinear partial
differential equation \cite{Agrawal2} -
%1.6
\begin{equation}
{\partial A \over \partial z} + \beta_{1} {\partial A \over \partial t} + {i \beta_{2} \over 2} {\partial^{2} A \over \partial t^{2}} = i \gamma |A|^{2}A,
\end{equation}
where $v_{g}=1/\beta_{1}$ is the group velocity of the pulse,
$\beta_{2}$
is the group velocity dispersion coefficient, %$\alpha$ is the fiber loss,
and $\gamma$ is the nonlinearity coefficient given by
%1.7
\begin{equation}
\gamma = {n_{2}\omega_{0} \over c A_{eff}} .
\end{equation}

Here $\omega_{0}$ is the central angular frequency of the pulse and
A$_{eff}$, the effective core area of the fiber.

Under transformation to  a frame of reference moving at the group
velocity of the pulse, the above equation takes the form of the so-called
`nonlinear Schr\"odinger equation' (NLSE), i.e.,
%1.8
\begin{equation}
{\partial A \over \partial z} + {i\beta_2 \over 2} {\partial^2
A \over \partial \tau^2} = i \gamma |A|^2A ,
\end{equation}
where
%1.9
\begin{equation}
\tau = t - {z \over v_g}
\end{equation}
is time measured in a frame of reference moving at the group
velocity
v$_g$ of the pulse.

\section{Numerical Pulse Propagation}

The NLSE, like most nonlinear partial differential equations, is not
amenable to analytical solution except in certain special cases where the
inverse scattering transform can be used \cite{Zakharov}. Thus a
numerical approach is necessary for understanding the physics of phenomena
governed by the NLSE. The numerical methods available can be classified as
finite-difference techniques and pseudo-spectral techniques. Usually
pseudo-spectral methods are an order of magnitude faster, the most
popular method being the Split-Step Fourier Method (SSFM) \cite{Agrawal2,Hardin,
Fisher}. The speed of the SSFM can be partly attributed to the use
of the finite fast-Fourier transform (FFT) algorithm
\cite{Cooley}.For an algorithmic description of the SSFM the reader is
referred to Chap.\ 2, Sec.\ 2. Therein is also described an
unconditionally stable scheme for including linear multiplicative noise into
the SSFM without disturbing the conservative properties of the NLSE. In the
projects described in Chap.\ 3, simulations were carried out using a
combination of the SSFM and finite difference schemes. The SSFM is also used 
 to arrive at the simulated results described in Chap.\ 4.

\section{Experimental Pulse Diagnostics}

With the advent of frequency resolved optical gating
(FROG) \cite{Trebino,Kanejqe,Kaneoptlett}, it has become possible to not
only measure the optical spectrum and optical time trace of a light pulse
but to measure the full electric field envelope (intensity and phase) of the
light pulse. The two fields of nonlinear fiber optics and frequency resolved
optical gating (FROG) are yet to undergo cross pollination to their fullest
potential since the inception of FROG 10 years ago. This novel experimental
technique adds new dimensions to pulse measurement techniques, one of which
is the ability to measure how asymmetric a pulse is, i.e., measure its
skewness, kurtosis and all higher order moments. Asymmetric pulse
propagation is a subject of interest in Chap.\ 4, where a highly simplified
version of FROG \cite{OShealett} is used to measure pulse characteristics
before and after a fiber.

\section{Group Velocity Dispersion}

Group velocity dispersion \cite{Agrawal3} (GVD) involves the temporal broadening of a pulse as it propagates through an optical fiber. From the NLSE (Eq.\ 1.6) one can derive length scales relevant to linear dispersion (L$_{D}$=T$_{0}^{2}$/$\beta_{2}$) and nonlinearity (L$_{NL}$=1/$\gamma$P$_{0}$). Here T$_{0}$ is the pulse width and P$_{0}$ is the peak power of the pulse. The regime in which the effects of GVD dominate and the effects of nonlinearity are negligible is given by -
%1.10
\begin{equation}
{L_{D} \over L_{NL}}={\gamma P_{0} T_{0}^{2} \over |\beta_{2}|} \ll 1 .
\end{equation}

In this regime, optical pulses propagate as they undergo symmetric temporal broadening and linear chirping without any spectral broadening. The sign of the GVD parameter $\beta_{2}$ determines the sign of the induced chirp. If the input pulse is chirped, then it may undergo some initial pulse compression followed by temporal broadening. Unlike the second-order dispersion associated with GVD, third-order dispersion causes asymmetric temporal broadening with leading and trailing edges. It becomes important, when the operating wavelength is near the zero dispersion wavelength of the fiber (the wavelength at which $\beta_{2}$=0). GVD starts to limit optical fiber communication systems when consecutive pulses broaden so much that they start to overlap.   

\section{Self-Phase Modulation}

Self-phase modulation \cite{Agrawal4} (SPM) is a phenomenon that leads to spectral broadening and modulation of optical pulses. In the absence of GVD, SPM induced spectral broadening occurs without change in the temporal pulse shape. The spectral broadening occurs as a consequence of an intensity dependent phase-shift. The project described in Chap.\ 2 has the property that L$_{NL}$ $<$ L $\ll$ L$_D$, i.e., the nonlinear term representing SPM dominates. In the regime where both SPM and GVD are non-negligible (as in Chap.\ 4), phenomena qualitatively different from those described in this section and the previous section can occur. Both temporal and spectral broadening can occur simultaneously. In the regime of femtosecond pulse propagation (as in Chap.\ 4), GVD, third-order dispersion, intrapulse Raman scattering (discussed in Chap.\ 2) and higher order nonlinear effects have to be taken into account. If the input pulse is asymmetric, then SPM effects dominate over all other effects, as is observed in Chap.\ 3. In some cases SPM can lead to pulse compression, and in the anomalous dispersion regime ($\beta_2 < 0$), the balance between GVD and SPM can lead to soliton formation. 

\section{Four-wave-mixing}

Four-wave-mixing (FWM) \cite{Agrawal10} is a parametric process involving
the interaction
between four photons at different frequencies. Two different kinds of
four-wave-mixing processes are possible -
%1.11
\begin{eqnarray}
\omega_4 = \omega_1 + \omega_2 + \omega_3 \\
\omega_3 + \omega_4 = \omega_1 + \omega_2 .
\end{eqnarray}

The former process results in third harmonic generation for the special case
when $\omega_1 = \omega_2 = \omega_3$. Both processes require phase
matching to occur, in order to be efficient. For the latter case, with
the partial degeneracy of $\omega_1 = \omega_2$, it is relatively easy
to satisfy the phase matching condition of
%1.12
\begin{equation}
\Delta k = k_3 + k_4 - k_1 - k_2 = 0 .
\end{equation}

This process is of great interest to nonlinear dynamicists as the
evolution of the FWM process could constitute a route to chaos further
down-stream in the fiber. It is also of great interest to people working in
the field of optical communication systems, as it can cause cross-talk
between neighboring channels in a wavelength division multiplexing scheme
of communication.

\section{Cross-Phase Modulation}

Cross-phase modulation (XPM) \cite{Agrawal7} occurs in optical fibers when
two or more optical pulses having different central wavelengths propagate 
simultaneously inside a fiber, interacting through the fiber
nonlinearity which couples the two pulses nonlinearly.  The evolution of the
two pulses depends on the group velocity mismatch between them by virtue of 
their being centered at different wavelengths, although this is a linear
phenomenon. The group velocity mismatch also exists between light pulses
traveling along orthogonal polarization axes of a fiber, and centered around
identical wavelengths, since the slow axis and fast axis of the fiber have
different group velocities. In this case, too, the two polarizations interact
nonlinearly \cite{Agrawal6} through degenerate XPM (degenerate since the
central wavelengths are the same). In the case of degenerate XPM the 2nd order 
and higher dispersion parameters, and the nonlinear parameters (all of which
depend only on the wavelength), are also the same unlike in general XPM. The 
effects of XPM are more pronounced when one of the pulses (the pump) has much 
higher power than the other (the probe). Otherwise, the effects of self-phase 
modulation (SPM) tend to dominate.

\section{Stimulated Inelastic Scattering} 

Other nonlinear effects (apart from those due to the cubic $\chi^{(3)}$
nonlinearity) arise due to the interaction between the light
traveling in the fiber and the fiber medium. Interactions between
the light field and the vibrational levels of the fiber medium lead to
stimulated Brillouin scattering (SBS) and stimulated Raman
scattering (SRS). SRS and SBS were among the first nonlinear effects
studied in optical fibers \cite{Stolen,Ippen,Smith}.  In a simple quantum
mechanical picture \cite{Agrawal1} applicable to
both SRS and SBS, a photon of the incident field (called the pump) is
annihilated to create a photon at a lower frequency (belonging to the
Stoke's wave) and a phonon to conserve energy and momentum. SBS involves
an acoustic phonon whereas SRS involves an optical phonon, thus they have
qualitatively different dispersion relations. SBS has a much
lower threshold power and manifest itself through a backward propagating
wave in contrast to SRS which can involve both forward and backward
traveling waves. SBS has a maximum gain at a frequency 10\,GHz \cite{Agrawal9}
(down-shifted with respect to the pump) and
requires a very narrow bandwidth pump to manifest itself. SRS, in
contrast, has a maximum gain at a frequency 13\,THz \cite{Agrawal8} downshifted with
respect to the pump. For pulse-bandwidths larger than 13\,THz, the
phenomenon of Intrapulse Raman Scattering (IRS) manifests itself,
involving a self-frequency shift within the pulse from higher frequency
components to lower frequency components. Thus, SRS
becomes more important for shorter pulses (larger bandwidth) unlike SBS
which nearly ceases to occur for pulses shorter than 10\,ns. In both SRS
and SBS, the optical fiber plays an active role in the nonlinear process,
unlike the case of cross- and self-phase modulation, four-wave-mixing and
third harmonic generation, where the fiber plays a passive role by
mediating the interaction between several optical waves.

\section{Outline of Thesis}

In Chap.\ 2, we present the results of a computational study of the
influence of stochasticity on the dynamical evolution of multiple 
four-wave-mixing processes in a single mode optical fiber with spatially
and temporally $\delta$-correlated phase noise. A generalized nonlinear
Schr\"odinger equation (NLSE) with stochastic phase fluctuations along the
length of the fiber is solved using the Split-step Fourier method
(SSFM). Good agreement is obtained with previous experimental and
computational results based on a truncated-ODE (Ordinary Differential
Equation) model in which stochasticity was seen to play a key role in
determining the nature of the dynamics. The full NLSE allows for
simulations with high frequency resolution (60\,MHz) and frequency span (16
THz) compared to the truncated ODE model (300\,GHz and 2.8\,THz,
respectively), thus enabling a more detailed comparison with
observations. A physical basis for this hitherto phenomenological phase
noise is discussed and quantified.

In Chap.\ 3, we discuss the implications of spontaneous and stimulated
Raman scattering on the project discussed in Chap.\ 2, namely, the dynamical evolution of 
stochastic four-wave-mixing processes in an optical fiber.
The following question is asked - can stimulated Raman scattering be a mechanism by which
adequate multiplicative stochastic phase fluctuations are introduced in the 
electric field of light undergoing four-wave-mixing as? Adequately checked numerical
algorithms of stimulated Raman scattering (SRS), spontaneous Raman generation and intrapulse 
Raman scattering (IRS) are used while exploring this issue. The algorithms are described in detail, as also are 
the results of the simulations. It is found that a 50-meter length of fiber (as used in the experiments),
is too short to see the influence of Raman scattering, which is found to eventually 
dominate for longer fiber lengths.

In Chap.\ 4, self- and cross-phase modulation (XPM) of femtosecond pulses ($\sim$ 810
nm) propagating through a birefringent single-mode optical fiber ($\sim$ 6.9
cm) is studied both experimentally (using GRENOUILLE - Grating Eliminated 
No Nonsense Observation of Ultrafast Laser Light Electric Fields) 
%(using second harmonic
%generation-frequency resolved optical gating or SHG-FROG) 
and numerically
(by solving a set of coupled nonlinear Schr\"odinger equations or
CNLSEs). An optical spectrogram representation is derived from the
electric field of the pulses and is linearly juxtaposed with the
corresponding optical spectrum and optical time-trace. The effects of
intrapulse Raman scattering (IRS) are discussed and the question whether 
it can be a cause of asymmetric tranfer of pulse energies towards longer 
wavelengths is explored. The simulations are shown to be in good qualitative 
agreement with the experiments. Measured input pulse asymmetry, when incorporated 
into the simulations, is found to be the dominant cause of output spectral 
asymmetry. \renewcommand{\baselinestretch}{1} \small\footnotesize
\footnote{These averages are reported
for $45$ `detailed occupational codes', which is an intermediate
occupational classification (between two and three-digit codes)
given by the Current Population Survey (CPS).}
\renewcommand{\baselinestretch}{2} \small\normalsize
The results indicate that it is possible to modulate short pulses both temporally and spectrally by passage through polarization maintaining 
optical fibers with specified orientation and length. The modulation technique is very direct and straightforward. No frequency components of the broadband pulse have to be rejected as the entire spectrum is uniformly modulated. The technique is flexible as the modulation spacing can be varied by varying the fiber length.

Chapter 5 provides the conclusion to the thesis.

\section{Theorems}

\newtheorem{theorem}{Theorem}[chapter]
\begin{theorem}
This is my first theorem.
\end{theorem}


\section{Axioms}
\newtheorem{axiom}{Axiom}[chapter]
\begin{axiom}
This is my first axiom.
\end{axiom}

\begin{axiom}
This is my second axiom in chapter 1.
\end{axiom}

\section{Tables}

This is my table. 

\renewcommand{\baselinestretch}{1}
\small\normalsize

\begin{table}[h]
\caption[Short title]{Overview of test cases used in this study.}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Test & Quality & Setpoint & Manipulated \\
case & variable (QV) & for QV & variables (MVs)\\
\hline \hline
TE & G/H ratio & 1.226 & D-feed SP and Reactor Level SP\\
AZ & xB($H_2O$) & & Reflux flow and $5^{th}$ Tray temperature SP\\  
\hline
\end{tabular}
\end{center}
\label{test_over}
\end{table}

\renewcommand{\baselinestretch}{2}
\small\normalsize

My table is shown above.   Normally it is double-spaced but I have inserted a command (marked in blue) to make it single-spaced and then inserted a command (again in blue) to change the text back to double-spacing.

\

\subsection{Adding Extra Space between Text and Horizontal Lines}

\renewcommand{\baselinestretch}{1}
\small\normalsize

\setlength{\tablinesep}{5ex}

\begin{table}[h]
\caption{Table with Extra Space between the Text and Horizontal Lines.}
\begin{center}
\begin{tabular}{|p{.5in}|p{1in}|c|p{2.25in}|}
\hline
Test case& Quality variable QV)& Setpoint for QV & Manipulated  variables (MVs)\\
\hline \hline
TE & G/H ratio & 1.226 & D-feed SP and Reactor Level SP\\ \hline
AZ & xB($H_2O$) & & Reflux flow and $5^{th}$ Tray temperature SP \\
\hline
\end{tabular}
\end{center}
\label{test_over}
\end{table}

\renewcommand{\baselinestretch}{2}
\small\normalsize

The line \begin{verbatim}\usepackage{tabls}\end{verbatim} must be inserted in the preamble of your document.
The table is set up to be single-spaced by \begin{verbatim} \renewcommand{\baselinestretch}{1} \small\normalsize\end{verbatim} before \begin{verbatim}\begin{table}\end{verbatim}.  I set the first, second, and fourth columns as paragraphs, .5in, 1in, and 2.25in wide, respectively.  I then adjusted the separation between the words and the horizontal lines to 5ex by also adding \begin{verbatim}\setlength{\tablinesep}{5ex}\end{verbatim} before the \begin{verbatim}\begin{table}\end{verbatim} command.

After typing the table I change the document to be double-spaced from this point on.

\newpage


\section{Figures}

The figure on the following page is centered and the figure caption is indented and single-spaced.  Make sure you copy the last two lines \begin{verbatim}
\renewcommand{\baselinestretch}{2}\\
\small\normalsize\end{verbatim} to return to double-spacing of your text.

\begin{figure}
\begin{center}
\includegraphics[width=6in]{../figures/turtle.jpg}
\end{center}
\renewcommand{\baselinestretch}{1}
\small\normalsize
\begin{quote}
\caption[Figure with caption indented]{This figure caption is indented and single-spaced.  Comparison between the experimental measurements \cite{hart1} (black), the random initial condition NLSE model excluding phase noise (dashed curves) and the stochastic phase noise NLSE model (solid curves) showing the first- and second-order sideband evolution as a function of fiber length for P$_{0} = 5.5$\,W, $\Omega = 366$\,GHz, $\Delta\nu = 0.5$\,GHz, $\gamma = 0.019$\,W$^{-1}$m$^{-1}$, and $\beta^{(2)} = 55$\,ps$^2$/km: dynamical evolution of the: (a) power in the first-order blue-shifted sideband, (b) power in the first-order red-shifted sideband, (c) fluctuations in the first-order blue-shifted sideband, (d) fluctuations in the first-order red-shifted sideband, (e) power in the second-order blue-shifted sideband, (f) power in the second-order red-shifted sideband. \label{fig:fig27}}
\end{quote}
\end{figure} 
\renewcommand{\baselinestretch}{2}
\small\normalsize

The first figure is Fig.\ref{fig:fig27}.   Please note that the figure label should be placed inside the figure caption.  
\newpage

The next figure is placed landscape.  It is Fig.~\ref{fig:mpc}.

\begin{landscape}
\renewcommand{\baselinestretch}{1}
\small\normalsize
\begin{quote}
\begin{figure}
\begin{center}
\includegraphics[width=8.2in]{../figures/turtle.jpg}
\end{center}
\caption{Schematic illustrating receding horizon control.
\label{fig:mpc} }
\end{figure}
\end{quote}
\renewcommand{\baselinestretch}{2}
\small\normalsize
\end{landscape}

This is a my second figure which was placed landscape.  Although I have used the same figure, I have renamed the label to fig:mpc-1.  The second figure now becomes Figure~\ref{fig:mpc-1}.
\begin{landscape}
\renewcommand{\baselinestretch}{1}
\small\normalsize
\begin{quote}
\begin{figure}
\begin{center}
\includegraphics[width=8.2in]{../figures/turtle.jpg}
\end{center}
\caption[Figure placed landscape on page]{Schematic illustrating receding horizon control. \label{fig:mpc-1}}
\end{figure}
\end{quote}
\renewcommand{\baselinestretch}{2}
\small\normalsize
\end{landscape}

\subsection{Numbering Figures}

If you wish your figures to be numbered 1-100 without any reference to the chapter (e.g., Figure 1.1, 2.1, etc.), change the first line of your mainthesis.tex file to read \begin{verbatim}"\documentclass[12pt]{thesis-2}".\end{verbatim}  

\subsubsection{This is a Subsubsection}

This is my first subsubsection in Chapter 1.


\section[Short Titles]{Short Titles in the Table of Contents, List of Figures, or List of Tables}

The Table of Contents, List of Figures, or List of Tables usually show the entire title of a section, subsection, etc. or table, or the entire caption of a figure.  If you put a short title in square brackets after \begin{verbatim} \section, \table, or \figure, \end{verbatim} the short title will show in your Table of Contents or lists.

\renewcommand{\baselinestretch}{1}
\small\normalsize

\begin{verbatim}
\section[Short Title]{Title of Section} 
\subsection[Short Title]{Title of Subsection} 
\end{verbatim}

or when using a caption in a figure or table
\begin{verbatim}
\caption[Short Caption]{Full text of the caption.}
\end{verbatim}

\renewcommand{\baselinestretch}{2}
\small\normalsize


\section{Figures on Text Page}

Normally figures in the thesis are placed on a page by themselves.  The following figure is placed on the page with text before and after the figure by adding [!!h] after \begin{verbatim} \begin{figure}[!!h] \end{verbatim}.  Please note that the figure label is placed within the caption.

\renewcommand{\baselinestretch}{1}
\large\normalsize

\begin{verbatim}
\begin{figure}[!!h]
 \begin{center}
\includegraphics[width=5in]{../figures/turtle.jpg}
\end{center}
\caption[Short title]{Schematic illustrating receding horizon control.
\label{fig:mpc-2}}
\end{figure}
\end{verbatim}

\begin{figure}[!!h]
 \begin{center}
\includegraphics[width=5in]{../figures/turtle.jpg}
\end{center}
\caption{Schematic illustrating receding horizon control. \label{fig:mpc-2}}
\end{figure}

\renewcommand{\baselinestretch}{2}
\large\normalsize

This does not necessarily mean that the text before and after the figure will be exactly what you want.  Remember Latex will place the figure where it will fit on the page the best.   The previous figure is Figs.~\ref{fig:mpc-2}. 

\section{Wrapping Text around Figure}


\renewcommand{\baselinestretch}{1}
\begin{wrapfigure}{r}{0.4\textwidth}
\includegraphics[width=0.4\textwidth]{../figures/turtle.jpg}
\caption{ Text wrap around figure. \label{fig:test}}
\end{wrapfigure}

\renewcommand{\baselinestretch}{2}
\large\normalsize

By way of summary, at the end of the activity, I reminded the class of what we'd done:  by considering relatively nearby galaxies whose distance we had measured by some other means, we were able to establish a relationship locally between redshift and distance.  
By way of summary, at the end of the activity, I reminded the class of what we'd done:  by considering relatively nearby galaxies whose distance we had measured by some other means, we were able to establish a relationship locally between redshift and distance.  
By way of summary, at the end of the activity, I reminded the class of what we'd done:  by considering relatively nearby galaxies whose distance we had measured by some other means, we were able to establish a relationship locally between redshift and distance.  
By way of summary, at the end of the activity, I reminded the class of what we'd done:  by considering relatively nearby galaxies whose distance we had measured by some other means, we were able to establish a relationship locally between redshift and distance.  See Fig.~\ref{fig:test}.


\section{LaTeX -- A Typesetting Program}

A 13-page explanation of some of the features of LaTeX can be downloaded from http://www.jgsee.kmutt.ac.th/exell/General/LaTeX.html.


\section{Using Bibtex}

Using Bibtex with Latex documents is not difficult.  The bulk of the work is organizing your bibtex file, which is a data base compiled by you of the articles, books, etc. which you use in the bibliographies or reference sections of your publications.  

I have linked several files to this webpage, which will be helpful when you are using Bibtex.  These files can be downloaded from \newline
http://www.ireap.umd.edu/ireap/theses/bibtex.  Please read the file "BibtexInstructions.pdf".  The first two pages explain how to set up and run Bibtex; the remaining pages were taken from a published article and show how the references were cited in the .tex file.   The files BibtexInstructions.tex, Galactic.bib, Dottie.bib are the original .tex files used for BibtexInstructions.pdf.  The file BibtexSamples.tex contains examples of the information needed for the various publications you wish to reference (e.g., articles in refereed journals, books, unpublished articles, conference proceedings, etc.).

If you have questions concerning Bibtex, please contact me at 301-405-4955 or dbrosius at umd.edu.

\section{Using Natbib}

Another option of citing references in the bibliography is using Natbib instead of Bibtex.  You must still create a bibtex file, as noted above.  The command "backslash cite" cannot be used with natbib; instead "backslash citet" and "backslash citep" must be used.    "backslash citet" is used to show reference in the text (e.g., Eq.\ 8 in Reiser,1996 shows ...); "backslash citep" is used in the parenthetical (e.g., Eq.\ 8 (Reiser, 1996) shows ...).  

\begin{verbatim}
Add in preamble -- \usepackage[option]{natbib} 

Add at bottom of mainthesis.tex file --
\bibliography{name of your bibtex file}
\bibliographystyle{plainnat, abbrnat, or unsrtnat}
\end{verbatim}

Typesetting:   Latex, Bibtex, Latex, Latex

The reference sheet for natbib usage can be found at \newline "http://merkel.zoneo.net/Latex/natbib.php".

\section{APS Physical Review Style and Notation Guide}

The following style guide may be downloaded from The American Physical Society at http://forms.aps.org/author/styleguide.pdf:  Physical Review Style and Notation Guide, published by The American Physical Society, compiled and edited by Anne Waldron, Peggy Judd, and Valerie Miller, February 1993.  It may be old, but it is very useful.



==> Dedication.tex <==
%Dedication

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }

\vspace{-.65in}

\begin{center}
\large{Dedication}
\end{center}

To John Pretz, master of Science.


==> Foreword.tex <==
%Foreword

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{-.65in}

\begin{center}
\large{Foreword} 
\end{center} 

If needed.


==> GRB130427A.tex <==
redshift was z = 0.34. What does gilmore say about EBL here?

a very crude model for EBL at z = 0.34 is a 250 GeV cutoff.
a cutoff at 50 Get is more like z = 1
a cutoff at 125 GeV is more like a z = 0.5

divide spectrum into 3 regions:
  (4.5 to 11.5s) bulk of lower energy emission happens here. Not much high-E though, power law with A = 189 photons / (cm^2 s keV), Index = -3.34, Epiv = 100 keV
  (11.5 to 33s) has high energy emission happens here. Power law with A = 4.2e-4 photons / (cm^2 s keV), Index = -1.66, Epiv = 100 keV
  (33 to 196s) longest timescale but smallest A. Power law with A = 1.6e-6 photons / (cm^2 s keV), Index = -1.22, Epiv = 100 keV


==> Preface.tex <==
%Preface

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{-.65in}

\begin{center}
\large{Preface}
\end{center}

Depite the observational and theoretical advances made in the nearly 50 years since
the discovery of gamma-ray bursts (GRBs) many open questions remain. In particular,
relatively little is known about the behavior of prompt GRB emission at the highest
energies which is a regime of interest both for its ability to probe the phyiscial environment
of GRBs as well as the density of light in the high redshift Universe. The primary purpose of our
study is therefore to provide a measurement of GRB emission in the very-high energy (VHE) regime.

In Chapter 1 we present an overview of the major observational advances that have
informed the theoretical model for GRB emission. In doing so we emphasize the 
observational difficulties associated with performing measurements of GRB emission
at VHE energies in current ground-based Imaging Air Chereknov Telescopes and satellite-based experiments.
We use this to motivate the need for a new ground-based, wide-field gamma-ray experiment known
as the High-Altitude Water Cherenkov (HAWC) Observatory which expects to observe $\sim$1 GRB per year at
VHE photon energies.

In Chapter 2 we describe the physical processes behind the development of air showers measured in
ground-based observational techniques to inform our discussion of the experimental design of the HAWC
Observatory in Chapter 3 and its methodology for air shower reconstruction in Chapter 4.

Cite something to remove compile warning \cite{Vlasios:2008}.


==> cutoff.tex <==
There are two types of cutoffs out there: EBL and intrinsic. We know from FERMI that we have measured 100 GeV photons in the observing frame, so there is a class of GRBs with high enough bulk lorentz factors that
you can 100 GeV photons can escape. So we know pair production can be above that. How far above it, we don't quite know because the models of intrinsic cutoffs are quite uncertain. Do the example of using a 3 GeV
photon in 2-zone model at Gamma_minimum and then try inputting the upper limit for the same burst and show that at 1 TeV. Cutoffs above 500 GeV aren't really relevent because if you look at redshift = 0.5, only 10%
of photons at 500 GeV remain. EBL effectively accounts for cutoff at any reasonable redshift. That means the range we care about is the 100 - 500 GeV. Try taking a look at a cutoff at 250 GeV. In this case, we're less sensitive but the optimized parameters remain roughly the same. A more extreme case of 150 GeV shows... what?


==> cutrates.tex <==
\cite{GILMORE2012}
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{|c|c|}\hline
Selection & Passing Rate \\
\hline
All Events & 23.6 kHz\\
nHit $\ge$ 70 & 6.6 kHz \\
Zenith Spatial Bin & 7.7 Hz \\
Gamma-Hadron Cut & 0.9 Hz \\ \hline
\end{tabular}

\vspace{2cm}

\begin{tabular}{|l|l|c|}\hline
$\,\,$Cutoff & Short GRBs/year & Long GRBs/year \\
\hline
NA & $\quad\quad\,\,$ 1.4 & 0.25\\
500 GeV & $\quad\quad\,\,$ 1.3 & 0.22\\
400 GeV & $\quad\quad\,\,$ 1.2 & 0.20\\
300 GeV & $\quad\quad\,\,$ 0.97 & 0.15\\
200 GeV & $\quad\quad\,\,$ 0.54 & 0.08\\
150 GeV & $\quad\quad\,\,$ 0.27 & 0.04\\
100 GeV & $\quad\quad\,\,$ 0.07 & 0.01\\ \hline
\end{tabular}

\vspace{2cm}

\renewcommand{\arraystretch}{0.5}
\begin{table}[ht!]
\begin{center}
\begin{tabular}{|c|c|c|c|c|} \hline
  Duration  & Pre-Trial   & Effective      & Effective       & Post-Trial \\
  (seconds) & Probability & Spatial Trials & Temporal Trials & Probability \\ \hline
  0.20  & 3.91$\times$10$^{-14}$ & 1.37$\times$10$^4$ & 1.15$\times$10$^9$ & 0.46 \\
  1.00  & 8.97$\times$10$^{-15}$ & 3.54$\times$10$^4$ & 2.25$\times$10$^8$ & 0.07 \\
  10.00 & 2.51$\times$10$^{-13}$ & 1.06$\times$10$^5$ & 2.36$\times$10$^7$ & 0.47 \\ \hline
\end{tabular}
\caption{Best candidate obtained in each search duration. These candidates have significant
         pre-trial probabilities but are consistent with background after accouting for
         trials. Effective spatial and temporal trials are calculated according to the methods
         outlined in Chapter \ref{ch:method}. We apply an additional trial factor of 3 to 
         account for using three different time windows.}
\label{tab:besties}
\end{center}
\end{table}
\renewcommand{\arraystretch}{1.0}

\vspace{2cm}


\renewcommand{\arraystretch}{0.75}
\begin{table}[ht!]
\begin{center}
\begin{tabular}{|l|c|} \hline
 \multicolumn{2}{|c|}{1 Second Candidate} \\ \hline
 Date & 2015/05/30 \\
 Trigger Time & 08:20:59.67 UTC \\
 Duration & 1.0 second \\
 Obs. Counts & 9 \\
 Bkg. Counts & 0.115 \\
 $P_{pre}$ ($P_{post}$) & 8.97$\times10^{-15}$ (0.19) \\
 Right Ascension & 292.83$^\circ$ (J2000) \\
 Declination & -17.53$^\circ$ (J2000) \\
 Zenith & 40.48$^\circ$ \\ \hline
\end{tabular}
\caption{Details of the overall best candidate from all three searches.
         This candidate was found in the 1 second sliding time window.}
\label{tab:1seccand}
\end{center}
\end{table}
\renewcommand{\arraystretch}{1.0}



==> fliptable.tex <==
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{|c|c|c|c|}\hline
S & R & Q & \={Q} \\
\hline
1 & 0 & 1 & 0 \\
0 & 1 & 0 & 1 \\
0 & 0 & Latch & Latch \\
1 & 1 & 0 & 0 \\
\hline
\end{tabular}


==> logit <==
pdflatex thesis
This is pdfTeX, Version 3.14159265-2.6-1.40.16 (TeX Live 2015) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./thesis.tex
LaTeX2e <2015/01/01>
Babel <3.9l> and hyphenation patterns for 79 languages loaded.
(./thesis.cls
Document Class: thesis 2006/04/26 v0.1
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/size12.clo))
(./styles/titlesec.sty

LaTeX Warning: You have requested package `styles/titlesec',
               but the package provides `titlesec'.

) (/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/graphics.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/pdftex-def/pdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/lscape.sty)
(./styles/indentfirst.sty

LaTeX Warning: You have requested package `styles/indentfirst',
               but the package provides `indentfirst'.

) (./styles/latexsym.sty

LaTeX Warning: You have requested package `styles/latexsym',
               but the package provides `latexsym'.

) (./styles/multirow.sty) (./styles/tabls.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(./styles/slashbox.sty
slashbox style by K.Yasuoka, May 1993.
) (/usr/local/texlive/2015/texmf-dist/tex/latex/tools/longtable.sty)
(./styles/supertabular.sty

LaTeX Warning: You have requested package `styles/supertabular',
               but the package provides `supertabular'.

) (/usr/local/texlive/2015/texmf-dist/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/local/texlive/2015/texmf-dist/tex/latex/subfigure/subfigure.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2015/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/url/url.sty))

Package hyperref Message: Driver: hpdftex.

(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/lineno/lineno.sty) (./thesis.aux
(./Abstract.aux) (./Titlepage.aux) (./Copyright.aux) (./Abbreviations.aux)
(./GRBs.aux) (./Showers.aux))
(/usr/local/texlive/2015/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/color.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./thesis.out) (./thesis.out) (./Abstract.tex
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/ulasy.fd)) [1{/usr/local/tex
live/2015/texmf-var/fonts/map/pdftex/updmap/pdftex.map}] [2] (./Titlepage.tex)
[3] (./Copyright.tex
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/omscmr.fd)) [4]
(./thesis.toc) [2] (./thesis.lof) [3] (./Abbreviations.tex) [4] (./GRBs.tex
Chapter 1.

LaTeX Warning: Citation `Berger:2013jza' on page 1 undefined on input line 19.


LaTeX Warning: Citation `Meszaros:2006rc' on page 1 undefined on input line 25.



LaTeX Warning: Citation `Piran:1999kx' on page 1 undefined on input line 25.

pdfTeX warning (ext4): destination with the same identifier (name{page.1}) has 
been already used, duplicate ignored
<to be read again> 
                   \relax 
l.26 
      [1]

LaTeX Warning: Reference `ch:hawcobs' on page 2 undefined on input line 45.


LaTeX Warning: Reference `ch:Reco' on page 2 undefined on input line 45.


LaTeX Warning: Reference `ch:method' on page 2 undefined on input line 46.


LaTeX Warning: Reference `ch:sens' on page 2 undefined on input line 47.


LaTeX Warning: Reference `ch:results' on page 2 undefined on input line 47.

pdfTeX warning (ext4): destination with the same identifier (name{page.2}) has 
been already used, duplicate ignored
<to be read again> 
                   \relax 
l.49 
      [2]pdfTeX warning (ext4): destination with the same identifier (name{page
.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.73 \newpage
              [3]

LaTeX Warning: Citation `Gehrels:2009qy' on page 4 undefined on input line 81.


LaTeX Warning: Citation `Kleb:1973' on page 4 undefined on input line 82.

pdfTeX warning (ext4): destination with the same identifier (name{page.4}) has 
been already used, duplicate ignored
<to be read again> 
                   \relax 
l.88 \newpage
              [4]

LaTeX Warning: Citation `CGRO:1991' on page 5 undefined on input line 94.


LaTeX Warning: Citation `BATSE:1999' on page 5 undefined on input line 95.


LaTeX Warning: Citation `Gehrels:2009qy' on page 5 undefined on input line 97.

[5] <figures/batse_t90.png, id=130, 931.48pt x 692.5875pt>
<use figures/batse_t90.png>

LaTeX Warning: Citation `Mallozzi:2014a' on page 6 undefined on input line 114.



LaTeX Warning: Citation `Mallozzi:2014a' on page 6 undefined on input line 114.


[6 <./figures/batse_t90.png>]
<figures/batse_panel.png, id=138, 923.45pt x 911.405pt>
<use figures/batse_panel.png>

LaTeX Warning: Citation `Mallozzi:2014b' on page 7 undefined on input line 127.



LaTeX Warning: Citation `Mallozzi:2014b' on page 7 undefined on input line 127.


[7 <./figures/batse_panel.png>]

LaTeX Warning: Citation `Kaneko:2006' on page 8 undefined on input line 147.


LaTeX Warning: Citation `Gruber:2014' on page 8 undefined on input line 149.

[8] <figures/bandfuncfig.pdf, id=158, 612.09195pt x 615.50294pt>
<use figures/bandfuncfig.pdf>

LaTeX Warning: Citation `Briggs:1999' on page 9 undefined on input line 160.


LaTeX Warning: Citation `Briggs:1999' on page 9 undefined on input line 160.

[9 <./figures/bandfuncfig.pdf>]

LaTeX Warning: Citation `Gehrels:2009qy' on page 10 undefined on input line 169
.

<figures/batse_spatial.png, id=175, 980.66376pt x 706.64pt>
<use figures/batse_spatial.png>

LaTeX Warning: Citation `Briggs:2014a' on page 10 undefined on input line 177.

[10 <./figures/batse_spatial.png>]

LaTeX Warning: Citation `Bloom:2001' on page 11 undefined on input line 187.


LaTeX Warning: Citation `Ruderman:1975' on page 11 undefined on input line 195.


[11] <figures/jetbreak.png, id=188, 619.31375pt x 478.78876pt>
<use figures/jetbreak.png>

LaTeX Warning: Citation `kumar:2000' on page 12 undefined on input line 209.


LaTeX Warning: Citation `kumar:2000' on page 12 undefined on input line 209.


LaTeX Warning: Citation `Frail:2001' on page 12 undefined on input line 216.


LaTeX Warning: Citation `Woosley:1999' on page 12 undefined on input line 218.


LaTeX Warning: Citation `Woosley:2006' on page 12 undefined on input line 220.


LaTeX Warning: Citation `Gehrels:2004' on page 12 undefined on input line 226.


LaTeX Warning: Citation `Castro:2005' on page 12 undefined on input line 227.

[12 <./figures/jetbreak.png>]

LaTeX Warning: Citation `Perley:2016' on page 13 undefined on input line 233.


LaTeX Warning: Citation `Berger:2013jza' on page 13 undefined on input line 236
.

[13] <figures/redshift.png, id=202, 1025.8325pt x 832.10875pt>
<use figures/redshift.png>

LaTeX Warning: Citation `Berger:2013jza' on page 14 undefined on input line 247
.


LaTeX Warning: Citation `Berger:2013jza' on page 14 undefined on input line 247
.

[14 <./figures/redshift.png>]

LaTeX Warning: Citation `Meegan:2009' on page 15 undefined on input line 259.


LaTeX Warning: Citation `Atwood:2009ez' on page 15 undefined on input line 259.



LaTeX Warning: Citation `Abdo:2009' on page 15 undefined on input line 266.


LaTeX Warning: Citation `Ackermann:2010' on page 15 undefined on input line 268
.


LaTeX Warning: Citation `Ackermann:2013a' on page 15 undefined on input line 27
1.

[15] <figures/fluenceratio.png, id=213, 706.64pt x 689.57625pt>
<use figures/fluenceratio.png>

LaTeX Warning: Citation `Ackermann:2013a' on page 16 undefined on input line 28
9.


LaTeX Warning: Citation `Ackermann:2013a' on page 16 undefined on input line 28
9.


LaTeX Warning: Citation `Zhu:2013ufa' on page 16 undefined on input line 300.

[16 <./figures/fluenceratio.png>] [17]
<figures/fermicutoff.png, id=226, 960.58875pt x 728.7225pt>
<use figures/fermicutoff.png>

LaTeX Warning: Citation `Bregeon:2011bu' on page 18 undefined on input line 334
.


LaTeX Warning: Citation `Bregeon:2011bu' on page 18 undefined on input line 334
.

[18 <./figures/fermicutoff.png>]

LaTeX Warning: Citation `VERITAS:2013' on page 19 undefined on input line 395.


LaTeX Warning: Citation `HESS:2005' on page 19 undefined on input line 395.


LaTeX Warning: Citation `MAGIC:2016' on page 19 undefined on input line 395.


LaTeX Warning: Citation `Abeysekara:2013tza' on page 19 undefined on input line
 395.

[19] <figures/hess_scheme.jpg, id=239, 413.545pt x 385.44pt>
<use figures/hess_scheme.jpg>
<figures/wct.jpg, id=240, 602.25pt x 615.29875pt> <use figures/wct.jpg>

LaTeX Warning: Citation `MAGIC:2009' on page 20 undefined on input line 427.


LaTeX Warning: Citation `HESS:2009' on page 20 undefined on input line 427.


LaTeX Warning: Citation `VERITAS:2011' on page 20 undefined on input line 427.


LaTeX Warning: Citation `VERITAS:2014' on page 20 undefined on input line 431.

[20 <./figures/hess_scheme.jpg> <./figures/wct.jpg>]

LaTeX Warning: Citation `Atkins:2000' on page 21 undefined on input line 443.


LaTeX Warning: Citation `Vlasios:2008' on page 21 undefined on input line 448.

[21] [22] <figures/EffArea.png, id=261, 734.9859pt x 445.9059pt>
<use figures/EffArea.png> [23 <./figures/EffArea.png>]

LaTeX Warning: Citation `Meszaros:2006rc' on page 24 undefined on input line 51
4.


LaTeX Warning: Citation `Piran:1999kx' on page 24 undefined on input line 514.


LaTeX Warning: Citation `Gehrels:2009qy' on page 24 undefined on input line 519
.


LaTeX Warning: Citation `Lloyd:2000' on page 24 undefined on input line 522.


LaTeX Warning: Citation `Preece:1998' on page 24 undefined on input line 523.

[24] <figures/fireballmodel.png, id=275, 1154.3125pt x 899.36pt>
<use figures/fireballmodel.png>

LaTeX Warning: Citation `Gehrels:2002' on page 25 undefined on input line 535.


LaTeX Warning: Citation `Gehrels:2002' on page 25 undefined on input line 535.


LaTeX Warning: Citation `Sari:1998' on page 25 undefined on input line 542.


LaTeX Warning: Citation `Mezaros:2006' on page 25 undefined on input line 544.


LaTeX Warning: Citation `Gehrels:2009qy' on page 25 undefined on input line 546
.


LaTeX Warning: Citation `Zhu:2013ufa' on page 25 undefined on input line 551.


LaTeX Warning: Citation `Beloborodov:2014' on page 25 undefined on input line 5
55.


LaTeX Warning: Citation `Gehrels:2013' on page 25 undefined on input line 556.

[25 <./figures/fireballmodel.png>] [26] [27]

LaTeX Warning: Citation `Ruderman:1975' on page 28 undefined on input line 657.



LaTeX Warning: Citation `Berger:2013jza' on page 28 undefined on input line 659
.

[28]

LaTeX Warning: Reference `appendixC' on page 29 undefined on input line 672.


LaTeX Warning: Citation `Racusin:2011' on page 29 undefined on input line 677.


LaTeX Warning: Citation `Maselli:2013uza' on page 29 undefined on input line 67
7.


LaTeX Warning: Citation `ZHao:2011' on page 29 undefined on input line 680.


LaTeX Warning: Citation `Gehrels:2013' on page 29 undefined on input line 686.

[29]

LaTeX Warning: Citation `Gruber:2014' on page 30 undefined on input line 697.


LaTeX Warning: Citation `Gruber:2014' on page 30 undefined on input line 697.

[30] <figures/short_grb_cutoff.png, id=316, 800.9925pt x 677.53125pt>
<use figures/short_grb_cutoff.png> [31 <./figures/short_grb_cutoff.png>]

LaTeX Warning: Reference `ch:sens' on page 32 undefined on input line 730.


LaTeX Warning: Citation `GILMORE2012' on page 32 undefined on input line 734.


LaTeX Warning: Citation `Dwek:2013' on page 32 undefined on input line 740.


LaTeX Warning: Citation `GILMORE2012' on page 32 undefined on input line 740.


LaTeX Warning: Citation `Dominguez:2011' on page 32 undefined on input line 740
.

[32] <figures/ebl_flux.png, id=331, 1090.0725pt x 921.4425pt>
<use figures/ebl_flux.png>

LaTeX Warning: Citation `GILMORE2012' on page 33 undefined on input line 747.


LaTeX Warning: Citation `GILMORE2012' on page 33 undefined on input line 747.


LaTeX Warning: Citation `Dominguez:2011' on page 33 undefined on input line 754
.


LaTeX Warning: Citation `GILMORE2012' on page 33 undefined on input line 757.

[33 <./figures/ebl_flux.png>]
<figures/gilmore_2012_EBL_atten.png, id=340, 667.49374pt x 649.42625pt>
<use figures/gilmore_2012_EBL_atten.png>

LaTeX Warning: Citation `GILMORE2012' on page 34 undefined on input line 769.


LaTeX Warning: Citation `GILMORE2012' on page 34 undefined on input line 769.

[34 <./figures/gilmore_2012_EBL_atten.png>]

LaTeX Warning: Citation `Taboada:2013uza' on page 35 undefined on input line 80
3.


LaTeX Warning: Reference `sec:senswtrials' on page 35 undefined on input line 8
06.


LaTeX Warning: Citation `Bhat:2016' on page 35 undefined on input line 808.

[35]) [36] (./Showers.tex
Chapter 2.

LaTeX Warning: Citation `Ptuskin:2012' on page 37 undefined on input line 6.


LaTeX Warning: Citation `Abeysekara:2014a' on page 37 undefined on input line 7
.


LaTeX Warning: Reference `sec:crshower' on page 37 undefined on input line 16.


LaTeX Warning: Reference `sec:showplan' on page 37 undefined on input line 18.


LaTeX Warning: Reference `sec:diffthatthing' on page 37 undefined on input line
 19.


LaTeX Warning: Reference `ch:Reco' on page 37 undefined on input line 20.

[37] [38]

LaTeX Warning: Reference `sec:crshower' on page 39 undefined on input line 39.


Overfull \hbox (12.82234pt too wide) in paragraph at lines 36--41
\OT1/cmr/m/n/12 The elec-tron and positron pair sub-se-quently gen-er-ate more 
pho-tons via Bremsstrahlung

LaTeX Warning: Citation `Heitler:1954' on page 39 undefined on input line 54.

[39] <figures/gamma_shower_model.png, id=372, 650.43pt x 502.87875pt>
<use figures/gamma_shower_model.png>

LaTeX Warning: Citation `Matthews:2005' on page 40 undefined on input line 74.


LaTeX Warning: Citation `Matthews:2005' on page 40 undefined on input line 74.

[40]

LaTeX Warning: Reference `fig:gamma_prof' on page 41 undefined on input line 82
.

[41 <./figures/gamma_shower_model.png>]
<figures/gamma_shower_profile.png, id=386, 1200.485pt x 875.27pt>
<use figures/gamma_shower_profile.png>

LaTeX Warning: Citation `Grieder:2010' on page 42 undefined on input line 100.


LaTeX Warning: Citation `Grieder:2010' on page 42 undefined on input line 100.

[42 <./figures/gamma_shower_profile.png>]

LaTeX Warning: Citation `Kampert:2012' on page 43 undefined on input line 112.


LaTeX Warning: Citation `PDG' on page 43 undefined on input line 113.


LaTeX Warning: Citation `Kampert:2012' on page 43 undefined on input line 122.


LaTeX Warning: Citation `Sommers:2004' on page 43 undefined on input line 125.


LaTeX Warning: Citation `Grieder:2010' on page 43 undefined on input line 127.

[43]

LaTeX Warning: Citation `Grieder:2010' on page 44 undefined on input line 137.


LaTeX Warning: Reference `fig:cascade' on page 44 undefined on input line 137.

<figures/eas_diagram.png, id=399, 410.53375pt x 658.46pt>
<use figures/eas_diagram.png>

LaTeX Warning: Citation `Grieder:2010' on page 44 undefined on input line 142.


LaTeX Warning: Citation `Grieder:2010' on page 44 undefined on input line 142.

[44]

LaTeX Warning: Reference `fig:proton_prof' on page 45 undefined on input line 1
50.


LaTeX Warning: Reference `fig:proton_number' on page 45 undefined on input line
 154.


LaTeX Warning: Reference `fig:proton_prof' on page 45 undefined on input line 1
57.

[45 <./figures/eas_diagram.png>]

LaTeX Warning: Reference `fig:proton_prof' on page 46 undefined on input line 1
60.


LaTeX Warning: Reference `eq:proton_react' on page 46 undefined on input line 1
62.


LaTeX Warning: Citation `Kampert:2012' on page 46 undefined on input line 162.

[46] <figures/proton_shower_profile.png, id=415, 1200.485pt x 875.27pt>
<use figures/proton_shower_profile.png>

LaTeX Warning: Citation `Grieder:2010' on page 47 undefined on input line 176.


LaTeX Warning: Citation `Grieder:2010' on page 47 undefined on input line 176.

[47 <./figures/proton_shower_profile.png>]
<figures/proton_particle_number.png, id=421, 634.37pt x 718.685pt>
<use figures/proton_particle_number.png>

LaTeX Warning: Citation `Grieder:2010' on page 48 undefined on input line 187.


LaTeX Warning: Citation `Grieder:2010' on page 48 undefined on input line 187.

[48 <./figures/proton_particle_number.png>]

LaTeX Warning: Reference `fig:shower_timing' on page 49 undefined on input line
 198.


LaTeX Warning: Reference `ch:Reco' on page 49 undefined on input line 205.


LaTeX Warning: Reference `fig:shower_timing' on page 49 undefined on input line
 207.


LaTeX Warning: Citation `Grieder:2010' on page 49 undefined on input line 209.


LaTeX Warning: Citation `Atkins:2000' on page 49 undefined on input line 213.

[49] <figures/shower_timing.png, id=434, 562.1pt x 628.3475pt>
<use figures/shower_timing.png>

LaTeX Warning: Citation `Grieder:2010' on page 50 undefined on input line 221.


LaTeX Warning: Citation `Grieder:2010' on page 50 undefined on input line 221.

[50 <./figures/shower_timing.png>]

LaTeX Warning: Reference `fig:spreadthatstuffout' on page 51 undefined on input
 line 237.


LaTeX Warning: Reference `fig:spreadthatstuffout' on page 51 undefined on input
 line 239.


LaTeX Warning: Reference `ch:Reco' on page 51 undefined on input line 240.

<figures/side_shower.png, id=441, 608.2725pt x 744.7825pt>
<use figures/side_shower.png>

LaTeX Warning: Citation `Grieder:2010' on page 51 undefined on input line 254.


LaTeX Warning: Citation `Grieder:2010' on page 51 undefined on input line 254.

) [51] [52 <./figures/side_shower.png>] (./HAWC.tex
Chapter 3.

LaTeX Warning: Citation `ICRC2013' on page 53 undefined on input line 9.

[53] <figures/HAWC_overview.jpeg, id=459, 1080.035pt x 725.71124pt>
<use figures/HAWC_overview.jpeg> [54 <./figures/HAWC_overview.jpeg>]

LaTeX Warning: Reference `tanky' on page 55 undefined on input line 39.

[55] <figures/HAWC_tank.png, id=472, 839.135pt x 688.5725pt>
<use figures/HAWC_tank.png>
<figures/HAWC_bladder.png, id=473, 182.1204pt x 168.63pt>
<use figures/HAWC_bladder.png> [56 <./figures/HAWC_tank.png> <./figures/HAWC_bl
adder.png>]

LaTeX Warning: Reference `fig:pmt_diagram' on page 57 undefined on input line 7
4.

[57] <figures/regularpulse.png, id=486, 520.94624pt x 706.64pt>
<use figures/regularpulse.png>
<figures/HAWC_pmt.png, id=487, 171.039pt x 227.8914pt>
<use figures/HAWC_pmt.png> [58 <./figures/regularpulse.png> <./figures/HAWC_pmt
.png>]

LaTeX Warning: Citation `DCHOOZ2011' on page 59 undefined on input line 107.


LaTeX Warning: Reference `fig:single_pe_charge' on page 59 undefined on input l
ine 108.

[59] <figures/single_pe_charge.jpeg, id=501, 990.70125pt x 736.7525pt>
<use figures/single_pe_charge.jpeg> [60 <./figures/single_pe_charge.jpeg>]

LaTeX Warning: Reference `fig:QE_CE' on page 61 undefined on input line 135.


LaTeX Warning: Reference `fig:QE_CE' on page 61 undefined on input line 137.

[61] <figures/r5912_quantum_efficiency.png, id=512, 610.28pt x 664.4825pt>
<use figures/r5912_quantum_efficiency.png>
<figures/r7081_HQE_quantum_efficiency.png, id=513, 546.04pt x 696.6025pt>
<use figures/r7081_HQE_quantum_efficiency.png> [62 <./figures/r5912_quantum_eff
iciency.png> <./figures/r7081_HQE_quantum_efficiency.png>]

LaTeX Warning: Reference `fig:DAQ_block_diagram' on page 63 undefined on input 
line 162.


LaTeX Warning: Reference `fig:DAQ_block_diagram' on page 63 undefined on input 
line 170.

[63] <figures/signal_overview.png, id=528, 914.41624pt x 311.1625pt>
<use figures/signal_overview.png> [64 <./figures/signal_overview.png>]

LaTeX Warning: Reference `fig:DAQ_block_diagram' on page 65 undefined on input 
line 193.


LaTeX Warning: Reference `fig:coax_diagram' on page 65 undefined on input line 
216.

[65] <figures/coax_diagram.png, id=540, 484.81125pt x 483.8075pt>
<use figures/coax_diagram.png>

LaTeX Warning: Citation `HAYT' on page 66 undefined on input line 235.


LaTeX Warning: Reference `tab:coaxcab_hf' on page 66 undefined on input line 23
5.


LaTeX Warning: Reference `fig:coax_diagram' on page 66 undefined on input line 
236.

[66 <./figures/coax_diagram.png>]

LaTeX Warning: Reference `fig:coax_diagram' on page 67 undefined on input line 
253.


LaTeX Warning: Citation `HAYT' on page 67 undefined on input line 253.


LaTeX Warning: Reference `fig:coax_diagram' on page 67 undefined on input line 
253.


LaTeX Warning: Citation `HAYT' on page 67 undefined on input line 253.

<figures/circuit.png, id=548, 860.21375pt x 442.65375pt>
<use figures/circuit.png>

LaTeX Warning: Reference `fig:coax_diagram' on page 67 undefined on input line 
264.


LaTeX Warning: Reference `fig:coax_diagram' on page 67 undefined on input line 
264.

[67 <./figures/circuit.png>]

LaTeX Warning: Reference `tab:coaxcab_hf' on page 68 undefined on input line 27
0.


LaTeX Warning: Reference `fig:coax_circuit' on page 68 undefined on input line 
271.


LaTeX Warning: Reference `appendixB' on page 68 undefined on input line 284.

[68]

LaTeX Warning: Reference `eq:k_w_K_intext' on page 69 undefined on input line 3
05.


LaTeX Warning: Reference `fig:cable_prop' on page 69 undefined on input line 30
7.


LaTeX Warning: Reference `appendixB' on page 69 undefined on input line 312.


LaTeX Warning: Reference `eq:cable_prop_speed' on page 69 undefined on input li
ne 315.

[69] <figures/comp_cable.png, id=570, 1200.485pt x 875.27pt>
<use figures/comp_cable.png>

LaTeX Warning: Reference `eq:k_w_K_intext' on page 70 undefined on input line 3
21.


LaTeX Warning: Reference `eq:k_w_K_intext' on page 70 undefined on input line 3
21.

[70 <./figures/comp_cable.png>]
<figures/analog_circuit.png, id=576, 1186.4325pt x 665.48625pt>
<use figures/analog_circuit.png>

LaTeX Warning: Reference `fig:analog_circuit' on page 71 undefined on input lin
e 347.

[71 <./figures/analog_circuit.png>] [72]

LaTeX Warning: Reference `tab:analog_param' on page 73 undefined on input line 
377.


LaTeX Warning: Reference `fig:cable_prop' on page 73 undefined on input line 39
7.


LaTeX Warning: Reference `fig:4edge_analog' on page 73 undefined on input line 
400.


LaTeX Warning: Reference `fig:cable_prop' on page 73 undefined on input line 40
1.

[73]

LaTeX Warning: Reference `fig:4edge_analog' on page 74 undefined on input line 
409.


LaTeX Warning: Reference `fig:2edge_analog' on page 74 undefined on input line 
409.

[74] <figures/AnalogFEB_4edge.png, id=604, 1202.4925pt x 878.28125pt>
<use figures/AnalogFEB_4edge.png>

LaTeX Warning: Reference `fig:cable_prop' on page 75 undefined on input line 42
0.


LaTeX Warning: Reference `eq:amp_response' on page 75 undefined on input line 4
20.


LaTeX Warning: Reference `fig:cable_prop' on page 75 undefined on input line 42
0.


LaTeX Warning: Reference `eq:amp_response' on page 75 undefined on input line 4
20.

[75 <./figures/AnalogFEB_4edge.png>]
<figures/AnalogFEB_2edge.png, id=610, 1202.4925pt x 878.28125pt>
<use figures/AnalogFEB_2edge.png>

LaTeX Warning: Reference `eq:amp_response' on page 76 undefined on input line 4
33.


LaTeX Warning: Reference `eq:amp_response' on page 76 undefined on input line 4
33.

[76 <./figures/AnalogFEB_2edge.png>]
<figures/digital_logic.png, id=616, 968.61874pt x 628.3475pt>
<use figures/digital_logic.png>

LaTeX Warning: Reference `fig:digital_logic' on page 77 undefined on input line
 456.

[77 <./figures/digital_logic.png>]

LaTeX Warning: Reference `fig:latch_circuit' on page 78 undefined on input line
 461.


LaTeX Warning: Reference `fig:flip_flop' on page 78 undefined on input line 464
.

<figures/latch_circuit.png, id=624, 894.34125pt x 481.8pt>
<use figures/latch_circuit.png> [78 <./figures/latch_circuit.png>]
<figures/flip_flop_logic.png, id=632, 352.31625pt x 269.005pt>
<use figures/flip_flop_logic.png>
<figures/logic_table.png, id=633, 666.49pt x 470.75874pt>
<use figures/logic_table.png>

LaTeX Warning: Reference `fig:latch_resp' on page 79 undefined on input line 49
2.

[79 <./figures/flip_flop_logic.png> <./figures/logic_table.png>]
<figures/flip_flop_20ns.png, id=643, 700.6175pt x 476.78125pt>
<use figures/flip_flop_20ns.png> [80 <./figures/flip_flop_20ns.png>]
<figures/one-shot_width_vs_R.png, id=649, 901.3675pt x 777.90625pt>
<use figures/one-shot_width_vs_R.png>

LaTeX Warning: Reference `fig:one_shot_v_r' on page 81 undefined on input line 
521.

[81 <./figures/one-shot_width_vs_R.png>]

LaTeX Warning: Reference `fig:delay_circuit' on page 82 undefined on input line
 537.

[82] <figures/delay_circuit.png, id=659, 697.60625pt x 202.7575pt>
<use figures/delay_circuit.png>

LaTeX Warning: Reference `tab:risetimes' on page 83 undefined on input line 569
.

[83 <./figures/delay_circuit.png>]

LaTeX Warning: Reference `fig:digital_logic' on page 84 undefined on input line
 577.


LaTeX Warning: Reference `fig:digital_logic' on page 84 undefined on input line
 580.


LaTeX Warning: Reference `fig:fouredge' on page 84 undefined on input line 582.



LaTeX Warning: Reference `fig:4edge_analog' on page 84 undefined on input line 
582.


LaTeX Warning: Reference `tab:timingpar' on page 84 undefined on input line 589
.

[84] <figures/DigitalFEB_4edge.png, id=672, 1202.4925pt x 426.59375pt>
<use figures/DigitalFEB_4edge.png>
Overfull \hbox (43.36244pt too wide) in paragraph at lines 595--596
 [] 

LaTeX Warning: Reference `fig:4edge_analog' on page 85 undefined on input line 
601.


LaTeX Warning: Reference `fig:digital_logic' on page 85 undefined on input line
 601.


LaTeX Warning: Reference `fig:4edge_analog' on page 85 undefined on input line 
601.


LaTeX Warning: Reference `fig:digital_logic' on page 85 undefined on input line
 601.

[85 <./figures/DigitalFEB_4edge.png>]

LaTeX Warning: Reference `fig:fouredge' on page 86 undefined on input line 623.



LaTeX Warning: Reference `fig:4edge_analog' on page 86 undefined on input line 
623.


LaTeX Warning: Reference `fig:fouredge' on page 86 undefined on input line 623.



LaTeX Warning: Reference `fig:4edge_analog' on page 86 undefined on input line 
623.

[86]

LaTeX Warning: Reference `fig:2edge_analog' on page 87 undefined on input line 
630.


LaTeX Warning: Reference `fig:twoedge_dig' on page 87 undefined on input line 6
34.

<figures/DigitalFEB_2edge.png, id=683, 1202.4925pt x 426.59375pt>
<use figures/DigitalFEB_2edge.png>
Overfull \hbox (43.36244pt too wide) in paragraph at lines 638--639
 [] 

LaTeX Warning: Reference `fig:2edge_analog' on page 87 undefined on input line 
643.


LaTeX Warning: Reference `fig:2edge_analog' on page 87 undefined on input line 
643.

[87 <./figures/DigitalFEB_2edge.png>]

LaTeX Warning: Reference `fig:fouredge' on page 88 undefined on input line 652.



LaTeX Warning: Reference `fig:twoedge_dig' on page 88 undefined on input line 6
52.


LaTeX Warning: Reference `sec:DFEB' on page 88 undefined on input line 657.


LaTeX Warning: Reference `fig:edgeevent' on page 88 undefined on input line 663
.


LaTeX Warning: Reference `ch:method' on page 88 undefined on input line 665.


LaTeX Warning: Reference `ch:results' on page 88 undefined on input line 665.

[88]

LaTeX Warning: Reference `sec:trigger' on page 89 undefined on input line 671.

[89] <figures/early_TDC_event.png, id=698, 855.195pt x 610.28pt>
<use figures/early_TDC_event.png> [90 <./figures/early_TDC_event.png>]

LaTeX Warning: Reference `sec:TDCs' on page 91 undefined on input line 696.


LaTeX Warning: Reference `fig:onlinechain' on page 91 undefined on input line 7
03.


LaTeX Warning: Reference `sec:TDCs' on page 91 undefined on input line 704.


LaTeX Warning: Reference `fig:airshowtrig' on page 91 undefined on input line 7
07.


LaTeX Warning: Reference `ch:Reco' on page 91 undefined on input line 708.

[91] <figures/online_reco_chain.png, id=711, 1038.88126pt x 591.20876pt>
<use figures/online_reco_chain.png> [92 <./figures/online_reco_chain.png>]
<figures/timediagram.png, id=718, 1013.7875pt x 633.36626pt>
<use figures/timediagram.png>

LaTeX Warning: Reference `sec:edges' on page 93 undefined on input line 748.


LaTeX Warning: Reference `sec:edges' on page 93 undefined on input line 748.

[93 <./figures/timediagram.png>]

LaTeX Warning: Reference `fig:latency' on page 94 undefined on input line 761.

[94] <figures/OnlineLatencyBigBins.png, id=729, 922.44624pt x 617.30624pt>
<use figures/OnlineLatencyBigBins.png>

LaTeX Warning: Reference `fig:onlinechain' on page 95 undefined on input line 7
74.


LaTeX Warning: Reference `fig:onlinechain' on page 95 undefined on input line 7
74.

[95 <./figures/OnlineLatencyBigBins.png>]

LaTeX Warning: Reference `caloverview' on page 96 undefined on input line 789.


LaTeX Warning: Reference `chargecurve' on page 96 undefined on input line 790.


LaTeX Warning: Reference `slewingcurve' on page 96 undefined on input line 800.


[96]
<figures/Calibration_Simplified_Layout.png, id=742, 794.4882pt x 654.2844pt>
<use figures/Calibration_Simplified_Layout.png> [97 <./figures/Calibration_Simp
lified_Layout.png>]
<figures/chargecalib_curves_run5213_H13.png, id=748, 1367.1075pt x 701.62125pt>
<use figures/chargecalib_curves_run5213_H13.png> [98 <./figures/chargecalib_cur
ves_run5213_H13.png>] <figures/H13_slewing.png, id=756, 999.735pt x 774.895pt>
<use figures/H13_slewing.png>

LaTeX Warning: Reference `sec:prepulse' on page 99 undefined on input line 844.



LaTeX Warning: Reference `sec:prepulse' on page 99 undefined on input line 844.


[99 <./figures/H13_slewing.png>]

LaTeX Warning: Citation `Lubsand:2000' on page 100 undefined on input line 854.



LaTeX Warning: Reference `appendixbase' on page 100 undefined on input line 865
.

[100]

LaTeX Warning: Reference `fig:preTENpulse' on page 101 undefined on input line 
873.


LaTeX Warning: Citation `Fleming:2002' on page 101 undefined on input line 875.



LaTeX Warning: Reference `fig:preTENpulse' on page 101 undefined on input line 
877.


LaTeX Warning: Reference `fig:preTENpulse' on page 101 undefined on input line 
878.


LaTeX Warning: Reference `calmeup' on page 101 undefined on input line 878.

[101]

LaTeX Warning: Reference `fig:preTENpulse' on page 102 undefined on input line 
880.


LaTeX Warning: Reference `fig:preEIGHTpulse' on page 102 undefined on input lin
e 888.


LaTeX Warning: Citation `Karn:2013' on page 102 undefined on input line 888.


LaTeX Warning: Reference `fig:preEIGHTpulse' on page 102 undefined on input lin
e 892.


LaTeX Warning: Reference `calmeup' on page 102 undefined on input line 893.

[102] [103] <figures/10inch_lostart.png, id=782, 800.9925pt x 577.15625pt>
<use figures/10inch_lostart.png>
<figures/10inch_histart.png, id=783, 798.985pt x 574.145pt>
<use figures/10inch_histart.png> [104 <./figures/10inch_lostart.png> <./figures
/10inch_histart.png>]
<figures/8inch_lostart.png, id=791, 798.985pt x 574.145pt>
<use figures/8inch_lostart.png>
<figures/8inch_histart.png, id=792, 798.985pt x 574.145pt>
<use figures/8inch_histart.png> [105 <./figures/8inch_lostart.png> <./figures/8
inch_histart.png>]

LaTeX Warning: Citation `Ma:2009' on page 106 undefined on input line 941.


LaTeX Warning: Reference `fig:rateofhits' on page 106 undefined on input line 9
45.

[106] <figures/afterpulsing_rate.png, id=805, 937.5025pt x 669.50125pt>
<use figures/afterpulsing_rate.png> [107 <./figures/afterpulsing_rate.png>]

LaTeX Warning: Reference `sec:prepulse' on page 108 undefined on input line 965
.


LaTeX Warning: Citation `Ma:2009' on page 108 undefined on input line 973.


Overfull \hbox (0.59285pt too wide) in paragraph at lines 970--974
\OT1/cmr/m/n/12 for ion-iza-tion oc-cur-ring a dis-tance $\OML/cmm/m/it/12 s$ \
OT1/cmr/m/n/12 from the pho-to-cath-ode. The af-ter-pulse timescale

LaTeX Warning: Reference `fig:aftthatpulse' on page 108 undefined on input line
 976.


LaTeX Warning: Reference `calmeup' on page 108 undefined on input line 977.

[108]

LaTeX Warning: Reference `fig:aftthatpulse' on page 109 undefined on input line
 987.

[109] <figures/afterpulse_outer.png, id=822, 1200.485pt x 875.27pt>
<use figures/afterpulse_outer.png>
<figures/afterpulse_central.png, id=823, 1200.485pt x 875.27pt>
<use figures/afterpulse_central.png>

LaTeX Warning: Reference `fig:rateofhits' on page 110 undefined on input line 1
008.


LaTeX Warning: Reference `fig:rateofhits' on page 110 undefined on input line 1
008.

[110 <./figures/afterpulse_outer.png> <./figures/afterpulse_central.png>])
(./Reco.tex
Chapter 4.

LaTeX Warning: Reference `ch:hawcobs' on page 111 undefined on input line 5.


LaTeX Warning: Reference `ch:method' on page 111 undefined on input line 13.


LaTeX Warning: Citation `Braun:2016' on page 111 undefined on input line 18.


LaTeX Warning: Reference `ch:results' on page 111 undefined on input line 19.


LaTeX Warning: Reference `ch:method' on page 111 undefined on input line 20.


LaTeX Warning: Reference `sec:edges' on page 111 undefined on input line 20.


LaTeX Warning: Reference `sec:gammahadron' on page 111 undefined on input line 
20.


LaTeX Warning: Reference `sec:performance' on page 111 undefined on input line 
21.

[111]

LaTeX Warning: Reference `ch:hawcobs' on page 112 undefined on input line 33.


LaTeX Warning: Reference `fig:edgestream' on page 112 undefined on input line 3
3.


LaTeX Warning: Reference `sec:gammahadron' on page 112 undefined on input line 
41.

<figures/edgestream.png, id=836, 902.37125pt x 209.78375pt>
<use figures/edgestream.png>

LaTeX Warning: Reference `ch:hawcobs' on page 112 undefined on input line 61.

[112 <./figures/edgestream.png>]

LaTeX Warning: Reference `tab:edgecuts' on page 113 undefined on input line 68.



LaTeX Warning: Reference `fig:measured_tots' on page 113 undefined on input lin
e 71.

[113]

LaTeX Warning: Reference `ch:hawcobs' on page 114 undefined on input line 109.


LaTeX Warning: Reference `ch:hawcobs' on page 114 undefined on input line 109.

[114] <figures/LoTOT.png, id=854, 798.985pt x 574.145pt>
<use figures/LoTOT.png> <figures/HiTOT.png, id=855, 798.985pt x 574.145pt>
<use figures/HiTOT.png> <figures/T01.png, id=856, 798.985pt x 574.145pt>
<use figures/T01.png> <figures/T23.png, id=857, 798.985pt x 574.145pt>
<use figures/T23.png>

LaTeX Warning: Reference `tab:edgecuts' on page 115 undefined on input line 130
.


LaTeX Warning: Reference `tab:edgecuts' on page 115 undefined on input line 130
.

[115 <./figures/LoTOT.png> <./figures/HiTOT.png> <./figures/T01.png> <./figures
/T23.png>]

LaTeX Warning: Citation `Greisen:1960' on page 116 undefined on input line 145.



LaTeX Warning: Reference `fig:coredist' on page 116 undefined on input line 146
.

[116] <figures/SFCF.png, id=873, 710.655pt x 499.8675pt>
<use figures/SFCF.png>

LaTeX Warning: Citation `Braun:2016' on page 117 undefined on input line 161.


LaTeX Warning: Citation `Braun:2016' on page 117 undefined on input line 161.

[117 <./figures/SFCF.png>]

LaTeX Warning: Reference `fig:simshower' on page 118 undefined on input line 16
8.


LaTeX Warning: Reference `fig:realshower' on page 118 undefined on input line 1
68.


LaTeX Warning: Reference `eq:corelikely' on page 118 undefined on input line 18
3.


LaTeX Warning: Citation `Braun:2016' on page 118 undefined on input line 190.

[118] <figures/gamma_sim.png, id=886, 795.97375pt x 533.995pt>
<use figures/gamma_sim.png>
<figures/proton_sim.png, id=887, 801.99625pt x 533.995pt>
<use figures/proton_sim.png>

LaTeX Warning: Reference `sec:compactness' on page 119 undefined on input line 
210.


LaTeX Warning: Reference `sec:compactness' on page 119 undefined on input line 
210.

[119 <./figures/gamma_sim.png> <./figures/proton_sim.png>]
<figures/likely_gamma.png, id=897, 801.99625pt x 539.01375pt>
<use figures/likely_gamma.png>
<figures/likely_hadron.png, id=898, 803.0pt x 542.025pt>
<use figures/likely_hadron.png>
Overfull \hbox (9.47742pt too wide) in paragraph at lines 218--229
[][]     [][] 

LaTeX Warning: Reference `sec:compactness' on page 120 undefined on input line 
229.


LaTeX Warning: Reference `sec:compactness' on page 120 undefined on input line 
229.

[120 <./figures/likely_gamma.png> <./figures/likely_hadron.png>]

LaTeX Warning: Reference `fig:curvecorrdata' on page 121 undefined on input lin
e 242.


LaTeX Warning: Reference `sec:compactness' on page 121 undefined on input line 
244.


LaTeX Warning: Reference `sec:pincness' on page 121 undefined on input line 244
.


LaTeX Warning: Reference `fig:angleres' on page 121 undefined on input line 248
.


LaTeX Warning: Citation `Braun:2016' on page 121 undefined on input line 250.

[121] <figures/curvature_correct.png, id=916, 718.685pt x 548.0475pt>
<use figures/curvature_correct.png>

LaTeX Warning: Citation `Braun:2016' on page 122 undefined on input line 265.


LaTeX Warning: Citation `Braun:2016' on page 122 undefined on input line 265.

[122 <./figures/curvature_correct.png>]
<figures/angle_v_energy.png, id=925, 765.86125pt x 602.25pt>
<use figures/angle_v_energy.png> [123 <./figures/angle_v_energy.png>]

LaTeX Warning: Reference `fig:simshower' on page 124 undefined on input line 30
0.


LaTeX Warning: Reference `fig:realshower' on page 124 undefined on input line 3
00.

[124]

LaTeX Warning: Reference `sec:corefit' on page 125 undefined on input line 318.



LaTeX Warning: Reference `fig:invcompactness' on page 125 undefined on input li
ne 319.


LaTeX Warning: Reference `ch:method' on page 125 undefined on input line 328.


LaTeX Warning: Reference `ch:sens' on page 125 undefined on input line 328.

[125]
<figures/SP-invcompact-demo-20160404.png, id=944, 2849.64626pt x 2269.47874pt>
<use figures/SP-invcompact-demo-20160404.png> [126 <./figures/SP-invcompact-dem
o-20160404.png>]

LaTeX Warning: Reference `fig:pincnessdiag' on page 127 undefined on input line
 368.


LaTeX Warning: Reference `sec:anglefit' on page 127 undefined on input line 372
.


LaTeX Warning: Reference `fig:pincnessmoneyplot' on page 127 undefined on input
 line 378.


LaTeX Warning: Reference `sec:performance' on page 127 undefined on input line 
382.


Overfull \hbox (4.36082pt too wide) in paragraph at lines 375--383
[]\OT1/cmr/m/n/12 The asym-me-tries present in the spa-tial dis-tri-bu-tion of 
shower en-ergy in hadronic
[127] <figures/pinc.png, id=958, 998.73125pt x 662.475pt>
<use figures/pinc.png>

LaTeX Warning: Reference `sec:compactness' on page 128 undefined on input line 
395.


LaTeX Warning: Reference `sec:compactness' on page 128 undefined on input line 
395.

[128 <./figures/pinc.png>]
<figures/SP-pinc-demo-20160404.png, id=965, 2827.56375pt x 2269.47874pt>
<use figures/SP-pinc-demo-20160404.png> [129 <./figures/SP-pinc-demo-20160404.p
ng>]

LaTeX Warning: Citation `Weekes:1989' on page 130 undefined on input line 421.


LaTeX Warning: Citation `Younk:2015' on page 130 undefined on input line 426.


LaTeX Warning: Citation `Abeysekara:2013tza' on page 130 undefined on input lin
e 428.


LaTeX Warning: Reference `fig:dmc' on page 130 undefined on input line 430.


LaTeX Warning: Reference `ch:sens' on page 130 undefined on input line 438.

<figures/Crab_SP_RC0v2.jpg, id=972, 367.3725pt x 412.54124pt>
<use figures/Crab_SP_RC0v2.jpg>
<figures/crab_excess.png, id=973, 730.73pt x 692.5875pt>
<use figures/crab_excess.png>) [130] [131 <./figures/Crab_SP_RC0v2.jpg>]
[132 <./figures/crab_excess.png>] (./Method.tex
Chapter 5.

LaTeX Warning: Reference `sec:senswtrials' on page 133 undefined on input line 
11.

[133]

LaTeX Warning: Reference `sec:senswtrials' on page 134 undefined on input line 
32.


LaTeX Warning: Reference `ch:sens' on page 134 undefined on input line 38.

[134]

LaTeX Warning: Reference `ch:sens' on page 135 undefined on input line 47.


LaTeX Warning: Reference `fig:sigsky' on page 135 undefined on input line 57.

[135]

LaTeX Warning: Reference `fig:sigsky' on page 136 undefined on input line 66.


LaTeX Warning: Reference `sec:bgcalc' on page 136 undefined on input line 71.


LaTeX Warning: Reference `sec:trialscalc' on page 136 undefined on input line 7
1.

[136] <figures/exampleskymap.png, id=1009, 800.9925pt x 577.15625pt>
<use figures/exampleskymap.png> [137 <./figures/exampleskymap.png>]

LaTeX Warning: Reference `fig:timewindowdiag' on page 138 undefined on input li
ne 98.


LaTeX Warning: Citation `Vlasios:2008' on page 138 undefined on input line 102.


[138] <figures/timediagram_two.png, id=1021, 874.26625pt x 570.13pt>
<use figures/timediagram_two.png> [139 <./figures/timediagram_two.png>]

LaTeX Warning: Citation `Fiorino:2015' on page 140 undefined on input line 141.



LaTeX Warning: Reference `fig:backmap' on page 140 undefined on input line 142.



LaTeX Warning: Reference `sec:space' on page 140 undefined on input line 143.

[140] <figures/exbackground.png, id=1034, 798.985pt x 574.145pt>
<use figures/exbackground.png> [141 <./figures/exbackground.png>]

LaTeX Warning: Reference `fig:backmap' on page 142 undefined on input line 164.



LaTeX Warning: Reference `fig:poisson' on page 142 undefined on input line 176.


[142] <figures/poisson_check1.png, id=1047, 800.9925pt x 577.15625pt>
<use figures/poisson_check1.png> [143 <./figures/poisson_check1.png>]

LaTeX Warning: Reference `directint' on page 144 undefined on input line 204.

[144]

LaTeX Warning: Reference `ch:results' on page 145 undefined on input line 222.

[145]

LaTeX Warning: Reference `directint' on page 146 undefined on input line 236.


LaTeX Warning: Reference `cumulpoisson' on page 146 undefined on input line 238
.

[146]

LaTeX Warning: Reference `fig:pdistp2sec' on page 147 undefined on input line 2
56.


LaTeX Warning: Reference `fig:pdist10sec' on page 147 undefined on input line 2
56.


LaTeX Warning: Reference `sec:bgcalc' on page 147 undefined on input line 258.

[147] <figures/backstudy_pgraph_p2sec.png, id=1073, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_p2sec.png>

LaTeX Warning: Reference `eq:obspval' on page 148 undefined on input line 278.


LaTeX Warning: Reference `directint' on page 148 undefined on input line 278.


LaTeX Warning: Reference `eq:obspval' on page 148 undefined on input line 278.


LaTeX Warning: Reference `directint' on page 148 undefined on input line 278.


LaTeX Warning: Float too large for page by 7.41559pt on input line 281.

<figures/backstudy_pgraph_1sec.png, id=1074, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_1sec.png>

LaTeX Warning: Reference `eq:obspval' on page 148 undefined on input line 297.


LaTeX Warning: Reference `directint' on page 148 undefined on input line 297.


LaTeX Warning: Reference `eq:obspval' on page 148 undefined on input line 297.


LaTeX Warning: Reference `directint' on page 148 undefined on input line 297.

<figures/backstudy_pgraph_10sec.png, id=1075, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_10sec.png>

LaTeX Warning: Reference `eq:obspval' on page 148 undefined on input line 316.


LaTeX Warning: Reference `directint' on page 148 undefined on input line 316.


LaTeX Warning: Reference `fig:pdistp2sec' on page 148 undefined on input line 3
16.


LaTeX Warning: Reference `eq:obspval' on page 148 undefined on input line 316.


LaTeX Warning: Reference `directint' on page 148 undefined on input line 316.


LaTeX Warning: Reference `fig:pdistp2sec' on page 148 undefined on input line 3
16.


LaTeX Warning: Float too large for page by 9.7489pt on input line 319.

) [148 <./figures/backstudy_pgraph_p2sec.png>] [149 <./figures/backstudy_pgraph
_1sec.png>] [150 <./figures/backstudy_pgraph_10sec.png>] (./Trials.tex [151]

LaTeX Warning: Reference `eq:cumulativepp' on page 152 undefined on input line 
34.


LaTeX Warning: Reference `eq:twotrialcase' on page 152 undefined on input line 
38.


LaTeX Warning: Citation `Sidak:1967' on page 152 undefined on input line 43.

[152]

LaTeX Warning: Reference `eq:ntrialcase' on page 153 undefined on input line 51
.

[153]

LaTeX Warning: Reference `eq:ntrialcase' on page 154 undefined on input line 66
.


LaTeX Warning: Reference `fig:indeptrials' on page 154 undefined on input line 
77.


LaTeX Warning: Reference `eq:trialthat' on page 154 undefined on input line 80.


[154] <figures/inde_pdist.png, id=1119, 698.61pt x 875.27pt>
<use figures/inde_pdist.png>
<figures/inde_trials.png, id=1120, 698.61pt x 875.27pt>
<use figures/inde_trials.png> [155 <./figures/inde_pdist.png> <./figures/inde_t
rials.png>]

LaTeX Warning: Reference `eq:trialthat' on page 156 undefined on input line 108
.


LaTeX Warning: Reference `sec:indeptrials' on page 156 undefined on input line 
111.


LaTeX Warning: Reference `fig:corrtrials' on page 156 undefined on input line 1
16.


LaTeX Warning: Reference `eq:trialthat' on page 156 undefined on input line 116
.


LaTeX Warning: Reference `fig:indeptrials' on page 156 undefined on input line 
118.

[156] [157] <figures/corr_pdist.png, id=1138, 698.61pt x 875.27pt>
<use figures/corr_pdist.png>
<figures/wtangent.png, id=1139, 698.61pt x 875.27pt>
<use figures/wtangent.png>

LaTeX Warning: Reference `fig:indeptrials' on page 158 undefined on input line 
156.


LaTeX Warning: Reference `eq:trialthat' on page 158 undefined on input line 156
.


LaTeX Warning: Reference `fig:indeptrials' on page 158 undefined on input line 
156.


LaTeX Warning: Reference `eq:trialthat' on page 158 undefined on input line 156
.

[158 <./figures/corr_pdist.png> <./figures/wtangent.png>]

LaTeX Warning: Reference `fig:1seccumdistp' on page 159 undefined on input line
 170.


LaTeX Warning: Reference `eq:trialthat' on page 159 undefined on input line 171
.


LaTeX Warning: Reference `fig:p2secspacecorr' on page 159 undefined on input li
ne 173.


LaTeX Warning: Reference `fig:1secspacecorr' on page 159 undefined on input lin
e 173.


LaTeX Warning: Reference `fig:10secspacecorr' on page 159 undefined on input li
ne 174.


LaTeX Warning: Reference `sec:corrtrials' on page 159 undefined on input line 1
79.


LaTeX Warning: Reference `tab:spacefits' on page 159 undefined on input line 17
9.


LaTeX Warning: Reference `fig:p2secspacecorr' on page 159 undefined on input li
ne 181.


LaTeX Warning: Reference `fig:10secspacecorr' on page 159 undefined on input li
ne 181.

[159] <figures/gcumulative_1sec.png, id=1153, 1200.485pt x 875.27pt>
<use figures/gcumulative_1sec.png> [160 <./figures/gcumulative_1sec.png>]
<figures/gcorrection_p2sec.png, id=1160, 1200.485pt x 875.27pt>
<use figures/gcorrection_p2sec.png>
<figures/gcumulative_corr_p2sec.png, id=1161, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_p2sec.png> [161 <./figures/gcorrection_p2sec.png>
 <./figures/gcumulative_corr_p2sec.png>]
<figures/gcorrection_1sec.png, id=1170, 1200.485pt x 875.27pt>
<use figures/gcorrection_1sec.png>
<figures/gcumulative_corr_1sec.png, id=1171, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_1sec.png> [162 <./figures/gcorrection_1sec.png> <
./figures/gcumulative_corr_1sec.png>]
<figures/gcorrection_10sec.png, id=1180, 1200.485pt x 875.27pt>
<use figures/gcorrection_10sec.png>
<figures/gcumulative_corr_10sec.png, id=1181, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_10sec.png> [163 <./figures/gcorrection_10sec.png>
 <./figures/gcumulative_corr_10sec.png>]

LaTeX Warning: Reference `sec:space' on page 164 undefined on input line 274.


LaTeX Warning: Reference `sec:space' on page 164 undefined on input line 279.


LaTeX Warning: Reference `tab:timefits' on page 164 undefined on input line 280
.

[164] <figures/gcorrection_time_p2sec.png, id=1196, 917.4275pt x 754.82pt>
<use figures/gcorrection_time_p2sec.png> [165 <./figures/gcorrection_time_p2sec
.png>] <figures/gcorrection_time_1sec.png, id=1203, 914.41624pt x 747.79375pt>
<use figures/gcorrection_time_1sec.png> [166 <./figures/gcorrection_time_1sec.p
ng>] <figures/gcorrection_time_10sec.png, id=1210, 912.40875pt x 741.77126pt>
<use figures/gcorrection_time_10sec.png> [167 <./figures/gcorrection_time_10sec
.png>] [168]

LaTeX Warning: Reference `sec:space' on page 169 undefined on input line 368.


LaTeX Warning: Reference `sec:temporal' on page 169 undefined on input line 368
.

) [169] (./Sensitivity.tex
Chapter 6.

LaTeX Warning: Reference `ch:method' on page 170 undefined on input line 4.


LaTeX Warning: Reference `sec:optimalspatialbin' on page 170 undefined on input
 line 17.


LaTeX Warning: Reference `sec:finalcuts' on page 170 undefined on input line 17
.


LaTeX Warning: Citation `Taboada:2013uza' on page 170 undefined on input line 2
2.

[170]

LaTeX Warning: Reference `sec:duropt' on page 171 undefined on input line 24.


LaTeX Warning: Reference `sec:sensflu' on page 171 undefined on input line 33.


LaTeX Warning: Reference `ch:Reco' on page 171 undefined on input line 36.

[171]

LaTeX Warning: Citation `CORSIKA:1998' on page 172 undefined on input line 45.


LaTeX Warning: Citation `GEANT4:2016' on page 172 undefined on input line 45.


LaTeX Warning: Citation `Ahn:2010' on page 172 undefined on input line 47.

[172]

LaTeX Warning: Reference `fig:psf_geom' on page 173 undefined on input line 82.


[173] <figures/psf_geom.png, id=1249, 937.5025pt x 500.87125pt>
<use figures/psf_geom.png>

LaTeX Warning: Reference `fig:opt_gaus_bin' on page 174 undefined on input line
 108.

[174 <./figures/psf_geom.png>]
<figures/sens_v_spatial_bin_size.png, id=1258, 1200.485pt x 875.27pt>
<use figures/sens_v_spatial_bin_size.png>

LaTeX Warning: Reference `eq:gaus_sig' on page 175 undefined on input line 122.


[175 <./figures/sens_v_spatial_bin_size.png>]

LaTeX Warning: Reference `fig:psf_geom' on page 176 undefined on input line 148
.


LaTeX Warning: Reference `eq:signal_in_square' on page 176 undefined on input l
ine 154.


LaTeX Warning: Reference `fig:opt_gaus_bin' on page 176 undefined on input line
 156.

[176] [177]

LaTeX Warning: Reference `fig:poissonopt_check' on page 178 undefined on input 
line 181.


LaTeX Warning: Reference `fig:poissonoptrad' on page 178 undefined on input lin
e 181.


LaTeX Warning: Reference `fig:poissonopt_check' on page 178 undefined on input 
line 182.


LaTeX Warning: Reference `fig:poissonoptrad' on page 178 undefined on input lin
e 184.


LaTeX Warning: Reference `fig:poissonoptrad' on page 178 undefined on input lin
e 193.


LaTeX Warning: Reference `fig:poissonoptrad' on page 178 undefined on input lin
e 196.


LaTeX Warning: Reference `ch:Reco' on page 178 undefined on input line 198.

[178] [179]
<figures/sensitivity_v_tophat_radius_bg1000.png, id=1287, 1200.485pt x 875.27pt
> <use figures/sensitivity_v_tophat_radius_bg1000.png> [180 <./figures/sensitiv
ity_v_tophat_radius_bg1000.png>]
<figures/sensitivity_v_tophat_radius_bg_p1.png, id=1294, 1200.485pt x 875.27pt>
<use figures/sensitivity_v_tophat_radius_bg_p1.png> [181 <./figures/sensitivity
_v_tophat_radius_bg_p1.png>]

LaTeX Warning: Reference `ch:Reco' on page 182 undefined on input line 248.


LaTeX Warning: Citation `Abeysekara:2013tza' on page 182 undefined on input lin
e 255.


LaTeX Warning: Reference `ch:Reco' on page 182 undefined on input line 260.


LaTeX Warning: Reference `sec:poissonopt' on page 182 undefined on input line 2
62.

[182] [183]

LaTeX Warning: Reference `tab:grbmodels' on page 184 undefined on input line 27
4.


LaTeX Warning: Citation `GILMORE2012' on page 184 undefined on input line 275.

[184]

LaTeX Warning: Citation `Ackermann:2013a' on page 185 undefined on input line 2
94.


LaTeX Warning: Citation `Ackermann:2013a' on page 185 undefined on input line 2
94.


LaTeX Warning: Reference `fig:shortdiffsens' on page 185 undefined on input lin
e 305.


LaTeX Warning: Reference `fig:longdiffsens' on page 185 undefined on input line
 305.


LaTeX Warning: Reference `ch:Reco' on page 185 undefined on input line 315.


LaTeX Warning: Reference `sec:sensflu' on page 185 undefined on input line 323.


[185] [186]
<figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png, id=1327, 1200.485p
t x 875.27pt> <use figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png>

LaTeX Warning: Reference `tab:grbmodels' on page 187 undefined on input line 33
5.


LaTeX Warning: Reference `tab:grbmodels' on page 187 undefined on input line 33
5.

[187 <./figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png>]
<figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png, id=1334, 1200.485
pt x 875.27pt>
<use figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png>

LaTeX Warning: Reference `tab:grbmodels' on page 188 undefined on input line 35
0.


LaTeX Warning: Reference `tab:grbmodels' on page 188 undefined on input line 35
0.

[188 <./figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png>]

LaTeX Warning: Reference `sec:diffsens' on page 189 undefined on input line 361
.


LaTeX Warning: Reference `tab:paramspace' on page 189 undefined on input line 3
63.


LaTeX Warning: Reference `tab:fincut' on page 189 undefined on input line 370.

[189] [190]

LaTeX Warning: Reference `tab:fincut' on page 191 undefined on input line 412.


LaTeX Warning: Reference `fig:nearcrab' on page 191 undefined on input line 417
.

<figures/grb_cuts_near_crab.png, id=1351, 669.50125pt x 563.10374pt>
<use figures/grb_cuts_near_crab.png>

LaTeX Warning: Reference `tab:fincut' on page 191 undefined on input line 426.


LaTeX Warning: Reference `tab:fincut' on page 191 undefined on input line 426.

[191 <./figures/grb_cuts_near_crab.png>]

LaTeX Warning: Reference `tab:backpass' on page 192 undefined on input line 433
.


LaTeX Warning: Reference `tab:fincut' on page 192 undefined on input line 434.


LaTeX Warning: Reference `ch:hawcobs' on page 192 undefined on input line 436.


LaTeX Warning: Reference `sec:sensflu' on page 192 undefined on input line 441.



LaTeX Warning: Reference `tab:fincut' on page 192 undefined on input line 461.


LaTeX Warning: Reference `tab:fincut' on page 192 undefined on input line 461.

[192]

LaTeX Warning: Reference `fig:flushort' on page 193 undefined on input line 473
.


LaTeX Warning: Reference `fig:flulong' on page 193 undefined on input line 473.



LaTeX Warning: Reference `sec:diffsens' on page 193 undefined on input line 476
.


LaTeX Warning: Reference `ch:method' on page 193 undefined on input line 478.


LaTeX Warning: Reference `fig:flushort' on page 193 undefined on input line 485
.


LaTeX Warning: Reference `fig:flulong' on page 193 undefined on input line 485.


[193] <figures/sensitivity_money.png, id=1369, 1200.485pt x 875.27pt>
<use figures/sensitivity_money.png>

LaTeX Warning: Citation `Ackermann:2013a' on page 194 undefined on input line 5
06.


LaTeX Warning: Citation `Ackermann:2013a' on page 194 undefined on input line 5
06.

[194 <./figures/sensitivity_money.png>]
<figures/sensitivity_money_long.png, id=1375, 1200.485pt x 875.27pt>
<use figures/sensitivity_money_long.png>

LaTeX Warning: Citation `Zhu:2013GCN' on page 195 undefined on input line 525.


LaTeX Warning: Citation `Zhu:2013GCN' on page 195 undefined on input line 525.

[195 <./figures/sensitivity_money_long.png>]

LaTeX Warning: Citation `Ghisellini:2010' on page 196 undefined on input line 5
47.


LaTeX Warning: Citation `Beloborodov:2014' on page 196 undefined on input line 
550.


LaTeX Warning: Citation `Ferrara:2015' on page 196 undefined on input line 555.



LaTeX Warning: Citation `LAT:2016' on page 196 undefined on input line 556.

[196]

LaTeX Warning: Reference `fig:bgcorrlc' on page 197 undefined on input line 562
.


LaTeX Warning: Reference `fig:lcinhawc' on page 197 undefined on input line 562
.

<figures/bg_corrected_fermi.png, id=1386, 1200.485pt x 875.27pt>
<use figures/bg_corrected_fermi.png>
<figures/grb090510_on_hawc.png, id=1387, 1200.485pt x 875.27pt>
<use figures/grb090510_on_hawc.png> [197 <./figures/bg_corrected_fermi.png>]

LaTeX Warning: Reference `ch:method' on page 198 undefined on input line 601.

[198 <./figures/grb090510_on_hawc.png>]

LaTeX Warning: Citation `Beloborodov:2014' on page 199 undefined on input line 
608.


LaTeX Warning: Reference `tab:spanlong' on page 199 undefined on input line 610
.


LaTeX Warning: Reference `tab:spanshort' on page 199 undefined on input line 61
0.

[199] [200] [201]

LaTeX Warning: Reference `sec:spandur' on page 202 undefined on input line 703.



LaTeX Warning: Reference `tab:threelong' on page 202 undefined on input line 70
4.


LaTeX Warning: Reference `tab:threeshort' on page 202 undefined on input line 7
04.


LaTeX Warning: Reference `sec:spandur' on page 202 undefined on input line 714.


[202]) [203] [204] (./Results.tex
Chapter 7.

LaTeX Warning: Reference `ch:method' on page 205 undefined on input line 6.


LaTeX Warning: Reference `ch:sens' on page 205 undefined on input line 7.


LaTeX Warning: Reference `ch:Reco' on page 205 undefined on input line 8.


LaTeX Warning: Reference `sec:dataset' on page 205 undefined on input line 10.


LaTeX Warning: Reference `sec:bestcand' on page 205 undefined on input line 11.



LaTeX Warning: Reference `sec:limits' on page 205 undefined on input line 13.


LaTeX Warning: Reference `ch:sens' on page 205 undefined on input line 14.

[205]

LaTeX Warning: Reference `fig:datapie' on page 206 undefined on input line 38.

[206] <figures/datapie.png, id=1440, 985.6825pt x 631.35875pt>
<use figures/datapie.png> [207 <./figures/datapie.png>]

LaTeX Warning: Reference `tab:besties' on page 208 undefined on input line 64.


LaTeX Warning: Reference `ch:method' on page 208 undefined on input line 68.


LaTeX Warning: Reference `tab:besties' on page 208 undefined on input line 70.


LaTeX Warning: Reference `ch:method' on page 208 undefined on input line 86.


LaTeX Warning: Reference `ch:method' on page 208 undefined on input line 86.

[208]

LaTeX Warning: Reference `tab:1seccand' on page 209 undefined on input line 95.



LaTeX Warning: Reference `fig:rateplot' on page 209 undefined on input line 96.



LaTeX Warning: Reference `fig:myskymap' on page 209 undefined on input line 98.



LaTeX Warning: Reference `fig:thatsfine' on page 209 undefined on input line 99
.


LaTeX Warning: Reference `coarselc' on page 209 undefined on input line 102.


LaTeX Warning: Reference `fig:psmap' on page 209 undefined on input line 111.

[209] <figures/rate1_zoom.png, id=1457, 798.985pt x 574.145pt>
<use figures/rate1_zoom.png> [210 <./figures/rate1_zoom.png>]
<figures/inlay.png, id=1466, 987.69pt x 716.6775pt> <use figures/inlay.png>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 159--161
 [] 
[211 <./figures/inlay.png>]
<figures/candidate_lightcurve.png, id=1473, 899.36pt x 574.145pt>
<use figures/candidate_lightcurve.png>

LaTeX Warning: Reference `coarselc' on page 212 undefined on input line 176.


LaTeX Warning: Reference `coarselc' on page 212 undefined on input line 176.

[212 <./figures/candidate_lightcurve.png>]
<figures/lc_coarse.png, id=1480, 798.985pt x 574.145pt>
<use figures/lc_coarse.png> [213 <./figures/lc_coarse.png>]
<figures/candidate_location_full_skymap.png, id=1487, 433.62pt x 487.8225pt>
<use figures/candidate_location_full_skymap.png>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 208--210
 [] 
[214 <./figures/candidate_location_full_skymap.png>]

LaTeX Warning: Reference `ch:sens' on page 215 undefined on input line 223.

[215]

LaTeX Warning: Reference `fig:grbrate' on page 216 undefined on input line 244.



LaTeX Warning: Reference `fig:grbratelong' on page 216 undefined on input line 
244.


LaTeX Warning: Reference `ch:sens' on page 216 undefined on input line 252.


LaTeX Warning: Citation `Ackermann:2013a' on page 216 undefined on input line 2
59.


LaTeX Warning: Reference `tab:latburstlist' on page 216 undefined on input line
 264.

[216]

LaTeX Warning: Citation `Ackermann:2013a' on page 217 undefined on input line 2
70.


LaTeX Warning: Reference `fig:grbrate' on page 217 undefined on input line 281.



LaTeX Warning: Citation `Ackermann:2013a' on page 217 undefined on input line 2
83.

[217]

LaTeX Warning: Citation `Maselli:2013uza' on page 218 undefined on input line 3
33.


LaTeX Warning: Citation `FLUENCE:2013' on page 218 undefined on input line 333.



LaTeX Warning: Citation `Ackermann:2013a' on page 218 undefined on input line 3
33.


LaTeX Warning: Citation `Maselli:2013uza' on page 218 undefined on input line 3
33.


LaTeX Warning: Citation `FLUENCE:2013' on page 218 undefined on input line 333.



LaTeX Warning: Citation `Ackermann:2013a' on page 218 undefined on input line 3
33.

[218] <figures/limit_grbrate.png, id=1513, 1200.485pt x 875.27pt>
<use figures/limit_grbrate.png>

LaTeX Warning: Reference `ch:sens' on page 219 undefined on input line 354.


LaTeX Warning: Reference `ch:sens' on page 219 undefined on input line 354.

[219 <./figures/limit_grbrate.png>]
<figures/grbrate_long.png, id=1519, 1200.485pt x 875.27pt>
<use figures/grbrate_long.png> [220 <./figures/grbrate_long.png>] [221])
[222] (./AppendixC.tex
Appendix A.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\Gamma' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `subscript' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 5.


LaTeX Warning: Citation `Gould:1966' on page 223 undefined on input line 22.

[223]

LaTeX Warning: Reference `eq:Nthatthing' on page 224 undefined on input line 43
.

[224]

LaTeX Warning: Citation `Fermi:2008' on page 225 undefined on input line 65.

) [225] (./AppendixB.tex
Appendix B.

LaTeX Warning: Reference `fig:coax_circuit' on page 226 undefined on input line
 8.


LaTeX Warning: Reference `eq:redvolt' on page 226 undefined on input line 31.


LaTeX Warning: Reference `eq:redcurr' on page 226 undefined on input line 36.

[226]

LaTeX Warning: Reference `tab:coaxcab_hf' on page 227 undefined on input line 6
1.


LaTeX Warning: Citation `Wigington:1957' on page 227 undefined on input line 68
.


LaTeX Warning: Reference `eq:k_with_r' on page 227 undefined on input line 68.


LaTeX Warning: Reference `eq:k_w_K' on page 227 undefined on input line 74.

[227]) [228] (./AppendixD.tex
Appendix C.
<figures/analog_input_circuit.png, id=1593, 310.15875pt x 229.85875pt>
<use figures/analog_input_circuit.png>

LaTeX Warning: Reference `fig:analog_circuit' on page 229 undefined on input li
ne 10.


LaTeX Warning: Reference `eq:analog_input_circuit' on page 229 undefined on inp
ut line 14.

[229 <./figures/analog_input_circuit.png>]) [230] (./AppendixE.tex
Appendix D.
<figures/analog_load_circuit.png, id=1610, 845.1575pt x 345.29pt>
<use figures/analog_load_circuit.png>

LaTeX Warning: Reference `fig:analog_circuit' on page 231 undefined on input li
ne 11.

[231 <./figures/analog_load_circuit.png>]

LaTeX Warning: Reference `eq:trans_gain' on page 232 undefined on input line 42
.

) [232] (./AppendixF.tex
Appendix E.

LaTeX Warning: Reference `fig:pmtbase' on page 233 undefined on input line 7.


LaTeX Warning: Reference `tab:resvolts' on page 233 undefined on input line 9.


LaTeX Warning: Reference `fig:pmtbase' on page 233 undefined on input line 30.


LaTeX Warning: Reference `fig:pmtbase' on page 233 undefined on input line 30.

<figures/milagro_pmt_base_via_bob_28nov11.pdf, id=1628, 614.295pt x 794.97pt>
<use figures/milagro_pmt_base_via_bob_28nov11.pdf>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 37--38
 [] 
) [233]

LaTeX Warning: Text page 234 contains only floats.

[234 <./figures/milagro_pmt_base_via_bob_28nov11.pdf>] (./thesis.bbl
Underfull \hbox (badness 2213) in paragraph at lines 19--22
[]\OT1/cmr/m/n/12 M. Briggs.  Gamma-Ray As-tro-physics NSSTC BATSE GRB.  \OT1/c
mr/m/it/12 URL
[235]
Underfull \hbox (badness 3407) in paragraph at lines 139--142
[]\OT1/cmr/m/n/12 S. et al. Woose-ley.  The Su-per-nova Gamma-ray Burst Con-nec
-tion.
[236] [237] [238]
Underfull \hbox (badness 3439) in paragraph at lines 429--434
[]\OT1/cmr/m/n/12 E. Fer-rara.  Caveats About An-a-lyz-ing LAT Pass 8 Data.  \O
T1/cmr/m/it/12 URL

Underfull \hbox (badness 10000) in paragraph at lines 436--441
[]\OT1/cmr/m/n/12 Fermi LAT Col-lab-o-ra-tion.  Fermi LAT GRBs.  \OT1/cmr/m/it/
12 URL

Underfull \hbox (badness 10000) in paragraph at lines 443--447
[]\OT1/cmr/m/n/12 S. No-bili.  GRB 130427A: A CHANCE NOT TO MISS.
[239]) [240] (./thesis.aux (./Abstract.aux) (./Titlepage.aux) (./Copyright.aux)
 (./Abbreviations.aux) (./GRBs.aux) (./Showers.aux) (./HAWC.aux) (./Reco.aux)
(./Method.aux) (./Trials.aux) (./Sensitivity.aux) (./Results.aux)
(./AppendixC.aux) (./AppendixB.aux) (./AppendixD.aux) (./AppendixE.aux)
(./AppendixF.aux))

Package rerunfilecheck Warning: File `thesis.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.


LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information)</usr/local/texlive/2015/te
xmf-dist/fonts/type1/public/amsfonts/cm/cmbx12.pfb></usr/local/texlive/2015/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2015/texm
f-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2015/texmf
-dist/fonts/type1/public/amsfonts/cm/cmmi12.pfb></usr/local/texlive/2015/texmf-
dist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2015/texmf-di
st/fonts/type1/public/amsfonts/cm/cmmi8.pfb></usr/local/texlive/2015/texmf-dist
/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2015/texmf-dist/f
onts/type1/public/amsfonts/cm/cmr12.pfb></usr/local/texlive/2015/texmf-dist/fon
ts/type1/public/amsfonts/cm/cmr6.pfb></usr/local/texlive/2015/texmf-dist/fonts/
type1/public/amsfonts/cm/cmr8.pfb></usr/local/texlive/2015/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2015/texmf-dist/fonts/type
1/public/amsfonts/cm/cmsy6.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/
public/amsfonts/cm/cmsy8.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmti12.pfb>
Output written on thesis.pdf (247 pages, 8928893 bytes).
Transcript written on thesis.log.
bibtex thesis
This is BibTeX, Version 0.99d (TeX Live 2015)
The top-level auxiliary file: thesis.aux
A level-1 auxiliary file: Abstract.aux
A level-1 auxiliary file: Titlepage.aux
A level-1 auxiliary file: Copyright.aux
A level-1 auxiliary file: Abbreviations.aux
A level-1 auxiliary file: GRBs.aux
A level-1 auxiliary file: Showers.aux
A level-1 auxiliary file: HAWC.aux
A level-1 auxiliary file: Reco.aux
A level-1 auxiliary file: Method.aux
A level-1 auxiliary file: Trials.aux
A level-1 auxiliary file: Sensitivity.aux
A level-1 auxiliary file: Results.aux
A level-1 auxiliary file: AppendixC.aux
A level-1 auxiliary file: AppendixB.aux
A level-1 auxiliary file: AppendixD.aux
A level-1 auxiliary file: AppendixE.aux
A level-1 auxiliary file: AppendixF.aux
The style file: unsrt.bst
Database file #1: Bibliography.bib
Warning--empty journal in Zhu:2013ufa
Warning--empty journal in DCHOOZ2011
Warning--empty author in GEANT4:2016
(There were 3 warnings)
pdflatex thesis
This is pdfTeX, Version 3.14159265-2.6-1.40.16 (TeX Live 2015) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./thesis.tex
LaTeX2e <2015/01/01>
Babel <3.9l> and hyphenation patterns for 79 languages loaded.
(./thesis.cls
Document Class: thesis 2006/04/26 v0.1
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/size12.clo))
(./styles/titlesec.sty

LaTeX Warning: You have requested package `styles/titlesec',
               but the package provides `titlesec'.

) (/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/graphics.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/pdftex-def/pdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/lscape.sty)
(./styles/indentfirst.sty

LaTeX Warning: You have requested package `styles/indentfirst',
               but the package provides `indentfirst'.

) (./styles/latexsym.sty

LaTeX Warning: You have requested package `styles/latexsym',
               but the package provides `latexsym'.

) (./styles/multirow.sty) (./styles/tabls.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(./styles/slashbox.sty
slashbox style by K.Yasuoka, May 1993.
) (/usr/local/texlive/2015/texmf-dist/tex/latex/tools/longtable.sty)
(./styles/supertabular.sty

LaTeX Warning: You have requested package `styles/supertabular',
               but the package provides `supertabular'.

) (/usr/local/texlive/2015/texmf-dist/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/local/texlive/2015/texmf-dist/tex/latex/subfigure/subfigure.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2015/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/url/url.sty))

Package hyperref Message: Driver: hpdftex.

(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/lineno/lineno.sty) (./thesis.aux
(./Abstract.aux) (./Titlepage.aux) (./Copyright.aux) (./Abbreviations.aux)
(./GRBs.aux) (./Showers.aux) (./HAWC.aux) (./Reco.aux) (./Method.aux)
(./Trials.aux

LaTeX Warning: Label `eq:trialthat' multiply defined.


LaTeX Warning: Label `fig:10secspacecorr' multiply defined.

) (./Sensitivity.aux) (./Results.aux) (./AppendixC.aux) (./AppendixB.aux)
(./AppendixD.aux) (./AppendixE.aux) (./AppendixF.aux))
(/usr/local/texlive/2015/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/color.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./thesis.out) (./thesis.out) (./Abstract.tex
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/ulasy.fd)) [1{/usr/local/tex
live/2015/texmf-var/fonts/map/pdftex/updmap/pdftex.map}] [2] (./Titlepage.tex)
[3] (./Copyright.tex
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/omscmr.fd)) [4]
(./thesis.toc [2] [3]) [4] (./thesis.lof
Overfull \hbox (14.12067pt too wide) in paragraph at lines 3--3
 [][] [][][]\OT1/cmr/m/n/12 Twelve light curves for mea-sured BATSE GRBs [[][]2
[][]]. The short timescales 
[5]
Overfull \hbox (18.10568pt too wide) in paragraph at lines 15--15
 \OT1/cmr/m/n/12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 03\OML/cmm/m/it/12 ; \OT1/c
mr/m/n/12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 25\OML/cmm/m/it/12 ; \OT1/cmr/m/n/
12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 5\OML/cmm/m/it/12 ; \OT1/cmr/m/n/12 1\OML
/cmm/m/it/12 :\OT1/cmr/m/n/12 0$ for the WMAP5 Fidu-cial (solid black), WMAP5+F
ixed 
[6] [7] [8] [9] [10] [11] [12]
Overfull \hbox (0.82274pt too wide) in paragraph at lines 59--59
 \OT1/cmr/m/n/12 cles (NKG) and elec-tro-mag-netic shower en-ergy (NKG/R) in a 
gamma- 
[13] [14] [15] [16] [17] [18] [19] [20] [21] [22]) [23] (./Abbreviations.tex)
[24] (./GRBs.tex
Chapter 1.
pdfTeX warning (ext4): destination with the same identifier (name{page.1}) has 
been already used, duplicate ignored
<to be read again> 
                   \relax 
l.26 
      [1]pdfTeX warning (ext4): destination with the same identifier (name{page
.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.49 
      [2]pdfTeX warning (ext4): destination with the same identifier (name{page
.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.73 \newpage
              [3]pdfTeX warning (ext4): destination with the same identifier (n
ame{page.4}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.88 \newpage
              [4] [5] <figures/batse_t90.png, id=1463, 931.48pt x 692.5875pt>
<use figures/batse_t90.png> [6 <./figures/batse_t90.png>]
<figures/batse_panel.png, id=1472, 923.45pt x 911.405pt>
<use figures/batse_panel.png> [7 <./figures/batse_panel.png>] [8]
<figures/bandfuncfig.pdf, id=1494, 612.09195pt x 615.50294pt>
<use figures/bandfuncfig.pdf> [9 <./figures/bandfuncfig.pdf>]
<figures/batse_spatial.png, id=1513, 980.66376pt x 706.64pt>
<use figures/batse_spatial.png> [10 <./figures/batse_spatial.png>] [11]
<figures/jetbreak.png, id=1530, 619.31375pt x 478.78876pt>
<use figures/jetbreak.png> [12 <./figures/jetbreak.png>] [13]
<figures/redshift.png, id=1557, 1025.8325pt x 832.10875pt>
<use figures/redshift.png> [14 <./figures/redshift.png>] [15]
<figures/fluenceratio.png, id=1580, 706.64pt x 689.57625pt>
<use figures/fluenceratio.png> [16 <./figures/fluenceratio.png>] [17]
<figures/fermicutoff.png, id=1596, 960.58875pt x 728.7225pt>
<use figures/fermicutoff.png> [18 <./figures/fermicutoff.png>] [19]
<figures/hess_scheme.jpg, id=1617, 413.545pt x 385.44pt>
<use figures/hess_scheme.jpg>
<figures/wct.jpg, id=1618, 602.25pt x 615.29875pt> <use figures/wct.jpg>
[20 <./figures/hess_scheme.jpg> <./figures/wct.jpg>] [21] [22]
<figures/EffArea.png, id=1651, 734.9859pt x 445.9059pt>
<use figures/EffArea.png> [23 <./figures/EffArea.png>] [24]
<figures/fireballmodel.png, id=1670, 1154.3125pt x 899.36pt>
<use figures/fireballmodel.png> [25 <./figures/fireballmodel.png>] [26]
[27] [28] [29] [30]
<figures/short_grb_cutoff.png, id=1732, 800.9925pt x 677.53125pt>
<use figures/short_grb_cutoff.png> [31 <./figures/short_grb_cutoff.png>]
[32] <figures/ebl_flux.png, id=1751, 1090.0725pt x 921.4425pt>
<use figures/ebl_flux.png> [33 <./figures/ebl_flux.png>]
<figures/gilmore_2012_EBL_atten.png, id=1766, 667.49374pt x 649.42625pt>
<use figures/gilmore_2012_EBL_atten.png> [34 <./figures/gilmore_2012_EBL_atten.
png>] [35]) [36] (./Showers.tex
Chapter 2.
[37] [38]
Overfull \hbox (12.82234pt too wide) in paragraph at lines 36--41
\OT1/cmr/m/n/12 The elec-tron and positron pair sub-se-quently gen-er-ate more 
pho-tons via Bremsstrahlung
[39] <figures/gamma_shower_model.png, id=1814, 650.43pt x 502.87875pt>
<use figures/gamma_shower_model.png> [40] [41 <./figures/gamma_shower_model.png
>] <figures/gamma_shower_profile.png, id=1832, 1200.485pt x 875.27pt>
<use figures/gamma_shower_profile.png> [42 <./figures/gamma_shower_profile.png>
] [43] <figures/eas_diagram.png, id=1855, 410.53375pt x 658.46pt>
<use figures/eas_diagram.png> [44] [45 <./figures/eas_diagram.png>] [46]
<figures/proton_shower_profile.png, id=1879, 1200.485pt x 875.27pt>
<use figures/proton_shower_profile.png> [47 <./figures/proton_shower_profile.pn
g>] <figures/proton_particle_number.png, id=1886, 634.37pt x 718.685pt>
<use figures/proton_particle_number.png> [48 <./figures/proton_particle_number.
png>] [49] <figures/shower_timing.png, id=1903, 562.1pt x 628.3475pt>
<use figures/shower_timing.png> [50 <./figures/shower_timing.png>]
<figures/side_shower.png, id=1914, 608.2725pt x 744.7825pt>
<use figures/side_shower.png>) [51] [52 <./figures/side_shower.png>]
(./HAWC.tex
Chapter 3.
[53] <figures/HAWC_overview.jpeg, id=1933, 1080.035pt x 725.71124pt>
<use figures/HAWC_overview.jpeg> [54 <./figures/HAWC_overview.jpeg>] [55]
<figures/HAWC_tank.png, id=1944, 839.135pt x 688.5725pt>
<use figures/HAWC_tank.png>
<figures/HAWC_bladder.png, id=1945, 182.1204pt x 168.63pt>
<use figures/HAWC_bladder.png> [56 <./figures/HAWC_tank.png> <./figures/HAWC_bl
adder.png>] [57] <figures/regularpulse.png, id=1957, 520.94624pt x 706.64pt>
<use figures/regularpulse.png>
<figures/HAWC_pmt.png, id=1958, 171.039pt x 227.8914pt>
<use figures/HAWC_pmt.png> [58 <./figures/regularpulse.png> <./figures/HAWC_pmt
.png>] [59] <figures/single_pe_charge.jpeg, id=1975, 990.70125pt x 736.7525pt>
<use figures/single_pe_charge.jpeg> [60 <./figures/single_pe_charge.jpeg>]
[61] <figures/r5912_quantum_efficiency.png, id=1987, 610.28pt x 664.4825pt>
<use figures/r5912_quantum_efficiency.png>
<figures/r7081_HQE_quantum_efficiency.png, id=1988, 546.04pt x 696.6025pt>
<use figures/r7081_HQE_quantum_efficiency.png> [62 <./figures/r5912_quantum_eff
iciency.png> <./figures/r7081_HQE_quantum_efficiency.png>] [63]
<figures/signal_overview.png, id=2003, 914.41624pt x 311.1625pt>
<use figures/signal_overview.png> [64 <./figures/signal_overview.png>] [65]
<figures/coax_diagram.png, id=2016, 484.81125pt x 483.8075pt>
<use figures/coax_diagram.png> [66 <./figures/coax_diagram.png>]
<figures/circuit.png, id=2031, 860.21375pt x 442.65375pt>
<use figures/circuit.png> [67 <./figures/circuit.png>] [68] [69]
<figures/comp_cable.png, id=2059, 1200.485pt x 875.27pt>
<use figures/comp_cable.png> [70 <./figures/comp_cable.png>]
<figures/analog_circuit.png, id=2067, 1186.4325pt x 665.48625pt>
<use figures/analog_circuit.png> [71 <./figures/analog_circuit.png>] [72]
[73] [74] <figures/AnalogFEB_4edge.png, id=2097, 1202.4925pt x 878.28125pt>
<use figures/AnalogFEB_4edge.png> [75 <./figures/AnalogFEB_4edge.png>]
<figures/AnalogFEB_2edge.png, id=2107, 1202.4925pt x 878.28125pt>
<use figures/AnalogFEB_2edge.png> [76 <./figures/AnalogFEB_2edge.png>]
<figures/digital_logic.png, id=2115, 968.61874pt x 628.3475pt>
<use figures/digital_logic.png> [77 <./figures/digital_logic.png>]
<figures/latch_circuit.png, id=2124, 894.34125pt x 481.8pt>
<use figures/latch_circuit.png> [78 <./figures/latch_circuit.png>]
<figures/flip_flop_logic.png, id=2130, 352.31625pt x 269.005pt>
<use figures/flip_flop_logic.png>
<figures/logic_table.png, id=2131, 666.49pt x 470.75874pt>
<use figures/logic_table.png> [79 <./figures/flip_flop_logic.png> <./figures/lo
gic_table.png>]
<figures/flip_flop_20ns.png, id=2141, 700.6175pt x 476.78125pt>
<use figures/flip_flop_20ns.png> [80 <./figures/flip_flop_20ns.png>]
<figures/one-shot_width_vs_R.png, id=2146, 901.3675pt x 777.90625pt>
<use figures/one-shot_width_vs_R.png> [81 <./figures/one-shot_width_vs_R.png>]
[82] <figures/delay_circuit.png, id=2158, 697.60625pt x 202.7575pt>
<use figures/delay_circuit.png> [83 <./figures/delay_circuit.png>] [84]
<figures/DigitalFEB_4edge.png, id=2176, 1202.4925pt x 426.59375pt>
<use figures/DigitalFEB_4edge.png>
Overfull \hbox (43.36244pt too wide) in paragraph at lines 595--596
 [] 
[85 <./figures/DigitalFEB_4edge.png>] [86]
<figures/DigitalFEB_2edge.png, id=2195, 1202.4925pt x 426.59375pt>
<use figures/DigitalFEB_2edge.png>
Overfull \hbox (43.36244pt too wide) in paragraph at lines 638--639
 [] 
[87 <./figures/DigitalFEB_2edge.png>] [88] [89]
<figures/early_TDC_event.png, id=2218, 855.195pt x 610.28pt>
<use figures/early_TDC_event.png> [90 <./figures/early_TDC_event.png>] [91]
<figures/online_reco_chain.png, id=2233, 1038.88126pt x 591.20876pt>
<use figures/online_reco_chain.png> [92 <./figures/online_reco_chain.png>]
<figures/timediagram.png, id=2240, 1013.7875pt x 633.36626pt>
<use figures/timediagram.png> [93 <./figures/timediagram.png>] [94]
<figures/OnlineLatencyBigBins.png, id=2254, 922.44624pt x 617.30624pt>
<use figures/OnlineLatencyBigBins.png> [95 <./figures/OnlineLatencyBigBins.png>
] [96]
<figures/Calibration_Simplified_Layout.png, id=2269, 794.4882pt x 654.2844pt>
<use figures/Calibration_Simplified_Layout.png> [97 <./figures/Calibration_Simp
lified_Layout.png>]
<figures/chargecalib_curves_run5213_H13.png, id=2274, 1367.1075pt x 701.62125pt
> <use figures/chargecalib_curves_run5213_H13.png> [98 <./figures/chargecalib_c
urves_run5213_H13.png>]
<figures/H13_slewing.png, id=2280, 999.735pt x 774.895pt>
<use figures/H13_slewing.png> [99 <./figures/H13_slewing.png>] [100] [101]
[102] [103] <figures/10inch_lostart.png, id=2321, 800.9925pt x 577.15625pt>
<use figures/10inch_lostart.png>
<figures/10inch_histart.png, id=2322, 798.985pt x 574.145pt>
<use figures/10inch_histart.png> [104 <./figures/10inch_lostart.png> <./figures
/10inch_histart.png>]
<figures/8inch_lostart.png, id=2329, 798.985pt x 574.145pt>
<use figures/8inch_lostart.png>
<figures/8inch_histart.png, id=2330, 798.985pt x 574.145pt>
<use figures/8inch_histart.png> [105 <./figures/8inch_lostart.png> <./figures/8
inch_histart.png>] [106]
<figures/afterpulsing_rate.png, id=2345, 937.5025pt x 669.50125pt>
<use figures/afterpulsing_rate.png> [107 <./figures/afterpulsing_rate.png>]
Overfull \hbox (0.59285pt too wide) in paragraph at lines 970--974
\OT1/cmr/m/n/12 for ion-iza-tion oc-cur-ring a dis-tance $\OML/cmm/m/it/12 s$ \
OT1/cmr/m/n/12 from the pho-to-cath-ode. The af-ter-pulse timescale
[108] [109] <figures/afterpulse_outer.png, id=2365, 1200.485pt x 875.27pt>
<use figures/afterpulse_outer.png>
<figures/afterpulse_central.png, id=2366, 1200.485pt x 875.27pt>
<use figures/afterpulse_central.png> [110 <./figures/afterpulse_outer.png> <./f
igures/afterpulse_central.png>]) (./Reco.tex
Chapter 4.
[111] <figures/edgestream.png, id=2391, 902.37125pt x 209.78375pt>
<use figures/edgestream.png> [112 <./figures/edgestream.png>] [113] [114]
<figures/LoTOT.png, id=2411, 798.985pt x 574.145pt> <use figures/LoTOT.png>
<figures/HiTOT.png, id=2412, 798.985pt x 574.145pt> <use figures/HiTOT.png>
<figures/T01.png, id=2413, 798.985pt x 574.145pt> <use figures/T01.png>
<figures/T23.png, id=2414, 798.985pt x 574.145pt> <use figures/T23.png>
[115 <./figures/LoTOT.png> <./figures/HiTOT.png> <./figures/T01.png> <./figures
/T23.png>] [116] <figures/SFCF.png, id=2433, 710.655pt x 499.8675pt>
<use figures/SFCF.png> [117 <./figures/SFCF.png>] [118]
<figures/gamma_sim.png, id=2452, 795.97375pt x 533.995pt>
<use figures/gamma_sim.png>
<figures/proton_sim.png, id=2453, 801.99625pt x 533.995pt>
<use figures/proton_sim.png> [119 <./figures/gamma_sim.png> <./figures/proton_s
im.png>] <figures/likely_gamma.png, id=2464, 801.99625pt x 539.01375pt>
<use figures/likely_gamma.png>
<figures/likely_hadron.png, id=2465, 803.0pt x 542.025pt>
<use figures/likely_hadron.png>
Overfull \hbox (9.47742pt too wide) in paragraph at lines 218--229
[][]     [][] 
[120 <./figures/likely_gamma.png> <./figures/likely_hadron.png>] [121]
<figures/curvature_correct.png, id=2486, 718.685pt x 548.0475pt>
<use figures/curvature_correct.png> [122 <./figures/curvature_correct.png>]
<figures/angle_v_energy.png, id=2496, 765.86125pt x 602.25pt>
<use figures/angle_v_energy.png> [123 <./figures/angle_v_energy.png>] [124]
[125]
<figures/SP-invcompact-demo-20160404.png, id=2520, 2849.64626pt x 2269.47874pt>
<use figures/SP-invcompact-demo-20160404.png> [126 <./figures/SP-invcompact-dem
o-20160404.png>]
Overfull \hbox (4.36082pt too wide) in paragraph at lines 375--383
[]\OT1/cmr/m/n/12 The asym-me-tries present in the spa-tial dis-tri-bu-tion of 
shower en-ergy in hadronic
[127] <figures/pinc.png, id=2535, 998.73125pt x 662.475pt>
<use figures/pinc.png> [128 <./figures/pinc.png>]
<figures/SP-pinc-demo-20160404.png, id=2543, 2827.56375pt x 2269.47874pt>
<use figures/SP-pinc-demo-20160404.png> [129 <./figures/SP-pinc-demo-20160404.p
ng>] <figures/Crab_SP_RC0v2.jpg, id=2554, 367.3725pt x 412.54124pt>
<use figures/Crab_SP_RC0v2.jpg>
<figures/crab_excess.png, id=2555, 730.73pt x 692.5875pt>
<use figures/crab_excess.png>) [130] [131 <./figures/Crab_SP_RC0v2.jpg>]
[132 <./figures/crab_excess.png>] (./Method.tex
Chapter 5.
[133] [134] [135] [136]
<figures/exampleskymap.png, id=2597, 800.9925pt x 577.15625pt>
<use figures/exampleskymap.png> [137 <./figures/exampleskymap.png>] [138]
<figures/timediagram_two.png, id=2608, 874.26625pt x 570.13pt>
<use figures/timediagram_two.png> [139 <./figures/timediagram_two.png>]
[140] <figures/exbackground.png, id=2623, 798.985pt x 574.145pt>
<use figures/exbackground.png> [141 <./figures/exbackground.png>] [142]
<figures/poisson_check1.png, id=2638, 800.9925pt x 577.15625pt>
<use figures/poisson_check1.png> [143 <./figures/poisson_check1.png>] [144]
[145] [146] [147]
<figures/backstudy_pgraph_p2sec.png, id=2666, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_p2sec.png>

LaTeX Warning: Float too large for page by 7.41559pt on input line 281.

<figures/backstudy_pgraph_1sec.png, id=2671, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_1sec.png>
<figures/backstudy_pgraph_10sec.png, id=2676, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_10sec.png>

LaTeX Warning: Float too large for page by 9.7489pt on input line 319.

) [148 <./figures/backstudy_pgraph_p2sec.png>] [149 <./figures/backstudy_pgraph
_1sec.png>] [150 <./figures/backstudy_pgraph_10sec.png>] (./Trials.tex [151]
[152] [153] [154] <figures/inde_pdist.png, id=2728, 698.61pt x 875.27pt>
<use figures/inde_pdist.png>
<figures/inde_trials.png, id=2729, 698.61pt x 875.27pt>
<use figures/inde_trials.png> [155 <./figures/inde_pdist.png> <./figures/inde_t
rials.png>] [156] [157] <figures/corr_pdist.png, id=2750, 698.61pt x 875.27pt>
<use figures/corr_pdist.png>
<figures/wtangent.png, id=2751, 698.61pt x 875.27pt>
<use figures/wtangent.png> [158 <./figures/corr_pdist.png> <./figures/wtangent.
png>] [159] <figures/gcumulative_1sec.png, id=2777, 1200.485pt x 875.27pt>
<use figures/gcumulative_1sec.png> [160 <./figures/gcumulative_1sec.png>]
<figures/gcorrection_p2sec.png, id=2783, 1200.485pt x 875.27pt>
<use figures/gcorrection_p2sec.png>
<figures/gcumulative_corr_p2sec.png, id=2784, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_p2sec.png> [161 <./figures/gcorrection_p2sec.png>
 <./figures/gcumulative_corr_p2sec.png>]
<figures/gcorrection_1sec.png, id=2792, 1200.485pt x 875.27pt>
<use figures/gcorrection_1sec.png>
<figures/gcumulative_corr_1sec.png, id=2793, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_1sec.png> [162 <./figures/gcorrection_1sec.png> <
./figures/gcumulative_corr_1sec.png>]
<figures/gcorrection_10sec.png, id=2800, 1200.485pt x 875.27pt>
<use figures/gcorrection_10sec.png>
<figures/gcumulative_corr_10sec.png, id=2801, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_10sec.png> [163 <./figures/gcorrection_10sec.png>
 <./figures/gcumulative_corr_10sec.png>] [164]
<figures/gcorrection_time_p2sec.png, id=2816, 917.4275pt x 754.82pt>
<use figures/gcorrection_time_p2sec.png> [165 <./figures/gcorrection_time_p2sec
.png>] <figures/gcorrection_time_1sec.png, id=2822, 914.41624pt x 747.79375pt>
<use figures/gcorrection_time_1sec.png> [166 <./figures/gcorrection_time_1sec.p
ng>] <figures/gcorrection_time_10sec.png, id=2829, 912.40875pt x 741.77126pt>
<use figures/gcorrection_time_10sec.png> [167 <./figures/gcorrection_time_10sec
.png>] [168]) [169] (./Sensitivity.tex
Chapter 6.
[170] [171] [172] [173]
<figures/psf_geom.png, id=2881, 937.5025pt x 500.87125pt>
<use figures/psf_geom.png> [174 <./figures/psf_geom.png>]
<figures/sens_v_spatial_bin_size.png, id=2889, 1200.485pt x 875.27pt>
<use figures/sens_v_spatial_bin_size.png> [175 <./figures/sens_v_spatial_bin_si
ze.png>] [176] [177] [178] [179]
<figures/sensitivity_v_tophat_radius_bg1000.png, id=2927, 1200.485pt x 875.27pt
> <use figures/sensitivity_v_tophat_radius_bg1000.png> [180 <./figures/sensitiv
ity_v_tophat_radius_bg1000.png>]
<figures/sensitivity_v_tophat_radius_bg_p1.png, id=2932, 1200.485pt x 875.27pt>
<use figures/sensitivity_v_tophat_radius_bg_p1.png> [181 <./figures/sensitivity
_v_tophat_radius_bg_p1.png>] [182] [183] [184] [185] [186]
<figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png, id=2973, 1200.485p
t x 875.27pt> <use figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png>
[187 <./figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png>]
<figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png, id=2980, 1200.485
pt x 875.27pt>
<use figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png> [188 <./figur
es/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png>] [189] [190]
<figures/grb_cuts_near_crab.png, id=3003, 669.50125pt x 563.10374pt>
<use figures/grb_cuts_near_crab.png> [191 <./figures/grb_cuts_near_crab.png>]
[192] [193] <figures/sensitivity_money.png, id=3032, 1200.485pt x 875.27pt>
<use figures/sensitivity_money.png> [194 <./figures/sensitivity_money.png>]
<figures/sensitivity_money_long.png, id=3039, 1200.485pt x 875.27pt>
<use figures/sensitivity_money_long.png> [195 <./figures/sensitivity_money_long
.png>] [196] <figures/bg_corrected_fermi.png, id=3060, 1200.485pt x 875.27pt>
<use figures/bg_corrected_fermi.png>
<figures/grb090510_on_hawc.png, id=3061, 1200.485pt x 875.27pt>
<use figures/grb090510_on_hawc.png> [197 <./figures/bg_corrected_fermi.png>]
[198 <./figures/grb090510_on_hawc.png>] [199] [200] [201] [202]) [203] [204]
(./Results.tex
Chapter 7.
[205] [206] <figures/datapie.png, id=3124, 985.6825pt x 631.35875pt>
<use figures/datapie.png> [207 <./figures/datapie.png>] [208] [209]
<figures/rate1_zoom.png, id=3152, 798.985pt x 574.145pt>
<use figures/rate1_zoom.png> [210 <./figures/rate1_zoom.png>]
<figures/inlay.png, id=3158, 987.69pt x 716.6775pt> <use figures/inlay.png>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 159--161
 [] 
[211 <./figures/inlay.png>]
<figures/candidate_lightcurve.png, id=3164, 899.36pt x 574.145pt>
<use figures/candidate_lightcurve.png> [212 <./figures/candidate_lightcurve.png
>] <figures/lc_coarse.png, id=3171, 798.985pt x 574.145pt>
<use figures/lc_coarse.png> [213 <./figures/lc_coarse.png>]
<figures/candidate_location_full_skymap.png, id=3177, 433.62pt x 487.8225pt>
<use figures/candidate_location_full_skymap.png>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 208--210
 [] 
[214 <./figures/candidate_location_full_skymap.png>] [215] [216] [217] [218]
<figures/limit_grbrate.png, id=3217, 1200.485pt x 875.27pt>
<use figures/limit_grbrate.png> [219 <./figures/limit_grbrate.png>]
<figures/grbrate_long.png, id=3224, 1200.485pt x 875.27pt>
<use figures/grbrate_long.png> [220 <./figures/grbrate_long.png>] [221])
[222] (./AppendixC.tex
Appendix A.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\Gamma' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `subscript' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 5.

[223] [224]) [225] (./AppendixB.tex
Appendix B.
[226] [227]) [228] (./AppendixD.tex
Appendix C.
<figures/analog_input_circuit.png, id=3308, 310.15875pt x 229.85875pt>
<use figures/analog_input_circuit.png> [229 <./figures/analog_input_circuit.png
>]) [230] (./AppendixE.tex
Appendix D.
<figures/analog_load_circuit.png, id=3324, 845.1575pt x 345.29pt>
<use figures/analog_load_circuit.png> [231 <./figures/analog_load_circuit.png>]
) [232] (./AppendixF.tex
Appendix E.
<figures/milagro_pmt_base_via_bob_28nov11.pdf, id=3347, 614.295pt x 794.97pt>
<use figures/milagro_pmt_base_via_bob_28nov11.pdf>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 37--38
 [] 
) [233]

LaTeX Warning: Text page 234 contains only floats.

[234 <./figures/milagro_pmt_base_via_bob_28nov11.pdf>] (./thesis.bbl
Underfull \hbox (badness 2213) in paragraph at lines 64--67
[]\OT1/cmr/m/n/12 M. Briggs.  Gamma-Ray As-tro-physics NSSTC BATSE GRB.  \OT1/c
mr/m/it/12 URL
[235]
Underfull \hbox (badness 3407) in paragraph at lines 96--99
[]\OT1/cmr/m/n/12 S. et al. Woose-ley.  The Su-per-nova Gamma-ray Burst Con-nec
-tion.
[236] [237] [238]
Underfull \hbox (badness 3439) in paragraph at lines 429--434
[]\OT1/cmr/m/n/12 E. Fer-rara.  Caveats About An-a-lyz-ing LAT Pass 8 Data.  \O
T1/cmr/m/it/12 URL

Underfull \hbox (badness 10000) in paragraph at lines 436--441
[]\OT1/cmr/m/n/12 Fermi LAT Col-lab-o-ra-tion.  Fermi LAT GRBs.  \OT1/cmr/m/it/
12 URL
[239]
Underfull \hbox (badness 10000) in paragraph at lines 443--447
[]\OT1/cmr/m/n/12 S. No-bili.  GRB 130427A: A CHANCE NOT TO MISS.
) [240] (./thesis.aux (./Abstract.aux) (./Titlepage.aux) (./Copyright.aux)
(./Abbreviations.aux) (./GRBs.aux) (./Showers.aux) (./HAWC.aux) (./Reco.aux)
(./Method.aux) (./Trials.aux) (./Sensitivity.aux) (./Results.aux)
(./AppendixC.aux) (./AppendixB.aux) (./AppendixD.aux) (./AppendixE.aux)
(./AppendixF.aux))

LaTeX Warning: There were multiply-defined labels.

 )
(see the transcript file for additional information)</usr/local/texlive/2015/te
xmf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2015/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2015/texm
f-dist/fonts/type1/public/amsfonts/cm/cmmi12.pfb></usr/local/texlive/2015/texmf
-dist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2015/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmmi8.pfb></usr/local/texlive/2015/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2015/texmf-dist/
fonts/type1/public/amsfonts/cm/cmr12.pfb></usr/local/texlive/2015/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmr6.pfb></usr/local/texlive/2015/texmf-dist/fonts
/type1/public/amsfonts/cm/cmr8.pfb></usr/local/texlive/2015/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2015/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmsy6.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1
/public/amsfonts/cm/cmsy8.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmti12.pfb>
Output written on thesis.pdf (267 pages, 9013150 bytes).
Transcript written on thesis.log.


==> logit_v2 <==
pdflatex thesis
This is pdfTeX, Version 3.14159265-2.6-1.40.16 (TeX Live 2015) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./thesis.tex
LaTeX2e <2015/01/01>
Babel <3.9l> and hyphenation patterns for 79 languages loaded.
(./thesis.cls
Document Class: thesis 2006/04/26 v0.1
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/size12.clo))
(./styles/titlesec.sty

LaTeX Warning: You have requested package `styles/titlesec',
               but the package provides `titlesec'.

) (/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/graphics.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/pdftex-def/pdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/lscape.sty)
(./styles/indentfirst.sty

LaTeX Warning: You have requested package `styles/indentfirst',
               but the package provides `indentfirst'.

) (./styles/latexsym.sty

LaTeX Warning: You have requested package `styles/latexsym',
               but the package provides `latexsym'.

) (./styles/multirow.sty) (./styles/tabls.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(./styles/slashbox.sty
slashbox style by K.Yasuoka, May 1993.
) (/usr/local/texlive/2015/texmf-dist/tex/latex/tools/longtable.sty)
(./styles/supertabular.sty

LaTeX Warning: You have requested package `styles/supertabular',
               but the package provides `supertabular'.

) (/usr/local/texlive/2015/texmf-dist/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/local/texlive/2015/texmf-dist/tex/latex/subfigure/subfigure.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2015/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/url/url.sty))

Package hyperref Message: Driver: hpdftex.

(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/lineno/lineno.sty) (./thesis.aux
(./Abstract.aux) (./Titlepage.aux) (./Copyright.aux) (./Abbreviations.aux)
(./GRBs.aux) (./Showers.aux) (./HAWC.aux) (./Reco.aux) (./Method.aux)
(./Trials.aux) (./Sensitivity.aux) (./Results.aux) (./AppendixC.aux)
(./AppendixB.aux) (./AppendixD.aux) (./AppendixE.aux) (./AppendixF.aux))
(/usr/local/texlive/2015/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/color.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./thesis.out) (./thesis.out) (./Abstract.tex
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/ulasy.fd)) [1{/usr/local/tex
live/2015/texmf-var/fonts/map/pdftex/updmap/pdftex.map}] [2] (./Titlepage.tex)
[3] (./Copyright.tex
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/omscmr.fd)) [4]
(./thesis.toc [2] [3]) [4] (./thesis.lof
Overfull \hbox (14.12067pt too wide) in paragraph at lines 3--3
 [][] [][][]\OT1/cmr/m/n/12 Twelve light curves for mea-sured BATSE GRBs [[][]2
[][]]. The short timescales 
[5]
Overfull \hbox (18.10568pt too wide) in paragraph at lines 15--15
 \OT1/cmr/m/n/12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 03\OML/cmm/m/it/12 ; \OT1/c
mr/m/n/12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 25\OML/cmm/m/it/12 ; \OT1/cmr/m/n/
12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 5\OML/cmm/m/it/12 ; \OT1/cmr/m/n/12 1\OML
/cmm/m/it/12 :\OT1/cmr/m/n/12 0$ for the WMAP5 Fidu-cial (solid black), WMAP5+F
ixed 
[6] [7] [8] [9] [10] [11] [12]
Overfull \hbox (0.82274pt too wide) in paragraph at lines 59--59
 \OT1/cmr/m/n/12 cles (NKG) and elec-tro-mag-netic shower en-ergy (NKG/R) in a 
gamma- 
[13] [14] [15] [16] [17] [18] [19] [20] [21] [22]) [23] (./Abbreviations.tex)
[24] (./GRBs.tex
Chapter 1.
pdfTeX warning (ext4): destination with the same identifier (name{page.1}) has 
been already used, duplicate ignored
<to be read again> 
                   \relax 
l.26 
      [1]pdfTeX warning (ext4): destination with the same identifier (name{page
.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.49 
      [2]pdfTeX warning (ext4): destination with the same identifier (name{page
.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.73 \newpage
              [3]pdfTeX warning (ext4): destination with the same identifier (n
ame{page.4}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.88 \newpage
              [4] [5] <figures/batse_t90.png, id=1463, 931.48pt x 692.5875pt>
<use figures/batse_t90.png> [6 <./figures/batse_t90.png>]
<figures/batse_panel.png, id=1472, 923.45pt x 911.405pt>
<use figures/batse_panel.png> [7 <./figures/batse_panel.png>] [8]
<figures/bandfuncfig.pdf, id=1494, 612.09195pt x 615.50294pt>
<use figures/bandfuncfig.pdf> [9 <./figures/bandfuncfig.pdf>]
<figures/batse_spatial.png, id=1513, 980.66376pt x 706.64pt>
<use figures/batse_spatial.png> [10 <./figures/batse_spatial.png>] [11]
<figures/jetbreak.png, id=1530, 619.31375pt x 478.78876pt>
<use figures/jetbreak.png> [12 <./figures/jetbreak.png>] [13]
<figures/redshift.png, id=1557, 1025.8325pt x 832.10875pt>
<use figures/redshift.png> [14 <./figures/redshift.png>] [15]
<figures/fluenceratio.png, id=1580, 706.64pt x 689.57625pt>
<use figures/fluenceratio.png> [16 <./figures/fluenceratio.png>] [17]
<figures/fermicutoff.png, id=1596, 960.58875pt x 728.7225pt>
<use figures/fermicutoff.png> [18 <./figures/fermicutoff.png>] [19]
<figures/hess_scheme.jpg, id=1617, 413.545pt x 385.44pt>
<use figures/hess_scheme.jpg>
<figures/wct.jpg, id=1618, 602.25pt x 615.29875pt> <use figures/wct.jpg>
[20 <./figures/hess_scheme.jpg> <./figures/wct.jpg>] [21] [22]
<figures/EffArea.png, id=1651, 734.9859pt x 445.9059pt>
<use figures/EffArea.png> [23 <./figures/EffArea.png>] [24]
<figures/fireballmodel.png, id=1670, 1154.3125pt x 899.36pt>
<use figures/fireballmodel.png> [25 <./figures/fireballmodel.png>] [26]
[27] [28] [29] [30]
<figures/short_grb_cutoff.png, id=1732, 800.9925pt x 677.53125pt>
<use figures/short_grb_cutoff.png> [31 <./figures/short_grb_cutoff.png>]
[32] <figures/ebl_flux.png, id=1751, 1090.0725pt x 921.4425pt>
<use figures/ebl_flux.png> [33 <./figures/ebl_flux.png>]
<figures/gilmore_2012_EBL_atten.png, id=1766, 667.49374pt x 649.42625pt>
<use figures/gilmore_2012_EBL_atten.png> [34 <./figures/gilmore_2012_EBL_atten.
png>] [35]) [36] (./Showers.tex
Chapter 2.
[37] [38]
Overfull \hbox (12.82234pt too wide) in paragraph at lines 36--41
\OT1/cmr/m/n/12 The elec-tron and positron pair sub-se-quently gen-er-ate more 
pho-tons via Bremsstrahlung
[39] <figures/gamma_shower_model.png, id=1814, 650.43pt x 502.87875pt>
<use figures/gamma_shower_model.png> [40] [41 <./figures/gamma_shower_model.png
>] <figures/gamma_shower_profile.png, id=1832, 1200.485pt x 875.27pt>
<use figures/gamma_shower_profile.png> [42 <./figures/gamma_shower_profile.png>
] [43] <figures/eas_diagram.png, id=1855, 410.53375pt x 658.46pt>
<use figures/eas_diagram.png> [44] [45 <./figures/eas_diagram.png>] [46]
<figures/proton_shower_profile.png, id=1879, 1200.485pt x 875.27pt>
<use figures/proton_shower_profile.png> [47 <./figures/proton_shower_profile.pn
g>] <figures/proton_particle_number.png, id=1886, 634.37pt x 718.685pt>
<use figures/proton_particle_number.png> [48 <./figures/proton_particle_number.
png>] [49] <figures/shower_timing.png, id=1903, 562.1pt x 628.3475pt>
<use figures/shower_timing.png> [50 <./figures/shower_timing.png>]
<figures/side_shower.png, id=1914, 608.2725pt x 744.7825pt>
<use figures/side_shower.png>) [51] [52 <./figures/side_shower.png>]
(./HAWC.tex
Chapter 3.
[53] <figures/HAWC_overview.jpeg, id=1933, 1080.035pt x 725.71124pt>
<use figures/HAWC_overview.jpeg> [54 <./figures/HAWC_overview.jpeg>] [55]
<figures/HAWC_tank.png, id=1944, 839.135pt x 688.5725pt>
<use figures/HAWC_tank.png>
<figures/HAWC_bladder.png, id=1945, 182.1204pt x 168.63pt>
<use figures/HAWC_bladder.png> [56 <./figures/HAWC_tank.png> <./figures/HAWC_bl
adder.png>] [57] <figures/regularpulse.png, id=1957, 520.94624pt x 706.64pt>
<use figures/regularpulse.png>
<figures/HAWC_pmt.png, id=1958, 171.039pt x 227.8914pt>
<use figures/HAWC_pmt.png> [58 <./figures/regularpulse.png> <./figures/HAWC_pmt
.png>] [59] <figures/single_pe_charge.jpeg, id=1975, 990.70125pt x 736.7525pt>
<use figures/single_pe_charge.jpeg> [60 <./figures/single_pe_charge.jpeg>]
[61] <figures/r5912_quantum_efficiency.png, id=1987, 610.28pt x 664.4825pt>
<use figures/r5912_quantum_efficiency.png>
<figures/r7081_HQE_quantum_efficiency.png, id=1988, 546.04pt x 696.6025pt>
<use figures/r7081_HQE_quantum_efficiency.png> [62 <./figures/r5912_quantum_eff
iciency.png> <./figures/r7081_HQE_quantum_efficiency.png>] [63]
<figures/signal_overview.png, id=2003, 914.41624pt x 311.1625pt>
<use figures/signal_overview.png> [64 <./figures/signal_overview.png>] [65]
<figures/coax_diagram.png, id=2016, 484.81125pt x 483.8075pt>
<use figures/coax_diagram.png> [66 <./figures/coax_diagram.png>]
<figures/circuit.png, id=2031, 860.21375pt x 442.65375pt>
<use figures/circuit.png> [67 <./figures/circuit.png>] [68] [69]
<figures/comp_cable.png, id=2059, 1200.485pt x 875.27pt>
<use figures/comp_cable.png> [70 <./figures/comp_cable.png>]
<figures/analog_circuit.png, id=2067, 1186.4325pt x 665.48625pt>
<use figures/analog_circuit.png> [71 <./figures/analog_circuit.png>] [72]
[73] [74] <figures/AnalogFEB_4edge.png, id=2097, 1202.4925pt x 878.28125pt>
<use figures/AnalogFEB_4edge.png> [75 <./figures/AnalogFEB_4edge.png>]
<figures/AnalogFEB_2edge.png, id=2107, 1202.4925pt x 878.28125pt>
<use figures/AnalogFEB_2edge.png> [76 <./figures/AnalogFEB_2edge.png>]
<figures/digital_logic.png, id=2115, 968.61874pt x 628.3475pt>
<use figures/digital_logic.png> [77 <./figures/digital_logic.png>]
<figures/latch_circuit.png, id=2124, 894.34125pt x 481.8pt>
<use figures/latch_circuit.png> [78 <./figures/latch_circuit.png>]
<figures/flip_flop_logic.png, id=2130, 352.31625pt x 269.005pt>
<use figures/flip_flop_logic.png>
<figures/logic_table.png, id=2131, 666.49pt x 470.75874pt>
<use figures/logic_table.png> [79 <./figures/flip_flop_logic.png> <./figures/lo
gic_table.png>]
<figures/flip_flop_20ns.png, id=2141, 700.6175pt x 476.78125pt>
<use figures/flip_flop_20ns.png> [80 <./figures/flip_flop_20ns.png>]
<figures/one-shot_width_vs_R.png, id=2146, 901.3675pt x 777.90625pt>
<use figures/one-shot_width_vs_R.png> [81 <./figures/one-shot_width_vs_R.png>]
[82] <figures/delay_circuit.png, id=2158, 697.60625pt x 202.7575pt>
<use figures/delay_circuit.png> [83 <./figures/delay_circuit.png>] [84]
<figures/DigitalFEB_4edge.png, id=2176, 1202.4925pt x 426.59375pt>
<use figures/DigitalFEB_4edge.png>
Overfull \hbox (43.36244pt too wide) in paragraph at lines 595--596
 [] 
[85 <./figures/DigitalFEB_4edge.png>] [86]
<figures/DigitalFEB_2edge.png, id=2195, 1202.4925pt x 426.59375pt>
<use figures/DigitalFEB_2edge.png>
Overfull \hbox (43.36244pt too wide) in paragraph at lines 638--639
 [] 
[87 <./figures/DigitalFEB_2edge.png>] [88] [89]
<figures/early_TDC_event.png, id=2218, 855.195pt x 610.28pt>
<use figures/early_TDC_event.png> [90 <./figures/early_TDC_event.png>] [91]
<figures/online_reco_chain.png, id=2233, 1038.88126pt x 591.20876pt>
<use figures/online_reco_chain.png> [92 <./figures/online_reco_chain.png>]
<figures/timediagram.png, id=2240, 1013.7875pt x 633.36626pt>
<use figures/timediagram.png> [93 <./figures/timediagram.png>] [94]
<figures/OnlineLatencyBigBins.png, id=2254, 922.44624pt x 617.30624pt>
<use figures/OnlineLatencyBigBins.png> [95 <./figures/OnlineLatencyBigBins.png>
] [96]
<figures/Calibration_Simplified_Layout.png, id=2269, 794.4882pt x 654.2844pt>
<use figures/Calibration_Simplified_Layout.png> [97 <./figures/Calibration_Simp
lified_Layout.png>]
<figures/chargecalib_curves_run5213_H13.png, id=2274, 1367.1075pt x 701.62125pt
> <use figures/chargecalib_curves_run5213_H13.png> [98 <./figures/chargecalib_c
urves_run5213_H13.png>]
<figures/H13_slewing.png, id=2280, 999.735pt x 774.895pt>
<use figures/H13_slewing.png> [99 <./figures/H13_slewing.png>] [100] [101]
[102] [103] <figures/10inch_lostart.png, id=2321, 800.9925pt x 577.15625pt>
<use figures/10inch_lostart.png>
<figures/10inch_histart.png, id=2322, 798.985pt x 574.145pt>
<use figures/10inch_histart.png> [104 <./figures/10inch_lostart.png> <./figures
/10inch_histart.png>]
<figures/8inch_lostart.png, id=2329, 798.985pt x 574.145pt>
<use figures/8inch_lostart.png>
<figures/8inch_histart.png, id=2330, 798.985pt x 574.145pt>
<use figures/8inch_histart.png> [105 <./figures/8inch_lostart.png> <./figures/8
inch_histart.png>] [106]
<figures/afterpulsing_rate.png, id=2345, 937.5025pt x 669.50125pt>
<use figures/afterpulsing_rate.png> [107 <./figures/afterpulsing_rate.png>]
Overfull \hbox (0.59285pt too wide) in paragraph at lines 970--974
\OT1/cmr/m/n/12 for ion-iza-tion oc-cur-ring a dis-tance $\OML/cmm/m/it/12 s$ \
OT1/cmr/m/n/12 from the pho-to-cath-ode. The af-ter-pulse timescale
[108] [109] <figures/afterpulse_outer.png, id=2365, 1200.485pt x 875.27pt>
<use figures/afterpulse_outer.png>
<figures/afterpulse_central.png, id=2366, 1200.485pt x 875.27pt>
<use figures/afterpulse_central.png> [110 <./figures/afterpulse_outer.png> <./f
igures/afterpulse_central.png>]) (./Reco.tex
Chapter 4.
[111] <figures/edgestream.png, id=2391, 902.37125pt x 209.78375pt>
<use figures/edgestream.png> [112 <./figures/edgestream.png>] [113] [114]
<figures/LoTOT.png, id=2411, 798.985pt x 574.145pt> <use figures/LoTOT.png>
<figures/HiTOT.png, id=2412, 798.985pt x 574.145pt> <use figures/HiTOT.png>
<figures/T01.png, id=2413, 798.985pt x 574.145pt> <use figures/T01.png>
<figures/T23.png, id=2414, 798.985pt x 574.145pt> <use figures/T23.png>
[115 <./figures/LoTOT.png> <./figures/HiTOT.png> <./figures/T01.png> <./figures
/T23.png>] [116] <figures/SFCF.png, id=2433, 710.655pt x 499.8675pt>
<use figures/SFCF.png> [117 <./figures/SFCF.png>] [118]
<figures/gamma_sim.png, id=2452, 795.97375pt x 533.995pt>
<use figures/gamma_sim.png>
<figures/proton_sim.png, id=2453, 801.99625pt x 533.995pt>
<use figures/proton_sim.png> [119 <./figures/gamma_sim.png> <./figures/proton_s
im.png>] <figures/likely_gamma.png, id=2464, 801.99625pt x 539.01375pt>
<use figures/likely_gamma.png>
<figures/likely_hadron.png, id=2465, 803.0pt x 542.025pt>
<use figures/likely_hadron.png>
Overfull \hbox (9.47742pt too wide) in paragraph at lines 218--229
[][]     [][] 
[120 <./figures/likely_gamma.png> <./figures/likely_hadron.png>] [121]
<figures/curvature_correct.png, id=2486, 718.685pt x 548.0475pt>
<use figures/curvature_correct.png> [122 <./figures/curvature_correct.png>]
<figures/angle_v_energy.png, id=2496, 765.86125pt x 602.25pt>
<use figures/angle_v_energy.png> [123 <./figures/angle_v_energy.png>] [124]
[125]
<figures/SP-invcompact-demo-20160404.png, id=2520, 2849.64626pt x 2269.47874pt>
<use figures/SP-invcompact-demo-20160404.png> [126 <./figures/SP-invcompact-dem
o-20160404.png>]
Overfull \hbox (4.36082pt too wide) in paragraph at lines 375--383
[]\OT1/cmr/m/n/12 The asym-me-tries present in the spa-tial dis-tri-bu-tion of 
shower en-ergy in hadronic
[127] <figures/pinc.png, id=2535, 998.73125pt x 662.475pt>
<use figures/pinc.png> [128 <./figures/pinc.png>]
<figures/SP-pinc-demo-20160404.png, id=2543, 2827.56375pt x 2269.47874pt>
<use figures/SP-pinc-demo-20160404.png> [129 <./figures/SP-pinc-demo-20160404.p
ng>] <figures/Crab_SP_RC0v2.jpg, id=2554, 367.3725pt x 412.54124pt>
<use figures/Crab_SP_RC0v2.jpg>
<figures/crab_excess.png, id=2555, 730.73pt x 692.5875pt>
<use figures/crab_excess.png>) [130] [131 <./figures/Crab_SP_RC0v2.jpg>]
[132 <./figures/crab_excess.png>] (./Method.tex
Chapter 5.
[133] [134] [135] [136]
<figures/exampleskymap.png, id=2597, 800.9925pt x 577.15625pt>
<use figures/exampleskymap.png> [137 <./figures/exampleskymap.png>] [138]
<figures/timediagram_two.png, id=2608, 874.26625pt x 570.13pt>
<use figures/timediagram_two.png> [139 <./figures/timediagram_two.png>]
[140] <figures/exbackground.png, id=2623, 798.985pt x 574.145pt>
<use figures/exbackground.png> [141 <./figures/exbackground.png>] [142]
<figures/poisson_check1.png, id=2638, 800.9925pt x 577.15625pt>
<use figures/poisson_check1.png> [143 <./figures/poisson_check1.png>] [144]
[145] [146] [147]
<figures/backstudy_pgraph_p2sec.png, id=2666, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_p2sec.png>

LaTeX Warning: Float too large for page by 7.41559pt on input line 281.

<figures/backstudy_pgraph_1sec.png, id=2671, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_1sec.png>
<figures/backstudy_pgraph_10sec.png, id=2676, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_10sec.png>

LaTeX Warning: Float too large for page by 9.7489pt on input line 319.

) [148 <./figures/backstudy_pgraph_p2sec.png>] [149 <./figures/backstudy_pgraph
_1sec.png>] [150 <./figures/backstudy_pgraph_10sec.png>] (./Trials.tex [151]
[152] [153] [154] <figures/inde_pdist.png, id=2728, 698.61pt x 875.27pt>
<use figures/inde_pdist.png>
<figures/inde_trials.png, id=2729, 698.61pt x 875.27pt>
<use figures/inde_trials.png> [155 <./figures/inde_pdist.png> <./figures/inde_t
rials.png>] [156] [157] <figures/corr_pdist.png, id=2750, 698.61pt x 875.27pt>
<use figures/corr_pdist.png>
<figures/wtangent.png, id=2751, 698.61pt x 875.27pt>
<use figures/wtangent.png> [158 <./figures/corr_pdist.png> <./figures/wtangent.
png>] [159] <figures/gcumulative_1sec.png, id=2777, 1200.485pt x 875.27pt>
<use figures/gcumulative_1sec.png> [160 <./figures/gcumulative_1sec.png>]
<figures/gcorrection_p2sec.png, id=2783, 1200.485pt x 875.27pt>
<use figures/gcorrection_p2sec.png>
<figures/gcumulative_corr_p2sec.png, id=2784, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_p2sec.png> [161 <./figures/gcorrection_p2sec.png>
 <./figures/gcumulative_corr_p2sec.png>]
<figures/gcorrection_1sec.png, id=2792, 1200.485pt x 875.27pt>
<use figures/gcorrection_1sec.png>
<figures/gcumulative_corr_1sec.png, id=2793, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_1sec.png> [162 <./figures/gcorrection_1sec.png> <
./figures/gcumulative_corr_1sec.png>]
<figures/gcorrection_10sec.png, id=2800, 1200.485pt x 875.27pt>
<use figures/gcorrection_10sec.png>
<figures/gcumulative_corr_10sec.png, id=2801, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_10sec.png> [163 <./figures/gcorrection_10sec.png>
 <./figures/gcumulative_corr_10sec.png>] [164]
<figures/gcorrection_time_p2sec.png, id=2816, 917.4275pt x 754.82pt>
<use figures/gcorrection_time_p2sec.png> [165 <./figures/gcorrection_time_p2sec
.png>] <figures/gcorrection_time_1sec.png, id=2822, 914.41624pt x 747.79375pt>
<use figures/gcorrection_time_1sec.png> [166 <./figures/gcorrection_time_1sec.p
ng>] <figures/gcorrection_time_10sec.png, id=2829, 912.40875pt x 741.77126pt>
<use figures/gcorrection_time_10sec.png> [167 <./figures/gcorrection_time_10sec
.png>] [168]) [169] (./Sensitivity.tex
Chapter 6.
[170] [171] [172] [173]
<figures/psf_geom.png, id=2881, 937.5025pt x 500.87125pt>
<use figures/psf_geom.png> [174 <./figures/psf_geom.png>]
<figures/sens_v_spatial_bin_size.png, id=2889, 1200.485pt x 875.27pt>
<use figures/sens_v_spatial_bin_size.png> [175 <./figures/sens_v_spatial_bin_si
ze.png>] [176] [177] [178] [179]
<figures/sensitivity_v_tophat_radius_bg1000.png, id=2927, 1200.485pt x 875.27pt
> <use figures/sensitivity_v_tophat_radius_bg1000.png> [180 <./figures/sensitiv
ity_v_tophat_radius_bg1000.png>]
<figures/sensitivity_v_tophat_radius_bg_p1.png, id=2932, 1200.485pt x 875.27pt>
<use figures/sensitivity_v_tophat_radius_bg_p1.png> [181 <./figures/sensitivity
_v_tophat_radius_bg_p1.png>] [182] [183] [184] [185] [186]
<figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png, id=2973, 1200.485p
t x 875.27pt> <use figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png>
[187 <./figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png>]
<figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png, id=2980, 1200.485
pt x 875.27pt>
<use figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png> [188 <./figur
es/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png>] [189] [190]
<figures/grb_cuts_near_crab.png, id=3003, 669.50125pt x 563.10374pt>
<use figures/grb_cuts_near_crab.png> [191 <./figures/grb_cuts_near_crab.png>]
[192] [193] <figures/sensitivity_money.png, id=3032, 1200.485pt x 875.27pt>
<use figures/sensitivity_money.png> [194 <./figures/sensitivity_money.png>]
<figures/sensitivity_money_long.png, id=3039, 1200.485pt x 875.27pt>
<use figures/sensitivity_money_long.png> [195 <./figures/sensitivity_money_long
.png>] [196] <figures/bg_corrected_fermi.png, id=3060, 1200.485pt x 875.27pt>
<use figures/bg_corrected_fermi.png>
<figures/grb090510_on_hawc.png, id=3061, 1200.485pt x 875.27pt>
<use figures/grb090510_on_hawc.png> [197 <./figures/bg_corrected_fermi.png>]
[198 <./figures/grb090510_on_hawc.png>] [199] [200] [201] [202]) [203] [204]
(./Results.tex
Chapter 7.
[205] [206] <figures/datapie.png, id=3124, 985.6825pt x 631.35875pt>
<use figures/datapie.png> [207 <./figures/datapie.png>] [208] [209]
<figures/rate1_zoom.png, id=3152, 798.985pt x 574.145pt>
<use figures/rate1_zoom.png> [210 <./figures/rate1_zoom.png>]
<figures/inlay.png, id=3158, 987.69pt x 716.6775pt> <use figures/inlay.png>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 159--161
 [] 
[211 <./figures/inlay.png>]
<figures/candidate_lightcurve.png, id=3164, 899.36pt x 574.145pt>
<use figures/candidate_lightcurve.png> [212 <./figures/candidate_lightcurve.png
>] <figures/lc_coarse.png, id=3171, 798.985pt x 574.145pt>
<use figures/lc_coarse.png> [213 <./figures/lc_coarse.png>]
<figures/candidate_location_full_skymap.png, id=3177, 433.62pt x 487.8225pt>
<use figures/candidate_location_full_skymap.png>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 208--210
 [] 
[214 <./figures/candidate_location_full_skymap.png>] [215] [216] [217] [218]
<figures/limit_grbrate.png, id=3217, 1200.485pt x 875.27pt>
<use figures/limit_grbrate.png> [219 <./figures/limit_grbrate.png>]
<figures/grbrate_long.png, id=3224, 1200.485pt x 875.27pt>
<use figures/grbrate_long.png> [220 <./figures/grbrate_long.png>] [221])
[222] (./AppendixC.tex
Appendix A.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\Gamma' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `subscript' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 5.

[223] [224]) [225] (./AppendixB.tex
Appendix B.
[226] [227]) [228] (./AppendixD.tex
Appendix C.
<figures/analog_input_circuit.png, id=3308, 310.15875pt x 229.85875pt>
<use figures/analog_input_circuit.png> [229 <./figures/analog_input_circuit.png
>]) [230] (./AppendixE.tex
Appendix D.
<figures/analog_load_circuit.png, id=3324, 845.1575pt x 345.29pt>
<use figures/analog_load_circuit.png> [231 <./figures/analog_load_circuit.png>]
) [232] (./AppendixF.tex
Appendix E.
<figures/milagro_pmt_base_via_bob_28nov11.pdf, id=3347, 614.295pt x 794.97pt>
<use figures/milagro_pmt_base_via_bob_28nov11.pdf>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 37--38
 [] 
) [233]

LaTeX Warning: Text page 234 contains only floats.

[234 <./figures/milagro_pmt_base_via_bob_28nov11.pdf>] (./thesis.bbl
Underfull \hbox (badness 2213) in paragraph at lines 19--22
[]\OT1/cmr/m/n/12 M. Briggs.  Gamma-Ray As-tro-physics NSSTC BATSE GRB.  \OT1/c
mr/m/it/12 URL
[235]
Underfull \hbox (badness 3407) in paragraph at lines 139--142
[]\OT1/cmr/m/n/12 S. et al. Woose-ley.  The Su-per-nova Gamma-ray Burst Con-nec
-tion.
[236] [237] [238]
Underfull \hbox (badness 3439) in paragraph at lines 429--434
[]\OT1/cmr/m/n/12 E. Fer-rara.  Caveats About An-a-lyz-ing LAT Pass 8 Data.  \O
T1/cmr/m/it/12 URL

Underfull \hbox (badness 10000) in paragraph at lines 436--441
[]\OT1/cmr/m/n/12 Fermi LAT Col-lab-o-ra-tion.  Fermi LAT GRBs.  \OT1/cmr/m/it/
12 URL

Underfull \hbox (badness 10000) in paragraph at lines 443--447
[]\OT1/cmr/m/n/12 S. No-bili.  GRB 130427A: A CHANCE NOT TO MISS.
[239]) [240] (./thesis.aux (./Abstract.aux) (./Titlepage.aux) (./Copyright.aux)
 (./Abbreviations.aux) (./GRBs.aux) (./Showers.aux) (./HAWC.aux) (./Reco.aux)
(./Method.aux) (./Trials.aux) (./Sensitivity.aux) (./Results.aux)
(./AppendixC.aux) (./AppendixB.aux) (./AppendixD.aux) (./AppendixE.aux)
(./AppendixF.aux)) )
(see the transcript file for additional information)</usr/local/texlive/2015/te
xmf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2015/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2015/texm
f-dist/fonts/type1/public/amsfonts/cm/cmmi12.pfb></usr/local/texlive/2015/texmf
-dist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2015/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmmi8.pfb></usr/local/texlive/2015/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2015/texmf-dist/
fonts/type1/public/amsfonts/cm/cmr12.pfb></usr/local/texlive/2015/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmr6.pfb></usr/local/texlive/2015/texmf-dist/fonts
/type1/public/amsfonts/cm/cmr8.pfb></usr/local/texlive/2015/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2015/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmsy6.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1
/public/amsfonts/cm/cmsy8.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmti12.pfb>
Output written on thesis.pdf (267 pages, 9013216 bytes).
Transcript written on thesis.log.
bibtex thesis
This is BibTeX, Version 0.99d (TeX Live 2015)
The top-level auxiliary file: thesis.aux
A level-1 auxiliary file: Abstract.aux
A level-1 auxiliary file: Titlepage.aux
A level-1 auxiliary file: Copyright.aux
A level-1 auxiliary file: Abbreviations.aux
A level-1 auxiliary file: GRBs.aux
A level-1 auxiliary file: Showers.aux
A level-1 auxiliary file: HAWC.aux
A level-1 auxiliary file: Reco.aux
A level-1 auxiliary file: Method.aux
A level-1 auxiliary file: Trials.aux
A level-1 auxiliary file: Sensitivity.aux
A level-1 auxiliary file: Results.aux
A level-1 auxiliary file: AppendixC.aux
A level-1 auxiliary file: AppendixB.aux
A level-1 auxiliary file: AppendixD.aux
A level-1 auxiliary file: AppendixE.aux
A level-1 auxiliary file: AppendixF.aux
The style file: unsrt.bst
Database file #1: Bibliography.bib
Warning--empty journal in Zhu:2013ufa
Warning--empty journal in DCHOOZ2011
Warning--empty author in GEANT4:2016
(There were 3 warnings)
pdflatex thesis
This is pdfTeX, Version 3.14159265-2.6-1.40.16 (TeX Live 2015) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./thesis.tex
LaTeX2e <2015/01/01>
Babel <3.9l> and hyphenation patterns for 79 languages loaded.
(./thesis.cls
Document Class: thesis 2006/04/26 v0.1
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/size12.clo))
(./styles/titlesec.sty

LaTeX Warning: You have requested package `styles/titlesec',
               but the package provides `titlesec'.

) (/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/graphics.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/pdftex-def/pdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/lscape.sty)
(./styles/indentfirst.sty

LaTeX Warning: You have requested package `styles/indentfirst',
               but the package provides `indentfirst'.

) (./styles/latexsym.sty

LaTeX Warning: You have requested package `styles/latexsym',
               but the package provides `latexsym'.

) (./styles/multirow.sty) (./styles/tabls.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(./styles/slashbox.sty
slashbox style by K.Yasuoka, May 1993.
) (/usr/local/texlive/2015/texmf-dist/tex/latex/tools/longtable.sty)
(./styles/supertabular.sty

LaTeX Warning: You have requested package `styles/supertabular',
               but the package provides `supertabular'.

) (/usr/local/texlive/2015/texmf-dist/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/local/texlive/2015/texmf-dist/tex/latex/subfigure/subfigure.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2015/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/url/url.sty))

Package hyperref Message: Driver: hpdftex.

(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/lineno/lineno.sty) (./thesis.aux
(./Abstract.aux) (./Titlepage.aux) (./Copyright.aux) (./Abbreviations.aux)
(./GRBs.aux) (./Showers.aux) (./HAWC.aux) (./Reco.aux) (./Method.aux)
(./Trials.aux) (./Sensitivity.aux) (./Results.aux) (./AppendixC.aux)
(./AppendixB.aux) (./AppendixD.aux) (./AppendixE.aux) (./AppendixF.aux))
(/usr/local/texlive/2015/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/color.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./thesis.out) (./thesis.out) (./Abstract.tex
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/ulasy.fd)) [1{/usr/local/tex
live/2015/texmf-var/fonts/map/pdftex/updmap/pdftex.map}] [2] (./Titlepage.tex)
[3] (./Copyright.tex
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/omscmr.fd)) [4]
(./thesis.toc [2] [3]) [4] (./thesis.lof
Overfull \hbox (14.12067pt too wide) in paragraph at lines 3--3
 [][] [][][]\OT1/cmr/m/n/12 Twelve light curves for mea-sured BATSE GRBs [[][]2
[][]]. The short timescales 
[5]
Overfull \hbox (18.10568pt too wide) in paragraph at lines 15--15
 \OT1/cmr/m/n/12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 03\OML/cmm/m/it/12 ; \OT1/c
mr/m/n/12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 25\OML/cmm/m/it/12 ; \OT1/cmr/m/n/
12 0\OML/cmm/m/it/12 :\OT1/cmr/m/n/12 5\OML/cmm/m/it/12 ; \OT1/cmr/m/n/12 1\OML
/cmm/m/it/12 :\OT1/cmr/m/n/12 0$ for the WMAP5 Fidu-cial (solid black), WMAP5+F
ixed 
[6] [7] [8] [9] [10] [11] [12]
Overfull \hbox (0.82274pt too wide) in paragraph at lines 59--59
 \OT1/cmr/m/n/12 cles (NKG) and elec-tro-mag-netic shower en-ergy (NKG/R) in a 
gamma- 
[13] [14] [15] [16] [17] [18] [19] [20] [21] [22]) [23] (./Abbreviations.tex)
[24] (./GRBs.tex
Chapter 1.
pdfTeX warning (ext4): destination with the same identifier (name{page.1}) has 
been already used, duplicate ignored
<to be read again> 
                   \relax 
l.26 
      [1]pdfTeX warning (ext4): destination with the same identifier (name{page
.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.49 
      [2]pdfTeX warning (ext4): destination with the same identifier (name{page
.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.73 \newpage
              [3]pdfTeX warning (ext4): destination with the same identifier (n
ame{page.4}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.88 \newpage
              [4] [5] <figures/batse_t90.png, id=1463, 931.48pt x 692.5875pt>
<use figures/batse_t90.png> [6 <./figures/batse_t90.png>]
<figures/batse_panel.png, id=1472, 923.45pt x 911.405pt>
<use figures/batse_panel.png> [7 <./figures/batse_panel.png>] [8]
<figures/bandfuncfig.pdf, id=1494, 612.09195pt x 615.50294pt>
<use figures/bandfuncfig.pdf> [9 <./figures/bandfuncfig.pdf>]
<figures/batse_spatial.png, id=1513, 980.66376pt x 706.64pt>
<use figures/batse_spatial.png> [10 <./figures/batse_spatial.png>] [11]
<figures/jetbreak.png, id=1530, 619.31375pt x 478.78876pt>
<use figures/jetbreak.png> [12 <./figures/jetbreak.png>] [13]
<figures/redshift.png, id=1557, 1025.8325pt x 832.10875pt>
<use figures/redshift.png> [14 <./figures/redshift.png>] [15]
<figures/fluenceratio.png, id=1580, 706.64pt x 689.57625pt>
<use figures/fluenceratio.png> [16 <./figures/fluenceratio.png>] [17]
<figures/fermicutoff.png, id=1596, 960.58875pt x 728.7225pt>
<use figures/fermicutoff.png> [18 <./figures/fermicutoff.png>] [19]
<figures/hess_scheme.jpg, id=1617, 413.545pt x 385.44pt>
<use figures/hess_scheme.jpg>
<figures/wct.jpg, id=1618, 602.25pt x 615.29875pt> <use figures/wct.jpg>
[20 <./figures/hess_scheme.jpg> <./figures/wct.jpg>] [21] [22]
<figures/EffArea.png, id=1651, 734.9859pt x 445.9059pt>
<use figures/EffArea.png> [23 <./figures/EffArea.png>] [24]
<figures/fireballmodel.png, id=1670, 1154.3125pt x 899.36pt>
<use figures/fireballmodel.png> [25 <./figures/fireballmodel.png>] [26]
[27] [28] [29] [30]
<figures/short_grb_cutoff.png, id=1732, 800.9925pt x 677.53125pt>
<use figures/short_grb_cutoff.png> [31 <./figures/short_grb_cutoff.png>]
[32] <figures/ebl_flux.png, id=1751, 1090.0725pt x 921.4425pt>
<use figures/ebl_flux.png> [33 <./figures/ebl_flux.png>]
<figures/gilmore_2012_EBL_atten.png, id=1766, 667.49374pt x 649.42625pt>
<use figures/gilmore_2012_EBL_atten.png> [34 <./figures/gilmore_2012_EBL_atten.
png>] [35]) [36] (./Showers.tex
Chapter 2.
[37] [38]
Overfull \hbox (12.82234pt too wide) in paragraph at lines 36--41
\OT1/cmr/m/n/12 The elec-tron and positron pair sub-se-quently gen-er-ate more 
pho-tons via Bremsstrahlung
[39] <figures/gamma_shower_model.png, id=1814, 650.43pt x 502.87875pt>
<use figures/gamma_shower_model.png> [40] [41 <./figures/gamma_shower_model.png
>] <figures/gamma_shower_profile.png, id=1832, 1200.485pt x 875.27pt>
<use figures/gamma_shower_profile.png> [42 <./figures/gamma_shower_profile.png>
] [43] <figures/eas_diagram.png, id=1855, 410.53375pt x 658.46pt>
<use figures/eas_diagram.png> [44] [45 <./figures/eas_diagram.png>] [46]
<figures/proton_shower_profile.png, id=1879, 1200.485pt x 875.27pt>
<use figures/proton_shower_profile.png> [47 <./figures/proton_shower_profile.pn
g>] <figures/proton_particle_number.png, id=1886, 634.37pt x 718.685pt>
<use figures/proton_particle_number.png> [48 <./figures/proton_particle_number.
png>] [49] <figures/shower_timing.png, id=1903, 562.1pt x 628.3475pt>
<use figures/shower_timing.png> [50 <./figures/shower_timing.png>]
<figures/side_shower.png, id=1914, 608.2725pt x 744.7825pt>
<use figures/side_shower.png>) [51] [52 <./figures/side_shower.png>]
(./HAWC.tex
Chapter 3.
[53] <figures/HAWC_overview.jpeg, id=1933, 1080.035pt x 725.71124pt>
<use figures/HAWC_overview.jpeg> [54 <./figures/HAWC_overview.jpeg>] [55]
<figures/HAWC_tank.png, id=1944, 839.135pt x 688.5725pt>
<use figures/HAWC_tank.png>
<figures/HAWC_bladder.png, id=1945, 182.1204pt x 168.63pt>
<use figures/HAWC_bladder.png> [56 <./figures/HAWC_tank.png> <./figures/HAWC_bl
adder.png>] [57] <figures/regularpulse.png, id=1957, 520.94624pt x 706.64pt>
<use figures/regularpulse.png>
<figures/HAWC_pmt.png, id=1958, 171.039pt x 227.8914pt>
<use figures/HAWC_pmt.png> [58 <./figures/regularpulse.png> <./figures/HAWC_pmt
.png>] [59] <figures/single_pe_charge.jpeg, id=1975, 990.70125pt x 736.7525pt>
<use figures/single_pe_charge.jpeg> [60 <./figures/single_pe_charge.jpeg>]
[61] <figures/r5912_quantum_efficiency.png, id=1987, 610.28pt x 664.4825pt>
<use figures/r5912_quantum_efficiency.png>
<figures/r7081_HQE_quantum_efficiency.png, id=1988, 546.04pt x 696.6025pt>
<use figures/r7081_HQE_quantum_efficiency.png> [62 <./figures/r5912_quantum_eff
iciency.png> <./figures/r7081_HQE_quantum_efficiency.png>] [63]
<figures/signal_overview.png, id=2003, 914.41624pt x 311.1625pt>
<use figures/signal_overview.png> [64 <./figures/signal_overview.png>] [65]
<figures/coax_diagram.png, id=2016, 484.81125pt x 483.8075pt>
<use figures/coax_diagram.png> [66 <./figures/coax_diagram.png>]
<figures/circuit.png, id=2031, 860.21375pt x 442.65375pt>
<use figures/circuit.png> [67 <./figures/circuit.png>] [68] [69]
<figures/comp_cable.png, id=2059, 1200.485pt x 875.27pt>
<use figures/comp_cable.png> [70 <./figures/comp_cable.png>]
<figures/analog_circuit.png, id=2067, 1186.4325pt x 665.48625pt>
<use figures/analog_circuit.png> [71 <./figures/analog_circuit.png>] [72]
[73] [74] <figures/AnalogFEB_4edge.png, id=2097, 1202.4925pt x 878.28125pt>
<use figures/AnalogFEB_4edge.png> [75 <./figures/AnalogFEB_4edge.png>]
<figures/AnalogFEB_2edge.png, id=2107, 1202.4925pt x 878.28125pt>
<use figures/AnalogFEB_2edge.png> [76 <./figures/AnalogFEB_2edge.png>]
<figures/digital_logic.png, id=2115, 968.61874pt x 628.3475pt>
<use figures/digital_logic.png> [77 <./figures/digital_logic.png>]
<figures/latch_circuit.png, id=2124, 894.34125pt x 481.8pt>
<use figures/latch_circuit.png> [78 <./figures/latch_circuit.png>]
<figures/flip_flop_logic.png, id=2130, 352.31625pt x 269.005pt>
<use figures/flip_flop_logic.png>
<figures/logic_table.png, id=2131, 666.49pt x 470.75874pt>
<use figures/logic_table.png> [79 <./figures/flip_flop_logic.png> <./figures/lo
gic_table.png>]
<figures/flip_flop_20ns.png, id=2141, 700.6175pt x 476.78125pt>
<use figures/flip_flop_20ns.png> [80 <./figures/flip_flop_20ns.png>]
<figures/one-shot_width_vs_R.png, id=2146, 901.3675pt x 777.90625pt>
<use figures/one-shot_width_vs_R.png> [81 <./figures/one-shot_width_vs_R.png>]
[82] <figures/delay_circuit.png, id=2158, 697.60625pt x 202.7575pt>
<use figures/delay_circuit.png> [83 <./figures/delay_circuit.png>] [84]
<figures/DigitalFEB_4edge.png, id=2176, 1202.4925pt x 426.59375pt>
<use figures/DigitalFEB_4edge.png>
Overfull \hbox (43.36244pt too wide) in paragraph at lines 595--596
 [] 
[85 <./figures/DigitalFEB_4edge.png>] [86]
<figures/DigitalFEB_2edge.png, id=2195, 1202.4925pt x 426.59375pt>
<use figures/DigitalFEB_2edge.png>
Overfull \hbox (43.36244pt too wide) in paragraph at lines 638--639
 [] 
[87 <./figures/DigitalFEB_2edge.png>] [88] [89]
<figures/early_TDC_event.png, id=2218, 855.195pt x 610.28pt>
<use figures/early_TDC_event.png> [90 <./figures/early_TDC_event.png>] [91]
<figures/online_reco_chain.png, id=2233, 1038.88126pt x 591.20876pt>
<use figures/online_reco_chain.png> [92 <./figures/online_reco_chain.png>]
<figures/timediagram.png, id=2240, 1013.7875pt x 633.36626pt>
<use figures/timediagram.png> [93 <./figures/timediagram.png>] [94]
<figures/OnlineLatencyBigBins.png, id=2254, 922.44624pt x 617.30624pt>
<use figures/OnlineLatencyBigBins.png> [95 <./figures/OnlineLatencyBigBins.png>
] [96]
<figures/Calibration_Simplified_Layout.png, id=2269, 794.4882pt x 654.2844pt>
<use figures/Calibration_Simplified_Layout.png> [97 <./figures/Calibration_Simp
lified_Layout.png>]
<figures/chargecalib_curves_run5213_H13.png, id=2274, 1367.1075pt x 701.62125pt
> <use figures/chargecalib_curves_run5213_H13.png> [98 <./figures/chargecalib_c
urves_run5213_H13.png>]
<figures/H13_slewing.png, id=2280, 999.735pt x 774.895pt>
<use figures/H13_slewing.png> [99 <./figures/H13_slewing.png>] [100] [101]
[102] [103] <figures/10inch_lostart.png, id=2321, 800.9925pt x 577.15625pt>
<use figures/10inch_lostart.png>
<figures/10inch_histart.png, id=2322, 798.985pt x 574.145pt>
<use figures/10inch_histart.png> [104 <./figures/10inch_lostart.png> <./figures
/10inch_histart.png>]
<figures/8inch_lostart.png, id=2329, 798.985pt x 574.145pt>
<use figures/8inch_lostart.png>
<figures/8inch_histart.png, id=2330, 798.985pt x 574.145pt>
<use figures/8inch_histart.png> [105 <./figures/8inch_lostart.png> <./figures/8
inch_histart.png>] [106]
<figures/afterpulsing_rate.png, id=2345, 937.5025pt x 669.50125pt>
<use figures/afterpulsing_rate.png> [107 <./figures/afterpulsing_rate.png>]
Overfull \hbox (0.59285pt too wide) in paragraph at lines 970--974
\OT1/cmr/m/n/12 for ion-iza-tion oc-cur-ring a dis-tance $\OML/cmm/m/it/12 s$ \
OT1/cmr/m/n/12 from the pho-to-cath-ode. The af-ter-pulse timescale
[108] [109] <figures/afterpulse_outer.png, id=2365, 1200.485pt x 875.27pt>
<use figures/afterpulse_outer.png>
<figures/afterpulse_central.png, id=2366, 1200.485pt x 875.27pt>
<use figures/afterpulse_central.png> [110 <./figures/afterpulse_outer.png> <./f
igures/afterpulse_central.png>]) (./Reco.tex
Chapter 4.
[111] <figures/edgestream.png, id=2391, 902.37125pt x 209.78375pt>
<use figures/edgestream.png> [112 <./figures/edgestream.png>] [113] [114]
<figures/LoTOT.png, id=2411, 798.985pt x 574.145pt> <use figures/LoTOT.png>
<figures/HiTOT.png, id=2412, 798.985pt x 574.145pt> <use figures/HiTOT.png>
<figures/T01.png, id=2413, 798.985pt x 574.145pt> <use figures/T01.png>
<figures/T23.png, id=2414, 798.985pt x 574.145pt> <use figures/T23.png>
[115 <./figures/LoTOT.png> <./figures/HiTOT.png> <./figures/T01.png> <./figures
/T23.png>] [116] <figures/SFCF.png, id=2433, 710.655pt x 499.8675pt>
<use figures/SFCF.png> [117 <./figures/SFCF.png>] [118]
<figures/gamma_sim.png, id=2452, 795.97375pt x 533.995pt>
<use figures/gamma_sim.png>
<figures/proton_sim.png, id=2453, 801.99625pt x 533.995pt>
<use figures/proton_sim.png> [119 <./figures/gamma_sim.png> <./figures/proton_s
im.png>] <figures/likely_gamma.png, id=2464, 801.99625pt x 539.01375pt>
<use figures/likely_gamma.png>
<figures/likely_hadron.png, id=2465, 803.0pt x 542.025pt>
<use figures/likely_hadron.png>
Overfull \hbox (9.47742pt too wide) in paragraph at lines 218--229
[][]     [][] 
[120 <./figures/likely_gamma.png> <./figures/likely_hadron.png>] [121]
<figures/curvature_correct.png, id=2486, 718.685pt x 548.0475pt>
<use figures/curvature_correct.png> [122 <./figures/curvature_correct.png>]
<figures/angle_v_energy.png, id=2496, 765.86125pt x 602.25pt>
<use figures/angle_v_energy.png> [123 <./figures/angle_v_energy.png>] [124]
[125]
<figures/SP-invcompact-demo-20160404.png, id=2520, 2849.64626pt x 2269.47874pt>
<use figures/SP-invcompact-demo-20160404.png> [126 <./figures/SP-invcompact-dem
o-20160404.png>]
Overfull \hbox (4.36082pt too wide) in paragraph at lines 375--383
[]\OT1/cmr/m/n/12 The asym-me-tries present in the spa-tial dis-tri-bu-tion of 
shower en-ergy in hadronic
[127] <figures/pinc.png, id=2535, 998.73125pt x 662.475pt>
<use figures/pinc.png> [128 <./figures/pinc.png>]
<figures/SP-pinc-demo-20160404.png, id=2543, 2827.56375pt x 2269.47874pt>
<use figures/SP-pinc-demo-20160404.png> [129 <./figures/SP-pinc-demo-20160404.p
ng>] <figures/Crab_SP_RC0v2.jpg, id=2554, 367.3725pt x 412.54124pt>
<use figures/Crab_SP_RC0v2.jpg>
<figures/crab_excess.png, id=2555, 730.73pt x 692.5875pt>
<use figures/crab_excess.png>) [130] [131 <./figures/Crab_SP_RC0v2.jpg>]
[132 <./figures/crab_excess.png>] (./Method.tex
Chapter 5.
[133] [134] [135] [136]
<figures/exampleskymap.png, id=2597, 800.9925pt x 577.15625pt>
<use figures/exampleskymap.png> [137 <./figures/exampleskymap.png>] [138]
<figures/timediagram_two.png, id=2608, 874.26625pt x 570.13pt>
<use figures/timediagram_two.png> [139 <./figures/timediagram_two.png>]
[140] <figures/exbackground.png, id=2623, 798.985pt x 574.145pt>
<use figures/exbackground.png> [141 <./figures/exbackground.png>] [142]
<figures/poisson_check1.png, id=2638, 800.9925pt x 577.15625pt>
<use figures/poisson_check1.png> [143 <./figures/poisson_check1.png>] [144]
[145] [146] [147]
<figures/backstudy_pgraph_p2sec.png, id=2666, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_p2sec.png>

LaTeX Warning: Float too large for page by 7.41559pt on input line 281.

<figures/backstudy_pgraph_1sec.png, id=2671, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_1sec.png>
<figures/backstudy_pgraph_10sec.png, id=2676, 800.9925pt x 777.90625pt>
<use figures/backstudy_pgraph_10sec.png>

LaTeX Warning: Float too large for page by 9.7489pt on input line 319.

) [148 <./figures/backstudy_pgraph_p2sec.png>] [149 <./figures/backstudy_pgraph
_1sec.png>] [150 <./figures/backstudy_pgraph_10sec.png>] (./Trials.tex [151]
[152] [153] [154] <figures/inde_pdist.png, id=2728, 698.61pt x 875.27pt>
<use figures/inde_pdist.png>
<figures/inde_trials.png, id=2729, 698.61pt x 875.27pt>
<use figures/inde_trials.png> [155 <./figures/inde_pdist.png> <./figures/inde_t
rials.png>] [156] [157] <figures/corr_pdist.png, id=2750, 698.61pt x 875.27pt>
<use figures/corr_pdist.png>
<figures/wtangent.png, id=2751, 698.61pt x 875.27pt>
<use figures/wtangent.png> [158 <./figures/corr_pdist.png> <./figures/wtangent.
png>] [159] <figures/gcumulative_1sec.png, id=2777, 1200.485pt x 875.27pt>
<use figures/gcumulative_1sec.png> [160 <./figures/gcumulative_1sec.png>]
<figures/gcorrection_p2sec.png, id=2783, 1200.485pt x 875.27pt>
<use figures/gcorrection_p2sec.png>
<figures/gcumulative_corr_p2sec.png, id=2784, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_p2sec.png> [161 <./figures/gcorrection_p2sec.png>
 <./figures/gcumulative_corr_p2sec.png>]
<figures/gcorrection_1sec.png, id=2792, 1200.485pt x 875.27pt>
<use figures/gcorrection_1sec.png>
<figures/gcumulative_corr_1sec.png, id=2793, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_1sec.png> [162 <./figures/gcorrection_1sec.png> <
./figures/gcumulative_corr_1sec.png>]
<figures/gcorrection_10sec.png, id=2800, 1200.485pt x 875.27pt>
<use figures/gcorrection_10sec.png>
<figures/gcumulative_corr_10sec.png, id=2801, 1200.485pt x 875.27pt>
<use figures/gcumulative_corr_10sec.png> [163 <./figures/gcorrection_10sec.png>
 <./figures/gcumulative_corr_10sec.png>] [164]
<figures/gcorrection_time_p2sec.png, id=2816, 917.4275pt x 754.82pt>
<use figures/gcorrection_time_p2sec.png> [165 <./figures/gcorrection_time_p2sec
.png>] <figures/gcorrection_time_1sec.png, id=2822, 914.41624pt x 747.79375pt>
<use figures/gcorrection_time_1sec.png> [166 <./figures/gcorrection_time_1sec.p
ng>] <figures/gcorrection_time_10sec.png, id=2829, 912.40875pt x 741.77126pt>
<use figures/gcorrection_time_10sec.png> [167 <./figures/gcorrection_time_10sec
.png>] [168]) [169] (./Sensitivity.tex
Chapter 6.
[170] [171] [172] [173]
<figures/psf_geom.png, id=2881, 937.5025pt x 500.87125pt>
<use figures/psf_geom.png> [174 <./figures/psf_geom.png>]
<figures/sens_v_spatial_bin_size.png, id=2889, 1200.485pt x 875.27pt>
<use figures/sens_v_spatial_bin_size.png> [175 <./figures/sens_v_spatial_bin_si
ze.png>] [176] [177] [178] [179]
<figures/sensitivity_v_tophat_radius_bg1000.png, id=2927, 1200.485pt x 875.27pt
> <use figures/sensitivity_v_tophat_radius_bg1000.png> [180 <./figures/sensitiv
ity_v_tophat_radius_bg1000.png>]
<figures/sensitivity_v_tophat_radius_bg_p1.png, id=2932, 1200.485pt x 875.27pt>
<use figures/sensitivity_v_tophat_radius_bg_p1.png> [181 <./figures/sensitivity
_v_tophat_radius_bg_p1.png>] [182] [183] [184] [185] [186]
<figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png, id=2973, 1200.485p
t x 875.27pt> <use figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png>
[187 <./figures/redshift0p5_index1p6_duration1p0_flux5e5_dec40.png>]
<figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png, id=2980, 1200.485
pt x 875.27pt>
<use figures/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png> [188 <./figur
es/redshift0p5_index2p0_duration10p0_flux5e6_dec40.png>] [189] [190]
<figures/grb_cuts_near_crab.png, id=3003, 669.50125pt x 563.10374pt>
<use figures/grb_cuts_near_crab.png> [191 <./figures/grb_cuts_near_crab.png>]
[192] [193] <figures/sensitivity_money.png, id=3032, 1200.485pt x 875.27pt>
<use figures/sensitivity_money.png> [194 <./figures/sensitivity_money.png>]
<figures/sensitivity_money_long.png, id=3039, 1200.485pt x 875.27pt>
<use figures/sensitivity_money_long.png> [195 <./figures/sensitivity_money_long
.png>] [196] <figures/bg_corrected_fermi.png, id=3060, 1200.485pt x 875.27pt>
<use figures/bg_corrected_fermi.png>
<figures/grb090510_on_hawc.png, id=3061, 1200.485pt x 875.27pt>
<use figures/grb090510_on_hawc.png> [197 <./figures/bg_corrected_fermi.png>]
[198 <./figures/grb090510_on_hawc.png>] [199] [200] [201] [202]) [203] [204]
(./Results.tex
Chapter 7.
[205] [206] <figures/datapie.png, id=3124, 985.6825pt x 631.35875pt>
<use figures/datapie.png> [207 <./figures/datapie.png>] [208] [209]
<figures/rate1_zoom.png, id=3152, 798.985pt x 574.145pt>
<use figures/rate1_zoom.png> [210 <./figures/rate1_zoom.png>]
<figures/inlay.png, id=3158, 987.69pt x 716.6775pt> <use figures/inlay.png>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 159--161
 [] 
[211 <./figures/inlay.png>]
<figures/candidate_lightcurve.png, id=3164, 899.36pt x 574.145pt>
<use figures/candidate_lightcurve.png> [212 <./figures/candidate_lightcurve.png
>] <figures/lc_coarse.png, id=3171, 798.985pt x 574.145pt>
<use figures/lc_coarse.png> [213 <./figures/lc_coarse.png>]
<figures/candidate_location_full_skymap.png, id=3177, 433.62pt x 487.8225pt>
<use figures/candidate_location_full_skymap.png>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 208--210
 [] 
[214 <./figures/candidate_location_full_skymap.png>] [215] [216] [217] [218]
<figures/limit_grbrate.png, id=3217, 1200.485pt x 875.27pt>
<use figures/limit_grbrate.png> [219 <./figures/limit_grbrate.png>]
<figures/grbrate_long.png, id=3224, 1200.485pt x 875.27pt>
<use figures/grbrate_long.png> [220 <./figures/grbrate_long.png>] [221])
[222] (./AppendixC.tex
Appendix A.

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\Gamma' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `subscript' on input line 5.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 5.

[223] [224]) [225] (./AppendixB.tex
Appendix B.
[226] [227]) [228] (./AppendixD.tex
Appendix C.
<figures/analog_input_circuit.png, id=3308, 310.15875pt x 229.85875pt>
<use figures/analog_input_circuit.png> [229 <./figures/analog_input_circuit.png
>]) [230] (./AppendixE.tex
Appendix D.
<figures/analog_load_circuit.png, id=3324, 845.1575pt x 345.29pt>
<use figures/analog_load_circuit.png> [231 <./figures/analog_load_circuit.png>]
) [232] (./AppendixF.tex
Appendix E.
<figures/milagro_pmt_base_via_bob_28nov11.pdf, id=3347, 614.295pt x 794.97pt>
<use figures/milagro_pmt_base_via_bob_28nov11.pdf>
Overfull \hbox (7.22745pt too wide) in paragraph at lines 37--38
 [] 
) [233]

LaTeX Warning: Text page 234 contains only floats.

[234 <./figures/milagro_pmt_base_via_bob_28nov11.pdf>] (./thesis.bbl
Underfull \hbox (badness 2213) in paragraph at lines 19--22
[]\OT1/cmr/m/n/12 M. Briggs.  Gamma-Ray As-tro-physics NSSTC BATSE GRB.  \OT1/c
mr/m/it/12 URL
[235]
Underfull \hbox (badness 3407) in paragraph at lines 139--142
[]\OT1/cmr/m/n/12 S. et al. Woose-ley.  The Su-per-nova Gamma-ray Burst Con-nec
-tion.
[236] [237] [238]
Underfull \hbox (badness 3439) in paragraph at lines 429--434
[]\OT1/cmr/m/n/12 E. Fer-rara.  Caveats About An-a-lyz-ing LAT Pass 8 Data.  \O
T1/cmr/m/it/12 URL

Underfull \hbox (badness 10000) in paragraph at lines 436--441
[]\OT1/cmr/m/n/12 Fermi LAT Col-lab-o-ra-tion.  Fermi LAT GRBs.  \OT1/cmr/m/it/
12 URL

Underfull \hbox (badness 10000) in paragraph at lines 443--447
[]\OT1/cmr/m/n/12 S. No-bili.  GRB 130427A: A CHANCE NOT TO MISS.
[239]) [240] (./thesis.aux (./Abstract.aux) (./Titlepage.aux) (./Copyright.aux)
 (./Abbreviations.aux) (./GRBs.aux) (./Showers.aux) (./HAWC.aux) (./Reco.aux)
(./Method.aux) (./Trials.aux) (./Sensitivity.aux) (./Results.aux)
(./AppendixC.aux) (./AppendixB.aux) (./AppendixD.aux) (./AppendixE.aux)
(./AppendixF.aux)) )
(see the transcript file for additional information)</usr/local/texlive/2015/te
xmf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2015/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2015/texm
f-dist/fonts/type1/public/amsfonts/cm/cmmi12.pfb></usr/local/texlive/2015/texmf
-dist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2015/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmmi8.pfb></usr/local/texlive/2015/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2015/texmf-dist/
fonts/type1/public/amsfonts/cm/cmr12.pfb></usr/local/texlive/2015/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmr6.pfb></usr/local/texlive/2015/texmf-dist/fonts
/type1/public/amsfonts/cm/cmr8.pfb></usr/local/texlive/2015/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2015/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmsy6.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1
/public/amsfonts/cm/cmsy8.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmti12.pfb>
Output written on thesis.pdf (267 pages, 9013216 bytes).
Transcript written on thesis.log.

